DepthFM: Fast Monocular Depth Estimation with Flow Matching

Current discriminative depth estimation methods often produce blurry artifacts, while generative approaches suffer from slow sampling due to curvatures in the noise-to-depth transport. Our method addresses these challenges by framing depth estimation as a direct transport between image and depth distributions. We are the first to explore flow matching in this field, and we demonstrate that its interpolation trajectories enhance both training and sampling efficiency while preserving high performance. While generative models typically require extensive training data, we mitigate this dependency by integrating external knowledge from a pre-trained image diffusion model, enabling effective transfer even across differing objectives. To further boost our model performance, we employ synthetic data and utilize image-depth pairs generated by a discriminative model on an in-the-wild image dataset. As a generative model, our model can reliably estimate depth confidence, which provides an additional advantage. Our approach achieves competitive zero-shot performance on standard benchmarks of complex natural scenes while improving sampling efficiency and only requiring minimal synthetic data for training.

==> full_bibtex_rm_later.tex <==
% Long form of conference & journal abbreviations -- especially for camera ready
@String(PAMI  = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV  = {Int. J. Comput. Vis.})
@String(CVPR  = {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV  = {Int. Conf. Comput. Vis.})
@String(ECCV  = {Eur. Conf. Comput. Vis.})
@String(NeurIPS = {Adv. Neural Inform. Process. Syst.})
@String(ICML  = {Int. Conf. Mach. Learn.})
@String(ICLR  = {Int. Conf. Learn. Represent.})
@String(ACCV  = {Asian Conf. Comput. Vis.})
@String(BMVC  = {Brit. Mach. Vis. Conf.})
@String(CVPRW = {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(AAAI  = {AAAI})
@String(IJCAI = {IJCAI})
@String(ICIP  = {IEEE Int. Conf. Image Process.})
@String(ICPR  = {Int. Conf. Pattern Recog.})
@String(ICASSP=	{ICASSP})
@String(ICME  = {Int. Conf. Multimedia and Expo})
@String(JMLR  = {J. Mach. Learn. Res.})
@String(TMLR  = {Trans. Mach. Learn Res.})
@String(TOG   = {ACM Trans. Graph.})
@String(TIP   = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TCSVT = {IEEE Trans. Circuit Syst. Video Technol.})
@String(TMM   = {IEEE Trans. Multimedia})
@String(ACMMM = {ACM Int. Conf. Multimedia})
@String(PR    = {Pattern Recognition})

@String(MNI	  = {Nature Mach. Intell.})
@String(SPL	  = {IEEE Sign. Process. Letters})
@String(VR    = {Vis. Res.})
@String(JOV	  = {J. Vis.})
@String(TVC   = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF   = {Comput. Graph. Forum})
@String(CVM   = {Computational Visual Media})


% Short form of conference & journal abbreviations -- especially for submission version
% if desired, remove these macros in favor of the above ones
@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NeurIPS = {NeurIPS})
@String(ICML  = {ICML})
@String(ICLR  = {ICLR})
@String(ACCV  = {ACCV})
@String(BMVC  =	{BMVC})
@String(CVPRW = {CVPRW})
@String(AAAI  = {AAAI})
@String(IJCAI = {IJCAI})
@String(ICIP  = {ICIP})
@String(ICPR  = {ICPR})
@String(ICASSP=	{ICASSP})
@String(ICME  =	{ICME})
@String(JMLR  = {JMLR})
@String(TMLR  = {TMLR})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(PR    = {PR})


@inproceedings{tong2023improving,
  title={Improving and generalizing flow-based generative models with minibatch optimal transport},
  author={Tong, Alexander and Malkin, Nikolay and Huguet, Guillaume and Zhang, Yanlei and Rector-Brooks, Jarrid and Fatras, Kilian and Wolf, Guy and Bengio, Yoshua},
  booktitle={ICML Workshop on New Frontiers in Learning, Control, and Dynamical Systems},
  year={2023}
}

@article{albergo2023stochastic,
  title={Stochastic interpolants with data-dependent couplings},
  author={Albergo, Michael S and Goldstein, Mark and Boffi, Nicholas M and Ranganath, Rajesh and Vanden-Eijnden, Eric},
  journal={arXiv},
  year={2023}
}

@InProceedings{ke2023marigold,
        title={Repurposing Diffusion-Based Image Generators for Monocular Depth Estimation},
        author={Bingxin Ke and Anton Obukhov and Shengyu Huang and Nando Metzger and Rodrigo Caye Daudt and Konrad Schindler},
        booktitle = {CVPR},
        year={2024}
}

@article{yan2023_diffusionwithoutattention,
  title={Diffusion models without attention},
  author={Yan, Jing Nathan and Gu, Jiatao and Rush, Alexander M},
  journal={arXiv},
  year={2023}
}

@article{schusterbauer2023boosting,  
title={Boosting Latent Diffusion with Flow Matching},  
author={Schusterbauer, Johannes and Gui, Ming and Ma, Pingchuan and Stracke, Nick and Baumann, Stefan A and Ommer, Bj{\"o}rn}, 
journal={ECCV},  
year={2024}
}

@misc{unsplash,
    title = {{Unsplash} {\textbar} \url{https://unsplash.com/data}},
    author={Unsplash},
    url = {https://unsplash.com/data},
    language = {en},
    urldate = {2023-11-17},
}

@inproceedings{esser2021taming,
  title={Taming transformers for high-resolution image synthesis},
  author={Esser, Patrick and Rombach, Robin and Ommer, Bjorn},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={12873--12883},
  year={2021}
}

@misc{sora,
  author = "OpenAI",
  title = "Sora: Creating video from text",
  year = "2024",
  url = "https://openai.com/sora",
}

@article{yu2023robustifying,
  title={Robustifying State-space Models for Long Sequences via Approximate Diagonalization},
  author={Yu, Annan and Nigmetov, Arnur and Morozov, Dmitriy and Mahoney, Michael W and Erichson, N Benjamin},
  journal={arXiv preprint arXiv:2310.01698},
  year={2023}
}

@article{kitaev2020reformer,
  title={Reformer: The efficient transformer},
  author={Kitaev, Nikita and Kaiser, {\L}ukasz and Levskaya, Anselm},
  journal={arXiv preprint arXiv:2001.04451},
  year={2020}
}
@inproceedings{swin_transformer,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={10012--10022},
  year={2021}
}

@article{choromanski2020rethinking,
  title={Rethinking attention with performers},
  author={Choromanski, Krzysztof and Likhosherstov, Valerii and Dohan, David and Song, Xingyou and Gane, Andreea and Sarlos, Tamas and Hawkins, Peter and Davis, Jared and Mohiuddin, Afroz and Kaiser, Lukasz and others},
  journal={arXiv preprint arXiv:2009.14794},
  year={2020}
}


@inproceedings{sgfm,
  title = {Guided Diffusion from Self-Supervised Diffusion Features},
  author = {Hu, Vincent Tao and Chen, Yunlu and Caron, Mathilde and Asano, Yuki M. and Snoek, Cees G.M. and Ommer, Björn},
  year = {2023},
  booktitle = {ARXIV},
}

@inproceedings{motionfm,
  title = {Motion Flow Matching for Human Motion Synthesis and Editing},
  author = {Hu, Vincent Tao and Yin, Wenzhe and Ma, Pingchuan and Chen, Yunlu and Fernando, Basura and Asano, Yuki M. and Gavves, Efstratios and Mettes, Pascal and Ommer, Björn and Snoek, Cees G.M.},
  year = {2023},
  booktitle = {arxiv},
}


@article{liu2022flow,
  title={Flow straight and fast: Learning to generate and transfer data with rectified flow},
  author={Liu, Xingchao and Gong, Chengyue and Liu, Qiang},
  journal={arXiv},
  year={2022}
}

@inproceedings{esser2021taming_vqgan,
  title={Taming transformers for high-resolution image synthesis},
  author={Esser, Patrick and Rombach, Robin and Ommer, Bjorn},
  booktitle={CVPR},
  year={2021}
}


@article{actionmatching,
  title={Action Matching: A Variational Method for Learning Stochastic Dynamics from Samples},
  author={Neklyudov, Kirill and Severo, Daniel and Makhzani, Alireza},
  journal={arXiv},
  year={2022}
}

@article{rectifiedflow_iclr23,
  title={Flow straight and fast: Learning to generate and transfer data with rectified flow},
  author={Liu, Xingchao and Gong, Chengyue and Liu, Qiang},
  journal={ICLR},
  year={2023}
}

@article{neuralode_chen2018neural,
  title={Neural ordinary differential equations},
  author={Chen, Ricky TQ and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David K},
  journal={NeurIPS},
  year={2018}
}

@inproceedings{shen2020interpreting,
  title     = {Interpreting the Latent Space of GANs for Semantic Face Editing},
  author    = {Shen, Yujun and Gu, Jinjin and Tang, Xiaoou and Zhou, Bolei},
  booktitle = {CVPR},
  year      = {2020}
}

@article{chen2023riemannian,
  title={Riemannian flow matching on general geometries},
  author={Chen, Ricky TQ and Lipman, Yaron},
  journal={arXiv},
  year={2023}
}

@article{wu2022fast,
  title={Fast Point Cloud Generation with Straight Flows},
  author={Wu, Lemeng and Wang, Dilin and Gong, Chengyue and Liu, Xingchao and Xiong, Yunyang and Ranjan, Rakesh and Krishnamoorthi, Raghuraman and Chandra, Vikas and Liu, Qiang},
  journal={arXiv},
  year={2022}
}

@article{davtyan2022randomized,
  title={Randomized Conditional Flow Matching for Video Prediction},
  author={Davtyan, Aram and Sameni, Sepehr and Favaro, Paolo},
  journal={arXiv},
  year={2022}
}

@article{dit_peebles2022scalable,
  title={Scalable Diffusion Models with Transformers},
  author={Peebles, William and Xie, Saining},
  journal={arXiv},
  year={2022}
}

@article{yang2022your,
  title={Your vit is secretly a hybrid discriminative-generative diffusion model},
  author={Yang, Xiulong and Shih, Sheng-Min and Fu, Yinlin and Zhao, Xiaoting and Ji, Shihao},
  journal={arXiv},
  year={2022}
}

@inproceedings{ffhq_karras2019style,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle=CVPR,
  year={2019}
}
@article{uvit,
  title={All are Worth Words: a ViT Backbone for Score-based Diffusion Models},
  author={Bao, Fan and Li, Chongxuan and Cao, Yue and Zhu, Jun},
  journal=CVPR,
  year={2023}
}

@article{safeldm,
  title={Safe Latent Diffusion: Mitigating Inappropriate Degeneration in Diffusion Models},
  author={Schramowski, Patrick and Brack, Manuel and Deiseroth, Bj{\"o}rn and Kersting, Kristian},
  journal={arXiv},
  year={2022}
}


@article{forgetmenot,
  title={Forget-Me-Not: Learning to Forget in Text-to-Image Diffusion Models},
  author={Zhang, Eric and Wang, Kai and Xu, Xingqian and Wang, Zhangyang and Shi, Humphrey},
  journal={arXiv},
  year={2023}
}

@article{esd,
  title={Erasing Concepts from Diffusion Models},
  author={Gandikota, Rohit and Materzynska, Joanna and Fiotto-Kaufman, Jaden and Bau, David},
  journal={arXiv},
  year={2023}
}

@inproceedings{kim2022diffusionclip,
  title={Diffusionclip: Text-guided diffusion models for robust image manipulation},
  author={Kim, Gwanghyun and Kwon, Taesung and Ye, Jong Chul},
  booktitle=CVPR,
  year={2022}
}

@article{huberman2023edit,
  title={An Edit Friendly DDPM Noise Space: Inversion and Manipulations},
  author={Huberman-Spiegelglas, Inbar and Kulikov, Vladimir and Michaeli, Tomer},
  journal={arXiv},
  year={2023}
}




@article{zhang2022unsupervised,
  title={Unsupervised representation learning from pre-trained diffusion probabilistic models},
  author={Zhang, Zijian and Zhao, Zhou and Lin, Zhijie},
  journal=NeurIPS,
  year={2022}
}

@article{hspace_kwon2022diffusion,
  title={Diffusion models already have a semantic latent space},
  author={Kwon, Mingi and Jeong, Jaeseok and Uh, Youngjung},
  journal=ICLR,
  year={2023}
}


@article{haas2023discovering,
  title={Discovering Interpretable Directions in the Semantic Latent Space of Diffusion Models},
  author={Haas, Ren{\'e} and Huberman-Spiegelglas, Inbar and Mulayoff, Rotem and Michaeli, Tomer},
  journal={arXiv},
  year={2023}
}


@article{lipman2022flow,
  title={Flow matching for generative modeling},
  author={Lipman, Yaron and Chen, Ricky TQ and Ben-Hamu, Heli and Nickel, Maximilian and Le, Matt},
  journal={ICLR},
  year={2023}
}



@article{ma2023diffusionseg,
  title={DiffusionSeg: Adapting Diffusion Towards Unsupervised Object Discovery},
  author={Ma, Chaofan and Yang, Yuhuan and Ju, Chen and Zhang, Fei and Liu, Jinxiang and Wang, Yu and Zhang, Ya and Wang, Yanfeng},
  journal={arXiv preprint arXiv:2303.09813},
  year={2023}
}

@article{park2023unsupervised,
  title={Unsupervised Discovery of Semantic Latent Directions in Diffusion Models},
  author={Park, Yong-Hyun and Kwon, Mingi and Jo, Junghyo and Uh, Youngjung},
  journal={arXiv},
  year={2023}
}

@article{salimans2022progressive,
  title={Progressive distillation for fast sampling of diffusion models},
  author={Salimans, Tim and Ho, Jonathan},
  journal={arXiv},
  year={2022}
}





















@inproceedings{zhang2021deep,
  title={Deep long-tailed learning: A survey},
  author={Zhang, Yifan and Kang, Bingyi and Hooi, Bryan and Yan, Shuicheng and Feng, Jiashi},
  booktitle={ARXIV},
  year={2021}
}

@inproceedings{alexandridis2022long,
  title={Long-tailed Instance Segmentation using Gumbel Optimized Loss},
  author={Alexandridis, Konstantinos Panagiotis and Deng, Jiankang and Nguyen, Anh and Luo, Shan},
  booktitle=ECCV,
  year={2022},
}

@inproceedings{li2022equalized,
  title={Equalized focal loss for dense long-tailed object detection},
  author={Li, Bo and Yao, Yongqiang and Tan, Jingru and Zhang, Gang and Yu, Fengwei and Lu, Jianwei and Luo, Ye},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{duarte2022sign,
  title={Sign language video retrieval with free-form textual queries},
  author={Duarte, Amanda and Albanie, Samuel and Gir{\'o}-i-Nieto, Xavier and Varol, G{\"u}l},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{wang2022multi,
  title={Multi-query video retrieval},
  author={Wang, Zeyu and Wu, Yu and Narasimhan, Karthik and Russakovsky, Olga},
  booktitle={ECCV},
  year={2022},
}



@inproceedings{zhu2022balanced,
  title={Balanced contrastive learning for long-tailed visual recognition},
  author={Zhu, Jianggang and Wang, Zheng and Chen, Jingjing and Chen, Yi-Ping Phoebe and Jiang, Yu-Gang},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{xian2017zero,
  title={Zero-shot learning-the good, the bad and the ugly},
  author={Xian, Yongqin and Schiele, Bernt and Akata, Zeynep},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{chua2021fine,
  title={How fine-tuning allows for effective meta-learning},
  author={Chua, Kurtland and Lei, Qi and Lee, Jason D},
  booktitle={NeurIPS},
  year={2021}
}

@inproceedings{dubey2022vision,
  title={Vision transformer hashing for image retrieval},
  author={Dubey, Shiv Ram and Singh, Satish Kumar and Chu, Wei-Ta},
  booktitle={ICME},
  year={2022},
}



@inproceedings{xiong2012coaction,
  title={Coaction discovery: segmentation of common actions across multiple videos},
  author={Xiong, Caiming and Corso, Jason J},
  booktitle={Proceedings of the Twelfth International Workshop on Multimedia Data Mining},
  year={2012},
}

@InProceedings{hoai12,
  title = 	 {Maximum Margin Temporal Clustering},
  author = 	 {Minh Hoai and Fernando De La Torre},
  booktitle = 	 {Proceedings of the Fifteenth International Conference on Artificial Intelligence and Statistics},
  year = 	 {2012},
}

@inproceedings{liu2013video,
  title={Video event recognition using concept attributes},
  author={Liu, Jingen and Yu, Qian and Javed, Omar and Ali, Saad and Tamrakar, Amir and Divakaran, Ajay and Cheng, Hui and Sawhney, Harpreet},
  booktitle={WACV Workshop},
  year={2013},
}



@inproceedings{BuloNK17,
  author    = {Samuel Rota Bul{\`{o}} and
               Gerhard Neuhold and
               Peter Kontschieder},
  title     = {Loss Max-Pooling for Semantic Image Segmentation},
  booktitle   = {CoRR},
  year      = {2017}
}


@inproceedings{bulat2021improving,
  title={Improving memory banks for unsupervised learning with large mini-batch, consistency and hard negative mining},
  author={Bulat, Adrian and S{\'a}nchez-Lozano, Enrique and Tzimiropoulos, Georgios},
  booktitle={ICASSP},
  year={2021},
}

@inproceedings{2022_centerclip,
  author    = {Shuai Zhao and Linchao Zhu and Xiaohan Wang and Yi Yang},
  title     = {CenterCLIP: Token Clustering for Efficient Text-Video Retrieval},
  booktitle = {SIGIR},
  year      = {2022},
}

@inproceedings{arnab2021vivit,
  title={Vivit: A video vision transformer},
  author={Arnab, Anurag and Dehghani, Mostafa and Heigold, Georg and Sun, Chen and Lu{\v{c}}i{\'c}, Mario and Schmid, Cordelia},
  booktitle=ICCV,
  year={2021}
}



@inproceedings{douze2016circulant,
  title={Circulant temporal encoding for video retrieval and temporal alignment},
  author={Douze, Matthijs and Revaud, J{\'e}r{\^o}me and Verbeek, Jakob and J{\'e}gou, Herv{\'e} and Schmid, Cordelia},
  booktitle={IJCV},
  year={2016}
}


@inproceedings{mettes2019hyperspherical,
    title={Hyperspherical Prototype Networks},
    author={Pascal Mettes and Elise van der Pol and Cees G. M. Snoek},
    booktitle={ARXIV},
    year={2019}
}


@inproceedings{zhu2018compound,
  title={Compound memory networks for few-shot video classification},
  author={Zhu, Linchao and Yang, Yi},
  booktitle=ECCV,
  year={2018}
}

























@inproceedings{wang2020devil,
  title={The devil is in classification: A simple framework for long-tail instance segmentation},
  author={Wang, Tao and Li, Yu and Kang, Bingyi and Li, Junnan and Liew, Junhao and Tang, Sheng and Hoi, Steven and Feng, Jiashi},
  booktitle={ECCV},
  year={2020},
}

@inproceedings{pass_yuki,
  title={Pass: An imagenet replacement for self-supervised pretraining without humans},
  author={Asano, Yuki M and Rupprecht, Christian and Zisserman, Andrew and Vedaldi, Andrea},
  booktitle={NeurIPS},
  year={2021}
}

@inproceedings{longtail_survey,
  title={A survey on long-tailed visual recognition},
  author={Yang, Lu and Jiang, He and Song, Qing and Guo, Jun},
  booktitle={IJCV},
  year={2022},
}

@inproceedings{tian2020contrastive,
  title={Contrastive multiview coding},
  author={Tian et al.},
  booktitle={ECCV},
  year={2020},
}

@inproceedings{kasarla2022maximum,
  title={Maximum class separation as inductive bias in one matrix},
  author={Kasarla, Tejaswi and Burghouts, Gertjan J and van Spengler, Max and van der Pol, Elise and Cucchiara, Rita and Mettes, Pascal},
  booktitle={NeurIPS},
  year={2022}
}

@inproceedings{cao2020few,
  title={Few-shot video classification via temporal alignment},
  author={Cao, Kaidi and Ji, Jingwei and Cao, Zhangjie and Chang, Chien-Yi and Niebles, Juan Carlos},
  booktitle={CVPR},
  year={2020}
}

@inproceedings{hu2022sqn,
  title={Sqn: Weakly-supervised semantic segmentation of large-scale 3d point clouds},
  author={Hu, Qingyong and Yang, Bo and Fang, Guangchi and Guo, Yulan and Leonardis, Ale{\v{s}} and Trigoni, Niki and Markham, Andrew},
  booktitle={ECCV},
  year={2022},
}

@inproceedings{scharstein2014high,
  title={High-resolution stereo datasets with subpixel-accurate ground truth},
  author={Scharstein, Daniel and Hirschm{\"u}ller, Heiko and Kitajima, York and Krathwohl, Greg and Ne{\v{s}}i{\'c}, Nera and Wang, Xi and Westling, Porter},
  booktitle={Pattern Recognition: 36th German Conference, GCPR 2014, M{\"u}nster, Germany, September 2-5, 2014, Proceedings 36},
  pages={31--42},
  year={2014},
  organization={Springer}
}


@inproceedings{behley2019semantickitti,
  title={Semantickitti: A dataset for semantic scene understanding of lidar sequences},
  author={Behley, Jens and Garbade, Martin and Milioto, Andres and Quenzel, Jan and Behnke, Sven and Stachniss, Cyrill and Gall, Jurgen},
  booktitle={ICCV},
  year={2019}
}

@inproceedings{du2021save,
  title={How to Save your Annotation Cost for Panoptic Segmentation?},
  author={Du, Xuefeng and Jiang, ChenHan and Xu, Hang and Zhang, Gengwei and Li, Zhenguo},
  booktitle={AAAI},
  year={2021}
}

@inproceedings{cocostuff,
  title={Coco-stuff: Thing and stuff classes in context},
  author={Caesar, Holger and Uijlings, Jasper and Ferrari, Vittorio},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{gandissection,
  title={Gan dissection: Visualizing and understanding generative adversarial networks},
  author={Bau, David and Zhu, Jun-Yan and Strobelt, Hendrik and Zhou, Bolei and Tenenbaum, Joshua B and Freeman, William T and Torralba, Antonio},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{cam,
  title={Learning deep features for discriminative localization},
  author={Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
  booktitle={CVPR},
  year={2016}
}

@inproceedings{chen2020crowd,
  title={Crowd counting with crowd attention convolutional neural network},
  author={Chen, Jiwei and Su, Wen and Wang, Zengfu},
  booktitle={NeuroComputing},
  year={2020},
}

@inproceedings{holder2022efficient,
  title={On efficient real-time semantic segmentation: a survey},
  author={Holder, Christopher J and Shafique, Muhammad},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{jia2022stcm,
  title={STCM-Net: A symmetrical one-stage network for temporal language localization in videos},
  author={Jia, Zixi and Dong, Minglin and Ru, Jingyu and Xue, Lele and Yang, Sikai and Li, Chunbo},
  booktitle={Neurocomputing},
  year={2022},
}

@inproceedings{yang2022tubedetr,
  title={Tubedetr: Spatio-temporal video grounding with transformers},
  author={Yang, Antoine and Miech, Antoine and Sivic, Josef and Laptev, Ivan and Schmid, Cordelia},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{zhao2023segtad,
  title={Segtad: Precise temporal action detection via semantic segmentation},
  author={Zhao, Chen and Ramazanova, Merey and Xu, Mengmeng and Ghanem, Bernard},
  booktitle=ECCVW,
  year={2022},
}

@inproceedings{xiao2021boundary,
  title={Boundary proposal network for two-stage natural language video localization},
  author={Xiao, Shaoning and Chen, Long and Zhang, Songyang and Ji, Wei and Shao, Jian and Ye, Lu and Xiao, Jun},
  booktitle={AAAI},
  year={2021}
}

@inproceedings{xie2020polarmask,
  title={Polarmask: Single shot instance segmentation with polar representation},
  author={Xie, Enze and Sun, Peize and Song, Xiaoge and Wang, Wenhai and Liu, Xuebo and Liang, Ding and Shen, Chunhua and Luo, Ping},
  booktitle={CVPR},
  year={2020}
}

@inproceedings{minaee2021image,
  title={Image segmentation using deep learning: A survey},
  author={Minaee, Shervin and Boykov, Yuri Y and Porikli, Fatih and Plaza, Antonio J and Kehtarnavaz, Nasser and Terzopoulos, Demetri},
  booktitle={PAMI},
  year={2021},
}

@article{albergo2022building,
  title={Building normalizing flows with stochastic interpolants},
  author={Albergo, Michael S and Vanden-Eijnden, Eric},
  journal={arXiv preprint arXiv:2209.15571},
  year={2022}
}


@inproceedings{hulfm,
  title = {Latent Space Editing in Transformer-based Flow Matching},
  author = {Hu, Vincent Tao and Zhang, David W and Mettes, Pascal and Tang, Meng and Zhao, Deli and Snoek, Cees G.M.},
  year = {2024},
  booktitle = {AAAI},
}

@inproceedings{qiao2021detectors,
  title={Detectors: Detecting objects with recursive feature pyramid and switchable atrous convolution},
  author={Qiao, Siyuan and Chen, Liang-Chieh and Yuille, Alan},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{mettes2019pointly,
  title={Pointly-supervised action localization},
  author={Mettes, Pascal and Snoek, Cees G. M. },
  booktitle={IJCV},
  year={2019},
}
@inproceedings{joint_multimodal_generative,
  title={Joint multimodal learning with deep generative models},
  author={Suzuki, Masahiro and Nakayama, Kotaro and Matsuo, Yutaka},
  booktitle=ICLR,
  year={2016}
}

@article{ho2022cascaded,
  title={Cascaded diffusion models for high fidelity image generation},
  author={Ho, Jonathan and Saharia, Chitwan and Chan, William and Fleet, David J and Norouzi, Mohammad and Salimans, Tim},
  journal={JMLR},
  year={2022}
}

@inproceedings{foundationmodels,
  title={On the opportunities and risks of foundation models},
  author={Bommasani, Rishi and Hudson, Drew A and Adeli, Ehsan and Altman, Russ and Arora, Simran and von Arx, Sydney and Bernstein, Michael S and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and others},
  booktitle={ARXIV},
  year={2021}
}

@inproceedings{llm,
  title={Talking About Large Language Models},
  author={Shanahan, Murray},
  booktitle={ARXIV},
  year={2022}
}


@book{lao1997tao,
  title={Tao te ching},
  author={Lao Tzu, Li Er},
  year={1997},
  publisher={Wordsworth}
}



@inproceedings{suzuki2017overview,
  title={Overview of deep learning in medical imaging},
  author={Suzuki, Kenji},
  booktitle={Radiological Physics and Technology},
  year={2017},
}

@inproceedings{sultani2018real,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{igashov2022equivariant,
  title={Equivariant 3d-conditional diffusion models for molecular linker design},
  author={Igashov, Ilia and St{\"a}rk, Hannes and Vignac, Cl{\'e}ment and Satorras, Victor Garcia and Frossard, Pascal and Welling, Max and Bronstein, Michael and Correia, Bruno},
  booktitle={ARXIV},
  year={2022}
}

@book{kreiman2021biological,
  title={Biological and Computer Vision},
  author={Kreiman, Gabriel},
  year={2021},
  publisher={Cambridge University Press}
}

@inproceedings{alabdulmohsin2022revisiting,
  title={Revisiting neural scaling laws in language and vision},
  author={Alabdulmohsin, Ibrahim and Neyshabur, Behnam and Zhai, Xiaohua},
  booktitle={ARXIV},
  year={2022}
}

@book{molnar2020interpretable,
  title={Interpretable machine learning},
  author={Molnar, Christoph},
  year={2020},
  publisher={Lulu. com}
}

@inproceedings{toering2022self,
  title={Self-supervised video representation learning with cross-stream prototypical contrasting},
  author={Toering, Martine and Gatopoulos, Ioannis and Stol, Maarten and Hu, Vincent Tao},
  booktitle={WACV},
  year={2022}
}

@inproceedings{chen2020interactivity,
  title={Interactivity proposals for surveillance videos},
  author={Chen, Shuo and Mettes, Pascal and Hu, Tao and Snoek, Cees G. M. },
  booktitle={ICMR},
  year={2020}
}

@inproceedings{zhang2019accelerating,
  title={Accelerating Convolutional Neural Networks with Dynamic Channel Pruning.},
  author={Zhang, Chiliang and Hu, Tao and Guan, Yingda and Ye, Zuochang},
  booktitle={DCC},
  year={2019}
}



@inproceedings{hu2019dense,
  title={Dense In Dense: Training Segmentation from Scratch},
  author={Hu, Tao},
  booktitle={ACCV},
  year={2019}
}

@inproceedings{couairon2022diffedit,
  title={Diffedit: Diffusion-based semantic image editing with mask guidance},
  author={Couairon, Guillaume and Verbeek, Jakob and Schwenk, Holger and Cord, Matthieu},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{wirth2019pointatme,
  title={Pointatme: efficient 3d point cloud labeling in virtual reality},
  author={Wirth, Florian and Quehl, Jannik and Ota, Jeffrey and Stiller, Christoph},
  booktitle={IEEE Intelligent Vehicles Symposium},
  year={2019},
}

@inproceedings{yoon2022selective,
  title={Selective Query-Guided Debiasing for Video Corpus Moment Retrieval},
  author={Yoon, Sunjae and Hong, Ji Woo and Yoon, Eunseop and Kim, Dahyun and Kim, Junyeong and Yoon, Hee Suk and Yoo, Chang D},
  booktitle={ECCV},
  year={2022},
}

@inproceedings{zhang2021videolt,
  title={VideoLT: large-scale long-tailed video recognition},
  author={Zhang, Xing and Wu, Zuxuan and Weng, Zejia and Fu, Huazhu and Chen, Jingjing and Jiang, Yu-Gang and Davis, Larry S},
  booktitle={ICCV},
  year={2021}
}

@inproceedings{kuznetsova2021efficient,
  title={Efficient video annotation with visual interpolation and frame selection guidance},
  author={Kuznetsova, Alina and Talati, Aakrati and Luo, Yiwen and Simmons, Keith and Ferrari, Vittorio},
  booktitle={WACV},
  year={2021}
}


@inproceedings{tang2018regularized,
  title={On regularized losses for weakly-supervised cnn segmentation},
  author={Tang, Meng and Perazzi, Federico and Djelouah, Abdelaziz and Ben Ayed, Ismail and Schroers, Christopher and Boykov, Yuri},
  booktitle=ECCV,
  year={2018}
}

@inproceedings{maggiori2017can,
  title={Can semantic labeling methods generalize to any city? the inria aerial image labeling benchmark},
  author={Maggiori, Emmanuel and Tarabalka, Yuliya and Charpiat, Guillaume and Alliez, Pierre},
  booktitle={IEEE International Geoscience and Remote Sensing Symposium},
  year={2017}
}

@inproceedings{tao2018shk,
  title={Sobel Heuristic Kernel for aerial semantic segmentation},
  author={Tao Hu and Yao Wang and Peng Lu and Heng Wang},
  booktitle={ICIP},
  year={2018}
}

@inproceedings{karlinsky2019repmet,
  title={{RepMet}: Representative-based metric learning for classification and few-shot object detection},
  author={Karlinsky, Leonid and Shtok, Joseph and Harary, Sivan and Schwartz, Eli and Aides, Amit and Feris, Rogerio and Giryes, Raja and Bronstein, Alex M},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{kang2018few,
  title={Few-shot Object Detection via Feature Reweighting},
  author={Kang, Bingyi and Liu, Zhuang and Wang, Xin and Yu, Fisher and Feng, Jiashi and Darrell, Trevor},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{rakelly2018few,
  title={Few-shot segmentation propagation with guided networks},
  author={Rakelly, Kate and Shelhamer, Evan and Darrell, Trevor and Efros, Alexei A. and Levine, Sergey},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{michaelis2018,
    title = {One-Shot Instance Segmentation},
    author = {Michaelis, Claudio and Ustyuzhaninov, Ivan and Bethge, Matthias and Ecker, Alexander S.},
    year = {2018},
    booktitle = {ARXIV},
}

@inproceedings{michaelis2018one,
  title={One-shot segmentation in clutter},
  author={Michaelis, Claudio and Bethge, Matthias and Ecker, Alexander S.},
  booktitle=ICML,
  year={2018}
}
@inproceedings{carbonneau2018multiple,
	title={Multiple instance learning: A survey of problem characteristics and applications},
	author={Carbonneau, Marc-Andr{\'e} and Cheplygina, Veronika and Granger, Eric and Gagnon, Ghyslain},
	booktitle={Pattern Recognition},
	year={2018},
	publisher={Elsevier}
}
@inproceedings{xian2019f,
	title={{f-VAEGAN-D2}: A feature generating framework for any-shot learning},
	author={Xian, Yongqin and Sharma, Saurabh and Schiele, Bernt and Akata, Zeynep},
	booktitle=CVPR,
	year={2019}
}
@inproceedings{xian2019semantic,
	title={Semantic Projection Network for Zero-and Few-Label Semantic Segmentation},
	author={Xian, Yongqin and Choudhury, Subhabrata and He, Yang and Schiele, Bernt and Akata, Zeynep},
	booktitle=CVPR,
	year={2019}
}

@inproceedings{hadsell2006dimensionality,
  title={Dimensionality reduction by learning an invariant mapping},
  author={Hadsell, Raia and Chopra, Sumit and LeCun, Yann},
  booktitle={CVPR},
  year={2006},
}

@inproceedings{li2016weakly,
  title={Weakly supervised object localization with progressive domain adaptation},
  author={Li, Dong and Huang, Jia-Bin and Li, Yali and Wang, Shengjin and Yang, Ming-Hsuan},
  booktitle=CVPR,
  year={2016}
}

@inproceedings{ravi2016optimization,
	title={Optimization as a Model for Few-Shot Learning},
	author={Ravi, Sachin and Larochelle, Hugo},
	booktitle=ICLR,
	year={2017}
}

@misc{tensorpack,
	title={Tensorpack},
	author={Wu, Yuxin and others},
	howpublished={\url{https://github.com/tensorpack/}},
	year={2016}
}

@inproceedings{layernorm,
	title={Layer normalization},
	author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
	booktitle={ARXIV},
	year={2016}
}

@inproceedings{peephole,
	title={Learning Precise Timing with LSTM Recurrent Networks},
	author={Gers, Felix A and Schraudolph, Nicol N and Schmidhuber, J{\"u}rgen},
	booktitle=JMLR,
	year={2002}
}

@inproceedings{lstm,
	title={Long Short-Term Memory},
	author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
	booktitle=NC,
	year={1997},	
}

@inproceedings{deepsteer,
	title={Deep Steering: Learning End-to-End Driving Model from Spatial and Temporal Visual Cues},
	author={Chi, Lu and Mu, Yadong},
	booktitle={ARXIV preprint ARXIV:1708.03798},
	year={2017}
}

@inproceedings{convLSTM,
	title={Convolutional LSTM network: A machine learning approach for precipitation nowcasting},
	author={Xingjian, SHI and Chen, Zhourong and Wang, Hao and Yeung, Dit-Yan and Wong, Wai-Kin and Woo, Wang-chun},
	booktitle=NeurIPS,
	year={2015}
}

@inproceedings{relu,
	title={Rectified Linear Units Improve Restricted Boltzmann Machines},
	author={Nair, Vinod and Hinton, Geoffrey E},
	booktitle=ICML,
	year={2010}
}

@inproceedings{senet,
	title={Squeeze-and-Excitation Networks},
	author={Hu, Jie and Shen, Li and Sun, Gang},
	booktitle=CVPR,
	year={2018}
}



@inproceedings{caelles2017one,
	author = {S. Caelles and K.-K. Maninis and J. Pont-Tuset and L. Leal-Taix\'e and D. Cremers and L. {Van Gool}},
	title = {One-Shot Video Object Segmentation},
	booktitle =CVPR,
	year = {2017}
}

@inproceedings{hourglass,
	title={Stacked Hourglass Networks for Human Pose Estimation},
	author={Newell, Alejandro and Yang, Kaiyu and Deng, Jia},
	booktitle=ECCV,
	year={2016},
}



@inproceedings{sds,
	title={Simultaneous Detection and Segmentation},
	author={Hariharan, Bharath and Arbel{\'a}ez, Pablo and Girshick, Ross and Malik, Jitendra},
	booktitle=ECCV,
	year={2014},
}

@inproceedings{pascalvoc,
	title={The Pascal Visual Object Classes ({VOC}) Challenge},
	author={Everingham, Mark and Van Gool, Luc and Williams, Christopher K. I. and Winn, John and Zisserman, Andrew},
	booktitle=IJCV,
	year={2010},
}

@inproceedings{vgg,
	title={Very Deep Convolutional Networks for Large-Scale Image Recognition},
	author={Karen Simonyan and Andrew Zisserman},
	booktitle={NeurIPS},
	year={2014}
}

@inproceedings{resnet,
	title={Deep Residual Learning for Image Recognition},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=CVPR,
	year={2016}
}

@inproceedings{sgd,
	title={Large-scale machine learning with stochastic gradient descent},
	author={Bottou, L{\'e}on},
	booktitle={COMPSTAT},
	year={2010},
}

@inproceedings{bn,
	title={Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
	author={Sergey Ioffe and Christian Szegedy},
	booktitle=ICML,
	year={2015}
}





@inproceedings{wang2017residual,
	title={Residual Attention Network for Image Classification},
	author={Wang, Fei and Jiang, Mengqing and Qian, Chen and Yang, Shuo and Li, Cheng and Zhang, Honggang and Wang, Xiaogang and Tang, Xiaoou},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{shaban2017one,
  title={One-Shot Learning for Semantic Segmentation},
  author={Shaban, Amirreza and Bansal, Shray and Liu, Zhen and Essa, Irfan and Boots, Byron},
  booktitle=BMVC,
  year={2017}
}


@inproceedings{rakelly2018conditional,
	title={Conditional Networks for Few-Shot Semantic Segmentation},
	author={Rakelly, Kate and Shelhamer, Evan and Darrell, Trevor and Efros, Alyosha and Levine, Sergey},
	booktitle=ICLRW,
	year={2018}
}

@inproceedings{srivastava2014dropout,
	title={Dropout: A simple way to prevent neural networks from overfitting},
	author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
	booktitle=JMLR,
	year={2014},
}

@inproceedings{zink2018automated,
	title={Automated dataset generation for image recognition using the example of taxonomy},
	author={Zink, Jaro Milan},
	booktitle={ARXIV preprint ARXIV:1802.02207},
	year={2018}
}

@inproceedings{han2016dsd,
	title={Dsd: Regularizing deep neural networks with dense-sparse-dense training flow},
	author={Han, Song and Pool, Jeff and Narang, Sharan and Mao, Huizi and Tang, Shijian and Elsen, Erich and Catanzaro, Bryan and Tran, John and Dally, William J},
	booktitle={ARXIV preprint ARXIV:1607.04381},
	year={2016}
}

@inproceedings{han2015deep,
	title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
	author={Han, Song and Mao, Huizi and Dally, William J},
	booktitle={ARXIV preprint ARXIV:1510.00149},
	year={2015}
}

@inproceedings{he2016identity,
	title={Identity mappings in deep residual networks},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=ECCV,
	year={2016},
}

@inproceedings{visin2016reseg,
	title={Reseg: A recurrent neural network-based model for semantic segmentation},
	booktitle=CVPRW,
	year={2016},
	author={Visin, Francesco and Romero, Adriana and Cho, Kyunghyun and Matteucci, Matteo and Ciccone, Marco and Kastner, Kyle and Bengio, Yoshua and Courville, Aaron},
}

@inproceedings{deconvnet,
	title={Learning deconvolution network for semantic segmentation},
	author={Noh, Hyeonwoo and Hong, Seunghoon and Han, Bohyung},
	booktitle=ICCV,
	year={2015}
}

@inproceedings{hed,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle=ICCV,
	year={2015}
}

@inproceedings{shen2017dsod,
	title={Dsod: Learning deeply supervised object detectors from scratch},
	author={Shen, Zhiqiang and Liu, Zhuang and Li, Jianguo and Jiang, Yu-Gang and Chen, Yurong and Xue, Xiangyang},
	booktitle=ICCV,
	year={2017}
}


@inproceedings{wang2017understanding,
	title={Understanding convolution for semantic segmentation},
	author={Wang, Panqu and Chen, Pengfei and Yuan, Ye and Liu, Ding and Huang, Zehua and Hou, Xiaodi and Cottrell, Garrison},
	booktitle=WACV,
	year={2018}
}

@inproceedings{maggiori2017dataset,
	title={Can Semantic Labeling Methods Generalize to Any City? The Inria Aerial Image Labeling Benchmark},
	author={Maggiori, Emmanuel and Tarabalka, Yuliya and Charpiat, Guillaume and Alliez, Pierre},
	booktitle={IEEE International Geoscience and Remote Sensing Symposium (IGARSS)},
	year={2017},
}


@inproceedings{chen2017rethinking,
	title={Rethinking atrous convolution for semantic image segmentation},
	author={Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig},
	booktitle={ARXIV preprint ARXIV:1706.05587},
	year={2017}
}

@inproceedings{chen2020pointmixup,
  title={Pointmixup: Augmentation for point clouds},
  author={Chen, Yunlu and Hu, Vincent Tao and Gavves, Efstratios and Mensink, Thomas and Mettes, Pascal and Yang, Pengwan and Snoek, Cees G. M. },
  booktitle={ECCV},
  year={2020},
}

@inproceedings{sgdm,
          title={Self-Guided Diffusion Models},
          author={Vincent Tao Hu and David W Zhang and Yuki M. Asano and Gertjan J. Burghouts and Cees G. M. Snoek},
           booktitle={CVPR},
          year={2023},
      }
      

@inproceedings{glorot2010understanding,
	title={Understanding the difficulty of training deep feedforward neural networks},
	author={Glorot, Xavier and Bengio, Yoshua},
	booktitle={AISTATS},
	year={2010}
}

@inproceedings{kingma2014adam,
	title={Adam: A method for stochastic optimization},
	author={Kingma, Diederik P and Ba, Jimmy},
	booktitle={AISTATS},
	year={2016}
}

@inproceedings{abadi2016tensorflow,
	title={TensorFlow: A System for Large-Scale Machine Learning.},
	author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
	booktitle={OSDI},
	year={2016}
}

@inproceedings{jegou2017one,
	title={The one hundred layers tiramisu: Fully convolutional densenets for semantic segmentation},
	author={J{\'e}gou, Simon and Drozdzal, Michal and Vazquez, David and Romero, Adriana and Bengio, Yoshua},
	booktitle={CVPR Workshop},
	year={2017}
}

@inproceedings{liu2017learning,
	title={Learning affinity via spatial propagation networks},
	author={Liu, Sifei and De Mello, Shalini and Gu, Jinwei and Zhong, Guangyu and Yang, Ming-Hsuan and Kautz, Jan},
	booktitle={NeurIPS}},
	year={2017}
}

@inproceedings{zheng2015conditional,
	title={Conditional random fields as recurrent neural networks},
	author={Zheng, Shuai and Jayasumana, Sadeep and Romera-Paredes, Bernardino and Vineet, Vibhav and Su, Zhizhong and Du, Dalong and Huang, Chang and Torr, Philip H. S.},
	booktitle={CVPR},
	year={2015}
}

@inproceedings{pspnet,
	title={Pyramid scene parsing network},
	author={Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{unet,
	title={U-net: Convolutional networks for biomedical image segmentation},
	author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
	booktitle={MICCAI},
	year={2015},
}

@inproceedings{badrinarayanan2017segnet,
	title={SegNet: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle=PAMI,
	year={2017},
}

@inproceedings{szegedy2015going,
	title={Going Deeper with Convolutions},
	author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew and others},
	year={2015},
	booktitle=CVPR
}

@inproceedings{xie2015holistically,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle={Proceedings of the IEEE international conference on computer vision},
	pages={1395--1403},
	year={2015}
}

@inproceedings{oquab2014learning,
	title={Learning and transferring mid-level image representations using convolutional neural networks},
	author={Oquab, Maxime and Bottou, Leon and Laptev, Ivan and Sivic, Josef},
	booktitle={Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on},
	pages={1717--1724},
	year={2014},
	organization={IEEE}
}

@inproceedings{zagoruyko2016wide,
	title={Wide residual networks},
	author={Zagoruyko, Sergey and Komodakis, Nikos},
	booktitle={ARXIV preprint ARXIV:1605.07146},
	year={2016}
}

@inproceedings{krahenbuhl2011efficient,
	title={Efficient inference in fully connected crfs with gaussian edge potentials},
	author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
	booktitle=NeurIPS,
	year={2011}
}


@inproceedings{chen2018deeplab,
	title={DeepLab: Semantic Image Segmentation with Deep Convolutional Nets, Atrous Convolution, and Fully Connected CRFs},
	author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L},
	booktitle=PAMI,
	year={2018},
}


@inproceedings{imagenet,
	title={{ImageNet}: A large-scale hierarchical image database},
	author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
	booktitle=CVPR,
	year={2009},
}

@inproceedings{huang2017densely,
	title={Densely connected convolutional networks},
	author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
	booktitle=CVPR,
	year={2017}
}



@inproceedings{yu2015multi,
	title={Multi-Scale Context Aggregation by Dilated Convolutions},
	author={Yu, Fisher and Koltun, Vladlen},
	booktitle=ICLR,
	year={2016}
}
@inproceedings{krizhevsky2012imagenet,
	title={Imagenet classification with deep convolutional neural networks},
	author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
	booktitle=NeurIPS,
	year={2012}
}
@inproceedings{girshick15fastrcnn,
	Author = {Ross Girshick},
	Title = {Fast {R-CNN}},
	Booktitle =ICCV,
	Year = {2015}
}
@inproceedings{girshick2015fast,
	title={Fast r-cnn},
	author={Girshick, Ross},
	booktitle=ICCV,
	year={2015}
}


@inproceedings{chen2020simple_simclr,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@misc{Authors14b,
	author = {Authors},
	title = {Frobnication tutorial},
	note = {Supplied as additional material {\tt tr.pdf}},
	year = 2014
}

@inproceedings{Alpher02,
	author = {A. Alpher},
	title = {Frobnication},
	booktitle = {booktitle of Foo},
	volume = 12,
	number = 1,
	pages = {234--778},
	year = 2002
}

@inproceedings{Alpher03,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe},
	title = {Frobnication revisited},
	booktitle = {booktitle of Foo},
	volume = 13,
	number = 1,
	pages = {234--778},
	year = 2003
}

@inproceedings{Alpher04,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe and G. Gamow},
	title = {Can a machine frobnicate?},
	booktitle = {booktitle of Foo},
	volume = 14,
	number = 1,
	pages = {234--778},
	year = 2004
}

@inproceedings{segnet,
	title={SegNet: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle=PAMI,
	year={2017}
}

@inproceedings{sbd,
	title={Semantic Contours from Inverse Detectors},
	author={Hariharan, Bharath and Arbel{\'a}ez, Pablo and Bourdev, Lubomir and Maji, Subhransu and Malik, Jitendra},
	booktitle=ICCV,
	year={2011}
}


@inproceedings{aljundi2016expert,
	title={Expert Gate: Lifelong Learning with a Network of Experts},
	author={Aljundi, Rahaf and Chakravarty, Punarjay and Tuytelaars, Tinne},
	booktitle=ARXIV,
	year={2016}
}

@inproceedings{rannen2017encoder,
	title={Encoder based lifelong learning},
	author={Rannen Ep Triki, Amal and Aljundi, Rahaf and Blaschko, Matthew and Tuytelaars, Tinne},
	booktitle=ICCV,
	year={2017}
}
@inproceedings{catastrophic,
	title={Catastrophic forgetting in connectionist networks},
	author={French, Robert M},
	booktitle={Trends in cognitive sciences},
	year={1999},
}

@inproceedings{lwf,
	title={Learning without forgetting},
	author={Li, Zhizhong and Hoiem, Derek},
	booktitle=PAMI,
	year={2017}
}

@inproceedings{ewc,
	title={Overcoming catastrophic forgetting in neural networks},
	author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
	booktitle={Proceedings of the National Academy of Sciences},
	volume={114},
	number={13},
	pages={3521--3526},
	year={2017},
	publisher={National Acad Sciences}
}

@inproceedings{incremental-detector,
	title={Incremental Learning of Object Detectors without Catastrophic Forgetting},
	author={Shmelkov, Konstantin and Schmid, Cordelia and Alahari, Karteek},
	booktitle=ICCV,
	year={2017}
}

@inproceedings{ewc-moment,
	title={Overcoming catastrophic forgetting by incremental moment matching},
	author={Lee, Sang-Woo and Kim, Jin-Hwa and Jun, Jaehyun and Ha, Jung-Woo and Zhang, Byoung-Tak},
	booktitle={Advances in Neural Information Processing Systems},
	pages={4655--4665},
	year={2017}
}
@inproceedings{distilling,
	title={Distilling the knowledge in a neural network},
	author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
	booktitle=NIPS,
	year={2014}
}

@inproceedings{fcn,
	title={Fully convolutional networks for semantic segmentation},
	author={Long, Jonathan and Shelhamer, Evan and Darrell, Trevor},
	booktitle=CVPR,
	year={2015}
}

@inproceedings{coco,
	title={Microsoft COCO: Common Objects in Context},
	author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
	booktitle=ECCV,
	year={2014},
}



@inproceedings{thrun1996learning,
	title={Is learning the n-th thing any easier than learning the first?},
	author={Thrun, Sebastian},
	booktitle=NIPS,
	pages={640--646},
	year={1996}
}

@inproceedings{schlimmer1986case,
	title={A case study of incremental concept induction},
	author={Schlimmer, Jeffrey C and Fisher, Douglas},
	booktitle=AAAI,
	volume={86},
	pages={496--501},
	year={1986}
}

@inproceedings{ristin2014incremental,
	title={Incremental learning of NCM forests for large-scale image classification},
	author={Ristin, Marko and Guillaumin, Matthieu and Gall, Juergen and Van Gool, Luc},
	booktitle=CVPR,
	pages={3654--3661},
	year={2014}
}

@inproceedings{buciluǎ2006model,
	title={Model compression},
	author={Buciluǎ, Cristian and Caruana, Rich and Niculescu-Mizil, Alexandru},
	booktitle={Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={535--541},
	year={2006},
	organization={ACM}
}

@inproceedings{tzeng2015simultaneous,
	title={Simultaneous deep transfer across domains and tasks},
	author={Tzeng, Eric and Hoffman, Judy and Darrell, Trevor and Saenko, Kate},
	booktitle=ICCV,
	pages={4068--4076},
	year={2015},
	organization={IEEE}
}

@inproceedings{gupta2016cross,
	title={Cross modal distillation for supervision transfer},
	author={Gupta, Saurabh and Hoffman, Judy and Malik, Jitendra},
	booktitle=CVPR,
	pages={2827--2836},
	year={2016},
	organization={IEEE}
}

@inproceedings{goodfellow2013empirical,
	title={An empirical investigation of catastrophic forgetting in gradient-based neural networks},
	author={Goodfellow, Ian J and Mirza, Mehdi and Xiao, Da and Courville, Aaron and Bengio, Yoshua},
	booktitle={ARXIV preprint ARXIV:1312.6211},
	year={2013}
}

@inproceedings{french1994dynamically,
	title={Dynamically constraining connectionist networks to produce distributed, orthogonal representations to reduce catastrophic interference},
	author={French, Robert M},
	booktitle={network},
	volume={1111},
	pages={00001},
	year={1994},
	publisher={Citeseer}
}

@inproceedings{lecun1989backpropagation,
	title={Backpropagation applied to handwritten zip code recognition},
	author={LeCun, Yann and Boser, Bernhard and Denker, John S and Henderson, Donnie and Howard, Richard E and Hubbard, Wayne and Jackel, Lawrence D},
	booktitle={Neural computation},
	volume={1},
	number={4},
	pages={541--551},
	year={1989},
	publisher={MIT Press}
}

@inproceedings{ans2004self,
	title={Self-refreshing memory in artificial neural networks: Learning temporal sequences without catastrophic forgetting},
	author={Ans, Bernard and Rousset, St{\'e}phane and French, Robert M and Musca, Serban},
	booktitle={Connection Science},
	volume={16},
	number={2},
	pages={71--99},
	year={2004},
	publisher={Taylor \& Francis}
}


@inproceedings{torralba2011unbiased,
	title={Unbiased look at dataset bias},
	author={Torralba, Antonio and Efros, Alexei A},
	booktitle={Computer Vision and Pattern Recognition (CVPR), 2011 IEEE Conference on},
	pages={1521--1528},
	year={2011},
	organization={IEEE}
}

@inproceedings{icarl,
	title={icarl: Incremental classifier and representation learning},
	author={Rebuffi, Sylvestre-Alvise and Kolesnikov, Alexander and Sperl, Georg and Lampert, Christoph H},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{pnn,
	title={Progressive Neural Networks},
	author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
	booktitle=NIPS,
	year={2016}
}

@inproceedings{pathnet,
	title={Pathnet: Evolution channels gradient descent in super neural networks},
	author={Fernando, Chrisantha and Banarse, Dylan and Blundell, Charles and Zwols, Yori and Ha, David and Rusu, Andrei A and Pritzel, Alexander and Wierstra, Daan},
	booktitle={ARXIV preprint ARXIV:1701.08734},
	year={2017}
}

@inproceedings{road,
	title={ROAD: Reality oriented adaptation for semantic segmentation of urban scenes},
	author={Chen, Yuhua and Li, Wen and Van Gool, Luc},
	booktitle=CVPR,
	pages={7892--7901},
	year={2018}
}

@inproceedings{fcnwild,
	title={Fcns in the wild: Pixel-level adversarial and constraint-based adaptation},
	author={Hoffman, Judy and Wang, Dequan and Yu, Fisher and Darrell, Trevor},
	booktitle={ARXIV preprint ARXIV:1612.02649},
	year={2016}
}

@inproceedings{saito2017maximum,
	title={Maximum classifier discrepancy for unsupervised domain adaptation},
	author={Saito, Kuniaki and Watanabe, Kohei and Ushiku, Yoshitaka and Harada, Tatsuya},
	booktitle=CVPR,
	volume={3},
	year={2017}
}


@inproceedings{tsai2018learning,
	title={Learning to adapt structured output space for semantic segmentation},
	author={Tsai, Yi-Hsuan and Hung, Wei-Chih and Schulter, Samuel and Sohn, Kihyuk and Yang, Ming-Hsuan and Chandraker, Manmohan},
	booktitle=CVPR,
	year={2017}
}


@inproceedings{referseg,
	author = {Li, Ruiyu and Li, Kaican and Kuo, Yi-Chun and Shu, Michelle and Qi, Xiaojuan and Shen, Xiaoyong and Jia, Jiaya},
	title = {Referring Image Segmentation via Recurrent Refinement Networks},
	booktitle = CVPR,
	month = {June},
	year = {2018}
}

@inproceedings{ris,
	title={Recurrent Instance Segmentation},
	author={Romera-Paredes, Bernardino and Torr, Philip Hilaire Sean},
	booktitle=ECCV,
	pages={312--329},
	year={2016},
	organization={Springer}
}

@inproceedings{liu2018rotate,
	title={Rotate your Networks: Better Weight Consolidation and Less Catastrophic Forgetting},
	author={Liu, Xialei and Masana, Marc and Herranz, Luis and Van de Weijer, Joost and Lopez, Antonio M and Bagdanov, Andrew D},
	booktitle=ICPR,
	year={2018}
}

@inproceedings{ssd,
	title={{SSD}: Single shot multibox detector},
	author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C.},
	booktitle=ECCV,
	year={2016},
}

@inproceedings{yolo,
	title={You only look once: Unified, real-time object detection},
	author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
	booktitle=CVPR,
	year={2016}
}

@inproceedings{yolo9000,
	title={YOLO9000: better, faster, stronger},
	author={Redmon, Joseph and Farhadi, Ali},
	booktitle={ARXIV preprint},
	year={2017}
}

@inproceedings{retinanet,
	title={Focal loss for dense object detection},
	author={Lin, Tsung-Yi and Goyal, Priyal and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
	booktitle=PAMI,
	year={2018},
	publisher={IEEE}
}

@inproceedings{ionet,
	title={Inside-outside net: Detecting objects in context with skip pooling and recurrent neural networks},
	author={Bell, Sean and Lawrence Zitnick, C. and Bala, Kavita and Girshick, Ross},
	booktitle=CVPR,
	pages={2874--2883},
	year={2016}
}

@inproceedings{fasterrcnn,
	title={Faster r-cnn: Towards real-time object detection with region proposal networks},
	author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
	booktitle=NIPS,
	year={2015}
}



@inproceedings{maskrcnn,
	title={Mask r-cnn},
	author={He, Kaiming and Gkioxari, Georgia and Doll{\'a}r, Piotr and Girshick, Ross},
	booktitle={ICCV},
	year={2017},
}

@inproceedings{rcnn,
	title={Rich feature hierarchies for accurate object detection and semantic segmentation},
	author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
	booktitle={CVPR},
	year={2014}
}

@inproceedings{selectivesearch,
	title={Selective search for object recognition},
	author={Uijlings, Jasper RR and Van De Sande, Koen EA and Gevers, Theo and Smeulders, Arnold WM},
	booktitle=IJCV,
	year={2013},
}

@inproceedings{sppnet,
	title={Spatial pyramid pooling in deep convolutional networks for visual recognition},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=ECCV,
	year={2014},
}

@inproceedings{rfcn,
	title={R-fcn: Object detection via region-based fully convolutional networks},
	author={Dai, Jifeng and Li, Yi and He, Kaiming and Sun, Jian},
	booktitle=NeurIPS,
	year={2016}
}

@inproceedings{deformable,
	title={Deformable convolutional networks},
	author={Dai, Jifeng and Qi, Haozhi and Xiong, Yuwen and Li, Yi and Zhang, Guodong and Hu, Han and Wei, Yichen},
	booktitle={ARXIV},
	year={2017}
}

@inproceedings{fpn,
	title={Feature Pyramid Networks for Object Detection.},
	author={Lin, Tsung-Yi and Doll{\'a}r, Piotr and Girshick, Ross B. and He, Kaiming and Hariharan, Bharath and Belongie, Serge J.},
	booktitle={CVPR},
	year={2017}
}
@inproceedings{diba2017weakly,
	title={Weakly Supervised Cascaded Convolutional Networks.},
	author={Diba, Ali and Sharma, Vivek and Pazandeh, Ali Mohammad and Pirsiavash, Hamed and Van Gool, Luc},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{kantorov2016contextlocnet,
	title={Contextlocnet: Context-aware deep network models for weakly supervised localization},
	author={Kantorov, Vadim and Oquab, Maxime and Cho, Minsu and Laptev, Ivan},
	booktitle=ECCV,
	pages={350--365},
	year={2016},
	organization={Springer}
}

@inproceedings{bilen2016weakly,
	title={Weakly supervised deep detection networks},
	author={Bilen, Hakan and Vedaldi, Andrea},
	booktitle=CVPR,
	year={2016}
}

@inproceedings{cinbis2017weakly,
	title={Weakly supervised object localization with multi-fold multiple instance learning},
	author={Cinbis, Ramazan Gokberk and Verbeek, Jakob and Schmid, Cordelia},
	booktitle=PAMI,
	year={2017},
}

@inproceedings{bai2017multiple,
	title={Multiple instance detection network with online instance classifier refinement},
	author={Bai, Peng Tang Xinggang Wang Xiang and Liu, Wenyu},
	year={2017}
}

@inproceedings{tang2016large,
	title={Large scale semi-supervised object detection using visual and semantic knowledge transfer},
	author={Tang, Yuxing and Wang, Josiah and Gao, Boyang and Dellandr{\'e}a, Emmanuel and Gaizauskas, Robert and Chen, Liming},
	booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages={2119--2128},
	year={2016}
}

@inproceedings{kumar2016track,
	title={Track and transfer: Watching videos to simulate strong human supervision for weakly-supervised object detection},
	author={Kumar Singh, Krishna and Xiao, Fanyi and Jae Lee, Yong},
	booktitle=CVPR,
	pages={3548--3556},
	year={2016}
}

@inproceedings{dong2018fewexample,
	title   = {Few-Example Object Detection with Model Communication},
	author  = {Dong, Xuanyi and Zheng, Liang and Ma, Fan and Yang, Yi and Meng, Deyu},
	booktitle = PAMI,
	year    = {2018}
}

@inproceedings{yosinski2014transferable,
	title={How transferable are features in deep neural networks?},
	author={Yosinski, Jason and Clune, Jeff and Bengio, Yoshua and Lipson, Hod},
	booktitle=NIPS,
	pages={3320--3328},
	year={2014}
}

@inproceedings{donahue2014decaf,
	title={Decaf: A deep convolutional activation feature for generic visual recognition},
	author={Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
	booktitle={International conference on machine learning},
	pages={647--655},
	year={2014}
}

@inproceedings{liang2015towards,
	title={Towards computational baby learning: A weakly-supervised approach for object detection},
	author={Liang, Xiaodan and Liu, Si and Wei, Yunchao and Liu, Luoqi and Lin, Liang and Yan, Shuicheng},
	booktitle=CVPR,
	pages={999--1007},
	year={2015}
}

@inproceedings{bilen2015weakly,
	title={Weakly supervised object detection with convex clustering},
	author={Bilen, Hakan and Pedersoli, Marco and Tuytelaars, Tinne},
	booktitle=CVPR,
	pages={1081--1089},
	year={2015}
}


@inproceedings{li2016weakly,
	title={Weakly supervised object localization with progressive domain adaptation},
	author={Li, Dong and Huang, Jia-Bin and Li, Yali and Wang, Shengjin and Yang, Ming-Hsuan},
	booktitle=CVPR,
	pages={3512--3520},
	year={2016}
}

@inproceedings{ren2018meta,
	title={Meta-learning for semi-supervised few-shot classification},
	author={Ren, Mengye and Triantafillou, Eleni and Ravi, Sachin and Snell, Jake and Swersky, Kevin and Tenenbaum, Joshua B and Larochelle, Hugo and Zemel, Richard S},
	booktitle={ARXIV preprint ARXIV:1803.00676},
	year={2018}
}

@inproceedings{garcia2017few,
	title={Few-shot learning with graph neural networks},
	author={Garcia, Victor and Bruna, Joan},
	booktitle={ARXIV preprint ARXIV:1711.04043},
	year={2017}
}

@InProceedings{Razavian_2014_CVPR_Workshops,
	author = {Sharif Razavian, Ali and Azizpour, Hossein and Sullivan, Josephine and Carlsson, Stefan},
	title = {CNN Features Off-the-Shelf: An Astounding Baseline for Recognition},
	booktitle = CVPRW,
	year = {2014}
}

@InProceedings{yang2018learning,
	title={Learning to compare: Relation network for few-shot learning},
	author={Yang, Flood Sung Yongxin and Zhang, Li and Xiang, Tao and Torr, Philip H. S. and Hospedales, Timothy M.},
	booktitle = CVPR,
	year={2018}
}





@inproceedings{gadde2017semantic,
	title={Semantic video cnns through representation warping},
	author={Gadde, Raghudeep and Jampani, Varun and Gehler, Peter V},
	booktitle=ARXIV,
	year={2017}
}


@inproceedings{enet,
	title={ENet: A Deep Neural Network Architecture for Real-Time Semantic Segmentation},
	author={Paszke, Adam and Chaurasia, Abhishek and Kim, Sangpil and Culurciello, Eugenio},
	booktitle={ARXIV preprint ARXIV:1606.02147},
	year={2016}
}


@inproceedings{erfnet,
	title={ERFNet: Efficient Residual Factorized ConvNet for Real-Time Semantic Segmentation},
	author={Romera, Eduardo and Alvarez, Jos{\'e} M and Bergasa, Luis M and Arroyo, Roberto},
	booktitle={IEEE Transactions on Intelligent Transportation Systems},
	year={2018}
}


@inproceedings{frrn,
	title={Full-Resolution Residual Networks for Semantic Segmentation in Street Scenes},
	author={Pohlen, Tobias and Hermans, Alexander and Mathias, Markus and Leibe, Bastian},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{lrr,
	title={Laplacian pyramid reconstruction and refinement for semantic segmentation},
	author={Ghiasi, Golnaz and Fowlkes, Charless C},
	booktitle=ECCV,
	year={2016},
}

%dongzhuoyao 
@inproceedings{chen2018lstd,
	title={{LSTD}: A Low-Shot Transfer Detector for Object Detection},
	author={Chen, Hao and Wang, Yali and Wang, Guoyou and Qiao, Yu},
	booktitle=AAAI,
	year={2018}
}

@inproceedings{gori2005new,
	title={A new model for learning in graph domains},
	author={Gori, Marco and Monfardini, Gabriele and Scarselli, Franco},
	booktitle=IJCNN,
	year={2005},
}

@inproceedings{scarselli2009graph,
	title={The graph neural network model},
	author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
	booktitle={IEEE Transactions on Neural Networks},
	year={2009},
}

@inproceedings{li2015gated,
	title={Gated graph sequence neural networks},
	author={Li, Yujia and Tarlow, Daniel and Brockschmidt, Marc and Zemel, Richard},
	booktitle={ARXIV preprint ARXIV:1511.05493},
	year={2015}
}

@inproceedings{sukhbaatar2016learning,
	title={Learning multiagent communication with backpropagation},
	author={Sukhbaatar, Sainbayar and Fergus, Rob and others},
	booktitle=NIPS,
	year={2016}
}

@inproceedings{xu2015empirical,
	title={Empirical evaluation of rectified activations in convolutional network},
	author={Xu, Bing and Wang, Naiyan and Chen, Tianqi and Li, Mu},
	booktitle={ARXIV},
	year={2015}
}

@inproceedings{duvenaud2015convolutional,
	title={Convolutional networks on graphs for learning molecular fingerprints},
	author={Duvenaud, David K and Maclaurin, Dougal and Iparraguirre, Jorge and Bombarell, Rafael and Hirzel, Timothy and Aspuru-Guzik, Al{\'a}n and Adams, Ryan P},
	booktitle=NIPS,
	year={2015}
}

@inproceedings{kipf2016semi,
	title={Semi-supervised classification with graph convolutional networks},
	author={Kipf, Thomas N. and Welling, Max},
	booktitle={ARXIV},
	year={2016}
}

@inproceedings{bruna2017community,
	title={Community detection with graph neural networks},
	author={Bruna, Joan and Li, Xiang},
	booktitle={ARXIV preprint ARXIV:1705.08415},
	year={2017}
}


@inproceedings{gilmer2017neural,
	title={Neural message passing for quantum chemistry},
	author={Gilmer, Justin and Schoenholz, Samuel S. and Riley, Patrick F. and Vinyals, Oriol and Dahl, George E.},
	booktitle={ARXIV},
	year={2017}
}
@inproceedings{maml,
	title={Model-agnostic meta-learning for fast adaptation of deep networks},
	author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
	booktitle=ICML,
	year={2017}
}

@inproceedings{fewshotgnn,
	title={Few-shot learning with graph neural networks},
	author={Garcia, Victor and Bruna, Joan},
	booktitle=ICLR,
	year={2018}
}

@inproceedings{siamese,
	title={Siamese neural networks for one-shot image recognition},
	author={Koch, Gregory and Zemel, Richard and Salakhutdinov, Ruslan},
	booktitle=ICMLW,
	year={2015}
}

@inproceedings{matchingnetwork,
	title={Matching networks for one shot learning},
	author={Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
	booktitle=NIPS,
	year={2016}
}

@inproceedings{prototypical,
	title={Prototypical networks for few-shot learning},
	author={Snell, Jake and Swersky, Kevin and Zemel, Richard},
	booktitle=NIPS,
	year={2017}
}

@inproceedings{pytorch,
	title={Automatic differentiation in pytorch},
	author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
    booktitle={ARXIV},
	year={2017}
}

@INPROCEEDINGS{tao2018fss, 
	author = {Tao Hu and Pengwan Yang and Chiliang Zhang and Gang Yu and Yadong Mu and Cees G. M. Snoek}, 
	title = {Attention-based Multi-Context Guiding for Few-Shot Semantic Segmentation}, 
	booktitle = AAAI, 
	year = {2019}, 
	howpublished = "\url{http://taohu.me/note/few-shot-seg.pdf}"
}

@INPROCEEDINGS{focal,
        author = {Pengwan Yang and Vincent Tao Hu and Pascal Mettes and Cees G. M. Snoek},
        title = {Localizing the Common Action Among a Few Videos},
        booktitle = {ECCV},
       
        year = {2020},
      }
      

@inproceedings{transformer,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle=NIPS,
  year={2017}
}

@inproceedings{nl,
  title={Non-local neural networks},
  author={Wang, Xiaolong and Girshick, Ross and Gupta, Abhinav and He, Kaiming},
  booktitle=CVPR,
  year={2018}
}
@inproceedings{shi2017weakly,
  title={Weakly supervised object localization using things and stuff transfer},
  author={Shi, Miaojing and Caesar, Holger and Ferrari, Vittorio},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{wang2015relaxed,
  title={Relaxed multiple-instance SVM with application to object discovery},
  author={Wang, Xinggang and Zhu, Zhuotun and Yao, Cong and Bai, Xiang},
  booktitle=ICCV,
  year={2015}
}

@inproceedings{tang2018weakly,
  title={Weakly supervised region proposal network and object detection},
  author={Tang, Peng and Wang, Xinggang and Wang, Angtian and Yan, Yongluan and Liu, Wenyu and Huang, Junzhou and Yuille, Alan},
  booktitle=ECCV,
  year={2018}
}

@inproceedings{guo2013robust,
  title={Robust object co-detection},
  author={Guo, Xin and Liu, Dong and Jou, Brendan and Zhu, Mojun and Cai, Anni and Chang, Shih-Fu},
  booktitle=CVPR,
  year={2013}
}

@inproceedings{codetection,
  title={Object co-detection},
  author={Bao, Sid Yingze and Xiang, Yu and Savarese, Silvio},
  booktitle=ECCV,
  year={2012},
}

@inproceedings{hayder2014object,
  title={Object co-detection via efficient inference in a fully-connected crf},
  author={Hayder, Zeeshan and Salzmann, Mathieu and He, Xuming},
  booktitle=ECCV,
  year={2014},
}



@inproceedings{marcus2018deep,
  title={Deep learning: A critical appraisal},
  author={Marcus, Gary},
  booktitle={ARXIV},
  year={2018}
}


@inproceedings{jie2017deep,
  title={Deep self-taught learning for weakly supervised object localization},
  author={Jie, Zequn and Wei, Yunchao and Jin, Xiaojie and Feng, Jiashi and Liu, Wei},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{tang2017multiple,
  title={Multiple instance detection network with online instance classifier refinement},
  author={Tang, Peng and Wang, Xinggang and Bai, Xiang and Liu, Wenyu},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{wang2014weakly,
  title={Weakly supervised object localization with latent category learning},
  author={Wang, Chong and Ren, Weiqiang and Huang, Kaiqi and Tan, Tieniu},
  booktitle=ECCV,
  year={2014},
}


@inproceedings{bansal2018zero,
  title={Zero-shot object detection},
  author={Bansal, Ankan and Sikka, Karan and Sharma, Gaurav and Chellappa, Rama and Divakaran, Ajay},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{gavrilyuk2018actor,
  title={Actor and action video segmentation from a sentence},
  author={Gavrilyuk, Kirill and Ghodrati, Amir and Li, Zhenyang and Snoek, Cees G. M.},
  booktitle=CVPR,
  year={2018}
}

@INPROCEEDINGS{GavvesICCV15, 
  author = {Efstratios Gavves and Thomas Mensink and Tatiana Tommasi and Cees G. M. Snoek and Tinne Tuytelaars}, 
  title = {Active Transfer Learning with Zero-Shot Priors: Reusing Past Datasets for Future Tasks}, 
  booktitle = ICCV, 
  year = {2015}, 
}

@INPROCEEDINGS{gokberk2014multi,
  title={Multi-fold mil training for weakly supervised object localization},
  author={Gokberk Cinbis, Ramazan and Verbeek, Jakob and Schmid, Cordelia},
  booktitle ={CVPR}, 
  year={2014}
}


@inproceedings{cho2014properties,
  title={On the properties of neural machine translation: Encoder-decoder approaches},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Bahdanau, Dzmitry and Bengio, Yoshua},
  booktitle={ARXIV},
  year={2014}
}

@inproceedings{dai2017temporal,
  title={Temporal context network for activity localization in videos},
  author={Dai, Xiyang and Singh, Bharat and Zhang, Guyue and Davis, Larry S and Qiu Chen, Yan},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{wang2014action,
  title={Action recognition and detection by combining motion and appearance features},
  author={Wang, Limin and Qiao, Yu and Tang, Xiaoou},
  booktitle={THUMOS14 Action Recognition Challenge},
  year={2014}
}

@inproceedings{gao2018ctap,
  title={Ctap: Complementary temporal action proposal generation},
  author={Gao, Jiyang and Chen, Kan and Nevatia, Ram},
  booktitle=ECCV,
  year={2018}
}


@inproceedings{Duchenne2009,
  title={Automatic Annotation of Human Actions in Video},
  author={Olivier Duchenne and Ivan Laptev and Josef Sivic and Francis Bach and Jean Ponce},
  booktitle={ICCV},
  year={2009}
}

@inproceedings{maaten2008visualizing,
  title={Visualizing data using t-SNE},
  author={Maaten, Laurens van der and Hinton, Geoffrey},
  booktitle=JMLR,
  year={2008}
}

@inproceedings{liu2019large,
  title={Large-Scale Long-Tailed Recognition in an Open World},
  author={Liu, Ziwei and Miao, Zhongqi and Zhan, Xiaohang and Wang, Jiayun and Gong, Boqing and Yu, Stella X},
  booktitle={CVPR},
  year={2019}
}


@inproceedings{soomro2017unsupervised,
  title={Unsupervised action discovery and localization in videos},
  author={Soomro, Khurram and Shah, Mubarak},
  booktitle=ICCV,
  year={2017}
}



@inproceedings{junior2019zero,
  title={Zero-Shot Action Recognition in Videos: A Survey},
  author={Junior, Valter Lu{\'\i}s Estevam and Pedrini, Helio and Menotti, David},
  booktitle={ARXIV},
  year={2019}
}

@inproceedings{shaban2019learning,
  title={Learning to Find Common Objects Across Image Collections},
  author={Shaban, Amirreza and Rahimi, Amir and Gould, Stephen and Boots, Byron and Hartley, Richard},
  booktitle=ICCV,
  year={2019}
}


@inproceedings{oneata2013fisher,
  title={Action and event recognition with fisher vectors on a compact feature set},
  author={Dan Oneata and Jakob Verbeek and Cordelia Schmid},
  booktitle=ICCV,
  year={2013}
}



@InProceedings{gao2017iccv,
author = {Jiyang Gao and Zhenheng Yang and Chen Sun and Kan Chen and Ram Nevatia},
title = {TURN TAP: Temporal Unit Regression Network for Temporal Action Proposals},
booktitle = ICCV,
year = {2017}
}

@INPROCEEDINGS{damen2018epic,
   title={Scaling Egocentric Vision: The EPIC-KITCHENS Dataset},
   author={Damen, Dima and Doughty, Hazel and Farinella, Giovanni Maria  and Fidler, Sanja and 
           Furnari, Antonino and Kazakos, Evangelos and Moltisanti, Davide and Munro, Jonathan 
           and Perrett, Toby and Price, Will and Wray, Michael},
   booktitle=ECCV,
   year={2018}
} 

@inproceedings{lin2018bsn,
  title={{BSN}: Boundary Sensitive Network for Temporal Action Proposal Generation},
  author={Tianwei Lin and Xu Zhao and Haisheng Su and Chongjing Wang and Ming Yang},
  booktitle=ECCV,
  year={2018}
}

@InProceedings{nguyen2019iccv,
author = {Nguyen, Phuc Xuan and Ramanan, Deva and Fowlkes, Charless C.},
title = {Weakly-Supervised Action Localization With Background Modeling},
booktitle = ICCV,
year = {2019}
}

@inproceedings{paul2018wtalc,
  title={W-TALC: Weakly-supervised Temporal Activity Localization and Classification},
  author={Sujoy Paul and Sourya Roy and Amit K Roy-Chowdhury},
  booktitle=ECCV,
  year={2018}
}

@inproceedings{wang2017untrimmed,
  title={Untrimmednets for weakly supervised action recognition and detection},
  author={Limin Wang and Yuanjun Xiong and Dahua Lin and Luc Van Gool},
  booktitle=CVPR,
  year={2017}
}


@inproceedings{dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting},
  author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  booktitle=JMLR,
  year={2014},
}


@inproceedings{silco2019,
  title={SILCO: Show a Few Images, Localize the Common Object},
  author={Hu, Tao and Mettes, Pascal and Huang, Jia-Hong and Snoek, Cees G. M.},
  booktitle=ICCV,
  year={2019}
}



@inproceedings{mettes2017spatial,
	title={Spatial-aware object embeddings for zero-shot localization and classification of actions},
	author={Mettes, Pascal and Snoek, Cees G. M. },
	booktitle=ICCV,
	year={2017}
}

@inproceedings{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  booktitle=ICML,
  year={2017},
}

@inproceedings{yang2018one,
  title={One-shot action localization by learning sequence matching network},
  author={Yang, Hongtao and He, Xuming and Porikli, Fatih},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{xu2018similarity,
  title={Similarity R-C3D for Few-shot Temporal Activity Detection},
  author={Xu, Huijuan and Kang, Bingyi and Sun, Ximeng and Feng, Jiashi and Saenko, Kate and Darrell, Trevor},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{xu2017r,
  title={R-c3d: Region convolutional 3d network for temporal activity detection},
  author={Xu, Huijuan and Das, Abir and Saenko, Kate},
  booktitle=ICCV,
  year={2017}
}


@inproceedings{feng2018video,
  title={Video re-localization},
  author={Feng, Yang and Ma, Lin and Liu, Wei and Zhang, Tong and Luo, Jiebo},
  booktitle=ECCV,
  year={2018}
}
@inproceedings{buch2017sst,
  title={Sst: Single-stream temporal action proposals},
  author={Buch, Shyamal and Escorcia, Victor and Shen, Chuanqi and Ghanem, Bernard and Carlos Niebles, Juan},
  booktitle=CVPR,
  year={2017}
}
@inproceedings{liu2017neural,
  title={Neural person search machines},
  author={Liu, Hao and Feng, Jiashi and Jie, Zequn and Jayashree, Karlekar and Zhao, Bo and Qi, Meibin and Jiang, Jianguo and Yan, Shuicheng},
  booktitle=ICCV,
  year={2017}
}
@inproceedings{liu2017video,
  title={Video-based person re-identification with accumulative motion context},
  author={Liu, Hao and Jie, Zequn and Jayashree, Karlekar and Qi, Meibin and Jiang, Jianguo and Yan, Shuicheng and Feng, Jiashi},
  booktitle={IEEE T CIRC SYST VID},
  volume={28},
  number={10},
  pages={2788--2802},
  year={2017},
  publisher={IEEE}
}


@inproceedings{lin2015bilinear,
  title={Bilinear cnn models for fine-grained visual recognition},
  author={Lin, Tsung-Yu and RoyChowdhury, Aruni and Maji, Subhransu},
  booktitle=ICCV,
  year={2015}
}
@inproceedings{tran2015learning,
  title={Learning spatiotemporal features with 3d convolutional networks},
  author={Tran, Du and Bourdev, Lubomir and Fergus, Rob and Torresani, Lorenzo and Paluri, Manohar},
  booktitle=ICCV,
  year={2015}
}
@inproceedings{caba2015activitynet,
  title={Activitynet: A large-scale video benchmark for human activity understanding},
  author={Caba Heilbron, Fabian and Escorcia, Victor and Ghanem, Bernard and Carlos Niebles, Juan},
  booktitle=CVPR,
  year={2015}
}
@inproceedings{girshick2015fast,
  title={Fast r-cnn},
  author={Girshick, Ross},
  booktitle=ICCV,
  year={2015}
}



@inproceedings{kay2017kinetics,
  title={The kinetics human action video dataset},
  author={Kay, Will and Carreira, Joao and Simonyan, Karen and Zhang, Brian and Hillier, Chloe and Vijayanarasimhan, Sudheendra and Viola, Fabio and Green, Tim and Back, Trevor and Natsev, Paul and Suleyman, Mustafa  and Zisserman, Andrew},
  booktitle={ARXIV},
  year={2017}
}
@inproceedings{idrees2017thumos,
  title={The THUMOS challenge on action recognition for videos “in the wild”},
  author={Idrees, Haroon and Zamir, Amir R and Jiang, Yu-Gang and Gorban, Alex and Laptev, Ivan and Sukthankar, Rahul and Shah, Mubarak},
  booktitle={CVIU},
  year={2017}
}
@inproceedings{chen2011collecting,
  title={Collecting highly parallel data for paraphrase evaluation},
  author={Chen, David L and Dolan, William B},
  booktitle={ACL},
  year={2011}
  }
@inproceedings{gygli2014creating,
  title={Creating summaries from user videos},
  author={Gygli, Michael and Grabner, Helmut and Riemenschneider, Hayko and Van Gool, Luc},
  booktitle=ECCV,
  year={2014}
}
@inproceedings{gkioxari2015finding,
  title={Finding action tubes},
  author={Gkioxari, Georgia and Malik, Jitendra},
  booktitle=CVPR,
  year={2015}
}
@inproceedings{weinzaepfel2015learning,
  title={Learning to track for spatio-temporal action localization},
  author={Weinzaepfel, Philippe and Harchaoui, Zaid and Schmid, Cordelia},
  booktitle=ICCV,
  year={2015}
}
@inproceedings{yu2015fast,
  title={Fast action proposals for human action detection and search},
  author={Yu, Gang and Yuan, Junsong},
  booktitle=CVPR,
  year={2015}
}
@inproceedings{zhu2017tornado,
  title={Tornado: A spatio-temporal convolutional regression network for video action proposal},
  author={Zhu, Hongyuan and Vial, Romain and Lu, Shijian},
  booktitle=CVPR,
  year={2017}
}
@inproceedings{escorcia2016daps,
  title={Daps: Deep action proposals for action understanding},
  author={Escorcia, Victor and Heilbron, Fabian Caba and Niebles, Juan Carlos and Ghanem, Bernard},
  booktitle=ECCV,
  year={2016}
}
@inproceedings{ma2016learning,
  title={Learning activity progression in lstms for activity detection and early detection},
  author={Ma, Shugao and Sigal, Leonid and Sclaroff, Stan},
  booktitle=CVPR,
  year={2016}
}
@inproceedings{shou2016temporal,
  title={Temporal action localization in untrimmed videos via multi-stage cnns},
  author={Shou, Zheng and Wang, Dongang and Chang, Shih-Fu},
  booktitle=CVPR,
  year={2016}
}
@inproceedings{singh2016multi,
  title={A multi-stream bi-directional recurrent neural network for fine-grained action detection},
  author={Singh, Bharat and Marks, Tim K and Jones, Michael and Tuzel, Oncel and Shao, Ming},
  booktitle=CVPR,
  year={2016}
}
@inproceedings{yeung2016end,
  title={End-to-end learning of action detection from frame glimpses in videos},
  author={Yeung, Serena and Russakovsky, Olga and Mori, Greg and Fei-Fei, Li},
  booktitle=CVPR,
  year={2016}
}
@inproceedings{Seo2011Action,
  title={Action recognition from one example},
  author={Seo, H.J., Milanfar},
  booktitle=PAMI,
  year={2011}
}


@inproceedings{chao2018rethinking,
  title={Rethinking the faster r-cnn architecture for temporal action localization},
  author={Chao, Yu-Wei and Vijayanarasimhan, Sudheendra and Seybold, Bryan and Ross, David A and Deng, Jia and Sukthankar, Rahul},
  booktitle=CVPR,
  year={2018}
}
@inproceedings{zhang2019localizing,
  title={Localizing unseen activities in video via image query},
  author={Zhang, Zhu and Zhao, Zhou and Lin, Zhijie and Song, Jingkuan and Cai, Deng},
  booktitle={IJCAI},
  year={2019}
}
@inproceedings{hara2017learning,
  title={Learning spatio-temporal features with 3D residual networks for action recognition},
  author={Hara, Kensho and Kataoka, Hirokatsu and Satoh, Yutaka},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{ba2016layer,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  booktitle={ARXIV},
  year={2016}
}

@inproceedings{kalogeiton2017joint,
  title={Joint learning of object and action detectors},
  author={Kalogeiton, Vicky and Weinzaepfel, Philippe and Ferrari, Vittorio and Schmid, Cordelia},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{jain2015objects2action,
  title={Objects2action: Classifying and localizing actions without any video example},
  author={Jain, Mihir and van Gemert, Jan C and Mensink, Thomas and Snoek, Cees G. M. },
  booktitle=ICCV,
  year={2015}
}
@inproceedings{nguyen2018weakly,
  title={Weakly supervised action localization by sparse temporal pooling network},
  author={Nguyen, Phuc and Liu, Ting and Prasad, Gautam and Han, Bohyung},
  booktitle=CVPR,
  year={2018}
}
@inproceedings{karpathy2014large,
  title={Large-scale video classification with convolutional neural networks},
  author={Karpathy, Andrej and Toderici, George and Shetty, Sanketh and Leung, Thomas and Sukthankar, Rahul and Fei-Fei, Li},
  booktitle=CVPR,
  year={2014}
}
@inproceedings{bojanowski2014weakly,
  title={Weakly supervised action labeling in videos under ordering constraints},
  author={Bojanowski, Piotr and Lajugie, R{\'e}mi and Bach, Francis and Laptev, Ivan and Ponce, Jean and Schmid, Cordelia and Sivic, Josef},
  booktitle=ECCV,
  year={2014}
}
@inproceedings{kumar2017hide,
  title={Hide-and-seek: Forcing a network to be meticulous for weakly-supervised object and action localization},
  author={Kumar Singh, Krishna and Jae Lee, Yong},
  booktitle=ICCV,
  year={2017}
}
@inproceedings{yang2017common,
  title={Common action discovery and localization in unconstrained videos},
  author={Yang, Jiong and Yuan, Junsong},
  booktitle=ICCV,
  year={2017}
}
@inproceedings{kuehne2019hybrid,
  title={A Hybrid RNN-HMM Approach for Weakly Supervised Temporal Action Segmentation},
  author={Kuehne, Hilde and Richard, Alexander and Gall, Juergen},
  booktitle={ARXIV},
  year={2019}
}
@inproceedings{sawatzky2018ex,
  title={Ex Paucis Plura: Learning Affordance Segmentation from Very Few Examples},
  author={Sawatzky, Johann and Garbade, Martin and Gall, Juergen},
  booktitle={GCPR},
  year={2018}
}

@article{linemodsne,
author = {Hinterstoisser, Stefan and Cagniart, Cedric and Ilic, Slobodan and Sturm, Peter and Navab, Nassir and Fua, Pascal and Lepetit, Vincent and Lepetit, bullet},
year = {2012},
title = {Gradient Response Maps for Real-Time Detection of Texture-Less Objects},
journal = {PAMI},
}

@inproceedings{iqbal2019enhancing,
  title={Enhancing Temporal Action Localization with Transfer Learning from Action Recognition},
  author={Iqbal, Ahsan and Richard, Alexander and Gall, Juergen},
  booktitle={ICCV Workshops},
  year={2019}
}


@INPROCEEDINGS{JainCVPR20, 
  author = {Mihir Jain and Amir Ghodrati and Cees G. M. Snoek}, 
  title = {{ActionBytes}: Learning from Trimmed Videos to Localize Actions}, 
  booktitle = {CVPR}, 
  year = {2020}
}


@inproceedings{deepsteer,
	title={Deep Steering: Learning End-to-End Driving Model from Spatial and Temporal Visual Cues},
	author={Chi, Lu and Mu, Yadong},
	booktitle={ARXIV},
	year={2017}
}


@inproceedings{NLSPN,
    title={Non-Local Spatial Propagation Network for Depth Completion},
    author={Park, Jinsun and Joo, Kyungdon and Hu, Zhe and Liu, Chi-Kuei and Kweon, In So},
    booktitle={ECCV},
    year={2020}
}

@misc{StructMDC,
      title={Struct-MDC: Mesh-Refined Unsupervised Depth Completion Leveraging Structural Regularities from Visual SLAM}, 
      author={Jinwoo Jeon and Hyunjun Lim and Dong-Uk Seo and Hyun Myung},
      year={2022},
booktitle={Arxiv},
     
}

@article{DSN,
   title={On deep learning techniques to boost monocular depth estimation for autonomous navigation},
   journal={Robotics and Autonomous Systems},
   author={de Queiroz Mendes, Raul and Ribeiro, Eduardo Godinho and dos Santos Rosa, Nicolas and Grassi, Valdir},
   year={2021},
   }


@article{threefilterstonormal,
   title={Three-Filters-to-Normal: An Accurate and Ultrafast Surface Normal Estimator},
   journal={IEEE Robotics and Automation Letters},
   author={Fan, Rui and Wang, Hengli and Xue, Bohuan and Huang, Huaiyang and Wang, Yuan and Liu, Ming and Pitas, Ioannis},
   year={2021}
}


@book{normalestimategradient,
  added-at = {2015-03-23T00:00:00.000+0100},
  author = {Forsyth, David A. and Ponce, Jean},
  biburl = {https://www.bibsonomy.org/bibtex/24e26ef656dc22317d8ed6d0cfad2d3bc/dblp},
  ee = {http://vig.pearsoned.com/store/product/1,1207,store-12521_isbn-013608592X,00.html},
  interhash = {a4dfa38179479650cae77eb72b893bb6},
  intrahash = {4e26ef656dc22317d8ed6d0cfad2d3bc},
  isbn = {978-0-273-76414-4},
  keywords = {dblp},
  pages = {1-791},
  publisher = {Pitman},
  timestamp = {2015-06-18T09:49:18.000+0200},
  title = {Computer Vision - A Modern Approach, Second Edition.},
  year = 2012
}



@inproceedings{zink2018automated,
	title={Automated dataset generation for image recognition using the example of taxonomy},
	author={Zink, Jaro Milan},
	booktitle={ARXIV},
	year={2018}
}

@inproceedings{han2016dsd,
	title={Dsd: Regularizing deep neural networks with dense-sparse-dense training flow},
	author={Han, Song and Pool, Jeff and Narang, Sharan and Mao, Huizi and Tang, Shijian and Elsen, Erich and Catanzaro, Bryan and Tran, John and Dally, William J},
	booktitle={ARXIV preprint ARXIV:1607.04381},
	year={2016}
}

@inproceedings{han2015deep,
	title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
	author={Han, Song and Mao, Huizi and Dally, William J},
	booktitle={ARXIV preprint ARXIV:1510.00149},
	year={2015}
}

@inproceedings{he2016identity,
	title={Identity mappings in deep residual networks},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=ECCV,
	pages={630--645},
	year={2016},
	organization={Springer}
}



@inproceedings{deconvnet,
	title={Learning deconvolution network for semantic segmentation},
	author={Noh, Hyeonwoo and Hong, Seunghoon and Han, Bohyung},
	booktitle={Proceedings of the IEEE International Conference on Computer Vision},
	pages={1520--1528},
	year={2015}
}

@inproceedings{hed,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle={Proceedings of the IEEE international conference on computer vision},
	pages={1395--1403},
	year={2015}
}

@inproceedings{shen2017dsod,
	title={Dsod: Learning deeply supervised object detectors from scratch},
	author={Shen, Zhiqiang and Liu, Zhuang and Li, Jianguo and Jiang, Yu-Gang and Chen, Yurong and Xue, Xiangyang},
	booktitle={The IEEE International Conference on Computer Vision (ICCV)},
	volume={3},
	number={6},
	pages={7},
	year={2017}
}


@inproceedings{wang2017understanding,
	title={Understanding convolution for semantic segmentation},
	author={Wang, Panqu and Chen, Pengfei and Yuan, Ye and Liu, Ding and Huang, Zehua and Hou, Xiaodi and Cottrell, Garrison},
	booktitle={ARXIV preprint ARXIV:1702.08502},
	year={2017}
}

@inproceedings{maggiori2017dataset,
	title={Can Semantic Labeling Methods Generalize to Any City? The Inria Aerial Image Labeling Benchmark},
	author={Maggiori, Emmanuel and Tarabalka, Yuliya and Charpiat, Guillaume and Alliez, Pierre},
	booktitle={IEEE International Geoscience and Remote Sensing Symposium (IGARSS)},
	year={2017},
	organization={IEEE}
}


@inproceedings{chen2017rethinking,
	title={Rethinking atrous convolution for semantic image segmentation},
	author={Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig},
	booktitle={ARXIV preprint ARXIV:1706.05587},
	year={2017}
}





@inproceedings{liu2017learning,
	title={Learning affinity via spatial propagation networks},
	author={Liu, Sifei and De Mello, Shalini and Gu, Jinwei and Zhong, Guangyu and Yang, Ming-Hsuan and Kautz, Jan},
	booktitle={Advances in Neural Information Processing Systems},
	pages={1519--1529},
	year={2017}
}

@inproceedings{zheng2015conditional,
	title={Conditional random fields as recurrent neural networks},
	author={Zheng, Shuai and Jayasumana, Sadeep and Romera-Paredes, Bernardino and Vineet, Vibhav and Su, Zhizhong and Du, Dalong and Huang, Chang and Torr, Philip HS},
	booktitle=CVPR,
	year={2015}
}

@inproceedings{pspnet,
	title={Pyramid scene parsing network},
	author={Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
	booktitle={IEEE Conf. on Computer Vision and Pattern Recognition (CVPR)},
	pages={2881--2890},
	year={2017}
}



@inproceedings{badrinarayanan2017segnet,
	title={Segnet: A deep convolutional encoder-decoder architecture for image segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle=PAMI,
	volume={39},
	number={12},
	pages={2481--2495},
	year={2017},
	publisher={IEEE}
}


@inproceedings{xie2015holistically,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle={Proceedings of the IEEE international conference on computer vision},
	pages={1395--1403},
	year={2015}
}

@inproceedings{oquab2014learning,
	title={Learning and transferring mid-level image representations using convolutional neural networks},
	author={Oquab, Maxime and Bottou, Leon and Laptev, Ivan and Sivic, Josef},
	booktitle={Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on},
	pages={1717--1724},
	year={2014},
	organization={IEEE}
}

@inproceedings{zagoruyko2016wide,
	title={Wide residual networks},
	author={Zagoruyko, Sergey and Komodakis, Nikos},
	booktitle={ARXIV preprint ARXIV:1605.07146},
	year={2016}
}

@inproceedings{krahenbuhl2011efficient,
	title={Efficient inference in fully connected crfs with gaussian edge potentials},
	author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
	booktitle=NIPS,
	year={2011}
}




@inproceedings{huang2017densely,
	title={Densely connected convolutional networks},
	author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	volume={1},
	number={2},
	pages={3},
	year={2017}
}



@inproceedings{yu2015multi,
	title={Multi-scale context aggregation by dilated convolutions},
	author={Yu, Fisher and Koltun, Vladlen},
	booktitle={ARXIV preprint ARXIV:1511.07122},
	year={2015}
}


@misc{Authors14,
	author = {Authors},
	title = {The frobnicatable foo filter},
	note = {BMVC14 submission ID 324. Supplied as additional material {\tt bmvc14.pdf}},
	year = 2014
}

@misc{Authors14b,
	author = {Authors},
	title = {Frobnication tutorial},
	note = {Supplied as additional material {\tt tr.pdf}},
	year = 2014
}

@inproceedings{Alpher02,
	author = {A. Alpher},
	title = {Frobnication},
	booktitle = {booktitle of Foo},
	volume = 12,
	number = 1,
	pages = {234--778},
	year = 2002
}

@inproceedings{Alpher03,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe},
	title = {Frobnication revisited},
	booktitle = {booktitle of Foo},
	volume = 13,
	number = 1,
	pages = {234--778},
	year = 2003
}

@inproceedings{Alpher04,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe and G. Gamow},
	title = {Can a machine frobnicate?},
	booktitle = {booktitle of Foo},
	volume = 14,
	number = 1,
	pages = {234--778},
	year = 2004
}

@inproceedings{segnet,
	title={Segnet: A deep convolutional encoder-decoder architecture for image segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle={IEEE transactions on pattern analysis and machine intelligence},
	volume={39},
	number={12},
	pages={2481--2495},
	year={2017},
	publisher={IEEE}
}






@inproceedings{modelnet40,
  title={3d shapenets: A deep representation for volumetric shapes},
  author={Wu, Zhirong and Song, Shuran and Khosla, Aditya and Yu, Fisher and Zhang, Linguang and Tang, Xiaoou and Xiao, Jianxiong},
  booktitle=CVPR,
  year={2015}
}

@inproceedings{adamixup,
  title={Mixup as locally linear out-of-manifold regularization},
  author={Guo, Hongyu and Mao, Yongyi and Zhang, Richong},
  booktitle=AAAI,
  year={2019}
}

@inproceedings{ict,
  title={Interpolation consistency training for semi-supervised learning},
  author={Verma, Vikas and Lamb, Alex and Kannala, Juho and Bengio, Yoshua and Lopez-Paz, David},
  booktitle={IJCAI},
  year={2019}
}

@inproceedings{achlioptas2018learning,
  title={Learning Representations and Generative Models for 3D Point Clouds},
  author={Achlioptas, Panos and Diamanti, Olga and Mitliagkas, Ioannis and Guibas, Leonidas},
  booktitle=ICML,
  year={2018}
}

@inproceedings{liu2019morphing,
  title={Morphing and Sampling Network for Dense Point Cloud Completion},
  author={Liu, Minghua and Sheng, Lu and Yang, Sheng and Shao, Jing and Hu, Shi-Min},
  booktitle={CoRR},
  year={2019}
}

@inproceedings{berthelot2019mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin A},
  booktitle={NeurIPS},
  year={2019}
}

@inproceedings{cutout,
  title={Improved regularization of convolutional neural networks with cutout},
  author={DeVries, Terrance and Taylor, Graham W},
  booktitle={CoRR},
  year={2017}
}

@inproceedings{manifoldmixup,
  title={Manifold mixup: Better representations by interpolating hidden states},
  author={Verma, Vikas and Lamb, Alex and Beckham, Christopher and Najafi, Amir and Mitliagkas, Ioannis and Courville, Aaron and Lopez-Paz, David and Bengio, Yoshua},
  booktitle=ICML,
  year={2019}
}

@inproceedings{mixup,
  title={mixup: Beyond empirical risk minimization},
  author={Zhang, Hongyi and Cisse, Moustapha and Dauphin, Yann N and Lopez-Paz, David},
  booktitle=ICLR,
  year={2017}
}

@inproceedings{dropout,
  title={Dropout: a simple way to prevent neural networks from overfitting},
  author={Srivastava, Nitish and Hinton, Geoffrey and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  booktitle=JMLR,
  year={2014},
}

@inproceedings{li2018pointcnn,
  title={Pointcnn: Convolution on x-transformed points},
  author={Li, Yangyan and Bu, Rui and Sun, Mingchao and Wu, Wei and Di, Xinhan and Chen, Baoquan},
  booktitle={NeurIPS},
  year={2018}
}

@inproceedings{dgcnn,
  title={Dynamic graph cnn for learning on point clouds},
  author={Wang, Yue and Sun, Yongbin and Liu, Ziwei and Sarma, Sanjay E and Bronstein, Michael M and Solomon, Justin M},
  booktitle={TOG},
  year={2019}
}

@inproceedings{qi2017pointnet++,
  title={Pointnet++: Deep hierarchical feature learning on point sets in a metric space},
  author={Qi, Charles Ruizhongtai and Yi, Li and Su, Hao and Guibas, Leonidas J},
  booktitle={NeurIPS},
  year={2017}
}

@inproceedings{qi2017pointnet,
  title={Pointnet: Deep learning on point sets for 3d classification and segmentation},
  author={Qi, Charles R and Su, Hao and Mo, Kaichun and Guibas, Leonidas J},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{cheraghian2019transductive,
  title={Transductive Zero-Shot Learning for 3D Point Cloud Classification},
  author={Cheraghian, Ali and Rahman, Shafin and Campbell, Dylan and Petersson, Lars},
  booktitle=WACV,
  year={2019}
}

@inproceedings{cheraghian2019mitigating,
  title={Mitigating the hubness problem for zero-shot learning of 3d objects},
  author={Cheraghian, Ali and Rahman, Shafin and Campbell, Dylan and Petersson, Lars},
  booktitle=BMVC,
  year={2019}
}

@inproceedings{jain2019few,
  title={Few-Shot Point Cloud Region Annotation with Human in the Loop},
  author={Jain, Siddhant and Munukutla, Sowmya and Held, David},
  booktitle={ICML workshop},
  year={2019}
}

@inproceedings{cheraghian2019zero,
  title={Zero-shot learning of 3d point cloud objects},
  author={Cheraghian, Ali and Rahman, Shafin and Petersson, Lars},
  booktitle={International Conference on Machine Vision Applications (MVA)},
  year={2019},
}


@inproceedings{tokozume2018between,
  title={Between-class learning for image classification},
  author={Tokozume, Yuji and Ushiku, Yoshitaka and Harada, Tatsuya},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{jonker1987shortest,
  title={A shortest augmenting path algorithm for dense and sparse linear assignment problems},
  author={Jonker, Roy and Volgenant, Anton},
  booktitle={Computing},
  year={1987},
}

@inproceedings{rubner2000earth,
  title={The earth mover's distance as a metric for image retrieval},
  author={Rubner, Yossi and Tomasi, Carlo and Guibas, Leonidas J},
  booktitle={IJCV},
  year={2000}
}

@inproceedings{fan2017point,
  title={A point set generation network for 3d object reconstruction from a single image},
  author={Fan, Haoqiang and Su, Hao and Guibas, Leonidas J},
  booktitle={CVPR},
  year={2017}
}


@inproceedings{uy2019scanobjnn,
  title={Revisiting point cloud classification: A new benchmark dataset and classification model on real-world data},
  author={Uy, Mikaela Angelina and Pham, Quang-Hieu and Hua, Binh-Son and Nguyen, Thanh and Yeung, Sai-Kit},
  booktitle={ICCV},
  year={2019}
}

@inproceedings{xu2018spidercnn,
  title={Spidercnn: Deep learning on point sets with parameterized convolutional filters},
  author={Xu, Yifan and Fan, Tianqi and Xu, Mingye and Zeng, Long and Qiao, Yu},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{wu2019pointconv,
  title={Pointconv: Deep convolutional networks on 3d point clouds},
  author={Wu, Wenxuan and Qi, Zhongang and Fuxin, Li},
  booktitle={CVPR},
  year={2019}
}

@inproceedings{yun2019cutmix,
  title={Cutmix: Regularization strategy to train strong classifiers with localizable features},
  author={Yun, Sangdoo and Han, Dongyoon and Oh, Seong Joon and Chun, Sanghyuk and Choe, Junsuk and Yoo, Youngjoon},
  booktitle={ICCV},
  year={2019}
}

@inproceedings{zhang2019shellnet,
  title={Shellnet: Efficient point cloud convolutional neural networks using concentric shells statistics},
  author={Zhang, Zhiyuan and Hua, Binh-Son and Yeung, Sai-Kit},
  booktitle={ICCV},
  year={2019}
}

@inproceedings{zhang2019bag,
  title={Bag of freebies for training object detection neural networks},
  author={Zhang, Zhi and He, Tong and Zhang, Hang and Zhang, Zhongyuan and Xie, Junyuan and Li, Mu},
  booktitle={CoRR},
  year={2019}
}

@inproceedings{cuturi2013sinkhorn,
  title={Sinkhorn distances: Lightspeed computation of optimal transport},
  author={Cuturi, Marco},
  booktitle={NeurIPS},
  year={2013}
}

@inproceedings{solomon2015convolutional,
  title={Convolutional wasserstein distances: Efficient optimal transportation on geometric domains},
  author={Solomon, Justin and De Goes, Fernando and Peyr{\'e}, Gabriel and Cuturi, Marco and Butscher, Adrian and Nguyen, Andy and Du, Tao and Guibas, Leonidas},
  booktitle={TOG},
  year={2015},
}


@inproceedings{hua2016scenenn,
  title={Scenenn: A scene meshes dataset with annotations},
  author={Hua, Binh-Son and Pham, Quang-Hieu and Nguyen, Duc Thanh and Tran, Minh-Khoi and Yu, Lap-Fai and Yeung, Sai-Kit},
  booktitle={3DV},
  year={2016}
}



@inproceedings{french2019cowmix,
  title={Consistency regularization and CutMix for semi-supervised semantic segmentation},
  author={French, Geoff and Aila, Timo and Laine, Samuli and Mackiewicz, Michal and Finlayson, Graham},
  booktitle={CoRR},
  year={2019}
}

@inproceedings{xie2018attentional,
  title={Attentional shapecontextnet for point cloud recognition},
  author={Xie, Saining and Liu, Sainan and Chen, Zeyu and Tu, Zhuowen},
  booktitle={CVPR},
  year={2018}
}







@inproceedings{sung2018learning,
  title={Learning to compare: Relation network for few-shot learning},
  author={Sung, Flood and Yang, Yongxin and Zhang, Li and Xiang, Tao and Torr, Philip HS and Hospedales, Timothy M},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{berthelot2019remixmatch,
  title={ReMixMatch: Semi-Supervised Learning with Distribution Alignment and Augmentation Anchoring},
  author={Berthelot, David and Carlini, Nicholas and Cubuk, Ekin D and Kurakin, Alex and Sohn, Kihyuk and Zhang, Han and Raffel, Colin},
  booktitle={CoRR},
  year={2019}
}

@inproceedings{ravanbakhsh2016deep,
  title={Deep learning with sets and point clouds},
  author={Ravanbakhsh, Siamak and Schneider, Jeff and Poczos, Barnabas},
  booktitle={ARXIV},
  year={2016}
}

@inproceedings{li2018sonet,
  title={So-net: Self-organizing network for point cloud analysis},
  author={Li, Jiaxin and Chen, Ben M and Hee Lee, Gim},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{zaheer2017deep,
  title={Deep sets},
  author={Zaheer, Manzil and Kottur, Satwik and Ravanbakhsh, Siamak and Poczos, Barnabas and Salakhutdinov, Russ R and Smola, Alexander J},
  booktitle={NeurIPS},
  year={2017}
}

@inproceedings{yang2018foldingnet,
  title={Foldingnet: Point cloud auto-encoder via deep grid deformation},
  author={Yang, Yaoqing and Feng, Chen and Shen, Yiru and Tian, Dong},
  booktitle={CVPR},
  pages={206--215},
  year={2018}
}


%   new

@inproceedings{thomas2019kpconv,
  title={Kpconv: Flexible and deformable convolution for point clouds},
  author={Thomas, Hugues and Qi, Charles R and Deschaud, Jean-Emmanuel and Marcotegui, Beatriz and Goulette, Fran{\c{c}}ois and Guibas, Leonidas J},
  booktitle={ICCV},
  year={2019}
}

@inproceedings{li2020pointaugment,
  title={PointAugment: an Auto-Augmentation Framework for Point Cloud Classification},
  author={Li, Ruihui and Li, Xianzhi and Heng, Pheng-Ann and Fu, Chi-Wing},
  booktitle={CVPR},
  year={2020}
}

@inproceedings{wang2020sampling,
  title={Rethinking Sampling in 3D Point Cloud Generative Adversarial Networks},
  author={Wang, He and Jiang, Zetian and Yi, Li and Mo, Kaichun and Su, Hao and Guibas, Leonidas J},
  booktitle={ARXIV preprint ARXIV:2006.07029},
  year={2020}
}



@inproceedings{xian2017zero,
  title={Zero-shot learning-the good, the bad and the ugly},
  author={Xian, Yongqin and Schiele, Bernt and Akata, Zeynep},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{song2018self,
  title={Self-supervised video hashing with hierarchical binary auto-encoder},
  author={Song, Jingkuan and Zhang, Hanwang and Li, Xiangpeng and Gao, Lianli and Wang, Meng and Hong, Richang},
  booktitle={TIP},
  year={2018}
}

@inproceedings{mithun2019weakly,
  title={Weakly supervised video moment retrieval from text queries},
  author={Mithun, Niluthpol Chowdhury and Paul, Sujoy and Roy-Chowdhury, Amit K},
  booktitle={CVPR},
  year={2019}
}

@inproceedings{xiong2012coaction,
  title={Coaction discovery: segmentation of common actions across multiple videos},
  author={Xiong, Caiming and Corso, Jason J},
  booktitle={Proceedings of the Twelfth International Workshop on Multimedia Data Mining},
  pages={17--24},
  year={2012},
  organization={ACM}
}

@InProceedings{hoai12,
  title = 	 {Maximum Margin Temporal Clustering},
  author = 	 {Minh Hoai and Fernando De La Torre},
  booktitle = 	 {Proceedings of the Fifteenth International Conference on Artificial Intelligence and Statistics},
  pages = 	 {520--528},
  year = 	 {2012},
}

@inproceedings{liu2013video,
  title={Video event recognition using concept attributes},
  author={Liu, Jingen and Yu, Qian and Javed, Omar and Ali, Saad and Tamrakar, Amir and Divakaran, Ajay and Cheng, Hui and Sawhney, Harpreet},
  booktitle={2013 IEEE Workshop on Applications of Computer Vision (WACV)},
  pages={339--346},
  year={2013},
  organization={IEEE}
}


@inproceedings{oksuz2019imbalance,
    title={Imbalance Problems in Object Detection: A Review},
    author={Kemal Oksuz and Baris Can Cam and Sinan Kalkan and Emre Akbas},
    booktitle={ARXIV},
    year={2019},
}



@inproceedings{BuloNK17,
  author    = {Samuel Rota Bul{\`{o}} and
               Gerhard Neuhold and
               Peter Kontschieder},
  title     = {Loss Max-Pooling for Semantic Image Segmentation},
  booktitle   = {CoRR},
  year      = {2017}
}

@InProceedings{kervadec19a,
  title = 	 {Boundary loss for highly unbalanced segmentation},
  author = 	 {Kervadec, Hoel and Bouchtiba, Jihene and Desrosiers, Christian and Granger, Eric and Dolz, Jose and {Ben Ayed}, Ismail},
  booktitle = {MIDL},
  year = {2019}
}

@inproceedings{zhu2014capturing,
  title={Capturing long-tail distributions of object subcategories},
  author={Zhu, Xiangxin and Anguelov, Dragomir and Ramanan, Deva},
  booktitle=CVPR,
  year={2014}
}


@inproceedings{kang2003query,
  title={Query type classification for web document retrieval},
  author={Kang, In-Ho and Kim, GilChang},
  booktitle={SIGIR},
  year={2003}
}


@inproceedings{qin2017fast,
  title={Fast action retrieval from videos via feature disaggregation},
  author={Qin, Jie and Liu, Li and Yu, Mengyang and Wang, Yunhong and Shao, Ling},
  booktitle={CVIU},
  year={2017}
}

@inproceedings{douze2016circulant,
  title={Circulant temporal encoding for video retrieval and temporal alignment},
  author={Douze, Matthijs and Revaud, J{\'e}r{\^o}me and Verbeek, Jakob and J{\'e}gou, Herv{\'e} and Schmid, Cordelia},
  booktitle={IJCV},
  year={2016}
}

@inproceedings{ciptadi2014movement,
  title={Movement pattern histogram for action recognition and retrieval},
  author={Ciptadi, Arridhana and Goodwin, Matthew S and Rehg, James M},
  booktitle=ECCV,
  year={2014}
}

@inproceedings{mettes2019hyperspherical,
    title={Hyperspherical Prototype Networks},
    author={Pascal Mettes and Elise van der Pol and Cees G. M. Snoek},
    booktitle={NeurIPS},
    year={2020}
}


@inproceedings{zhu2018compound,
  title={Compound memory networks for few-shot video classification},
  author={Zhu, Linchao and Yang, Yi},
  booktitle=ECCV,
  year={2018}
}

@inproceedings{escorcia2019temporal,
  title={Temporal Localization of Moments in Video Collections with Natural Language},
  author={Escorcia, Victor and Soldan, Mattia and Sivic, Josef and Ghanem, Bernard and Russell, Bryan},
  booktitle={ARXIV},
  year={2019}
}

@inproceedings{wu2019long,
  title={Long-term feature banks for detailed video understanding},
  author={Wu, Chao-Yuan and Feichtenhofer, Christoph and Fan, Haoqi and He, Kaiming and Krahenbuhl, Philipp and Girshick, Ross},
  booktitle=CVPR,
  year={2019}
}



@inproceedings{chen19closerfewshot,
   author = {Chen, Wei-Yu and Liu, Yen-Cheng and Kira, Zsolt and Wang, Yu-Chiang and  Huang, Jia-Bin},
   title = {A Closer Look at Few-shot Classification},
   booktitle = ICCV,
   year = {2019}
}

@inproceedings{shchur2018pitfalls,
  title={Pitfalls of graph neural network evaluation},
  author={Shchur, Oleksandr and Mumme, Maximilian and Bojchevski, Aleksandar and G{\"u}nnemann, Stephan},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{fasttext,
  title={Bag of tricks for efficient text classification},
  author={Joulin, Armand and Grave, Edouard and Bojanowski, Piotr and Mikolov, Tomas},
  booktitle={ARXIV},
  year={2016}
}

@inproceedings{robins1995catastrophic,
  title={Catastrophic forgetting, rehearsal and pseudorehearsal},
  author={Robins, Anthony},
  booktitle={Connection Science},
  volume={7},
  number={2},
  year={1995}
}

@inproceedings{marginloss,
  title={Sampling matters in deep embedding learning},
  author={Wu, Chao-Yuan and Manmatha, R and Smola, Alexander J and Krahenbuhl, Philipp},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{proxynca,
  title={No fuss distance metric learning using proxies},
  author={Movshovitz-Attias, Yair and Toshev, Alexander and Leung, Thomas K and Ioffe, Sergey and Singh, Saurabh},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{npairs,
  title={Improved deep metric learning with multi-class n-pair loss objective},
  author={Sohn, Kihyuk},
  booktitle=NIPS,
  year={2016}
}


@inproceedings{serra2018overcoming,
	title={Overcoming catastrophic forgetting with hard attention to the task},
	author={Serr{\`a}, Joan and Sur{\'\i}s, D{\'\i}dac and Miron, Marius and Karatzoglou, Alexandros},
	booktitle={ARXIV},
	year={2018}
}

@inproceedings{triplenet,
  title={Deep metric learning using triplet network},
  author={Hoffer, Elad and Ailon, Nir},
  booktitle={IWPR},
  year={2015}
}

@inproceedings{snoek2009concept,
  title={Concept-based video retrieval},
  author={Snoek, Cees G. M. and Worring, Marcel},
  booktitle={Foundations and Trends in Information Retrieval},
  year={2009}
}






@inproceedings{hariharan2017low,
  title={Low-shot visual recognition by shrinking and hallucinating features},
  author={Hariharan, Bharath and Girshick, Ross},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{bart2005cross,
  title={Cross-generalization: Learning novel classes from a single example by feature replacement},
  author={Bart, Evgeniy and Ullman, Shimon},
  booktitle=CVPR,
  year={2005},
}

@inproceedings{luo2019few,
      title={Few-Shot Learning with Global Class Representations},
      author={Luo, Tiange and Li, Aoxue and Xiang, Tao and Huang, Weiran and Wang, Liwei},
      booktitle={ARXIV},
      year={2019}
      }
      


@inproceedings{rusu2018meta,
  title={Meta-learning with latent embedding optimization},
  author={Rusu, Andrei A and Rao, Dushyant and Sygnowski, Jakub and Vinyals, Oriol and Pascanu, Razvan and Osindero, Simon and Hadsell, Raia},
  booktitle={ARXIV},
  year={2018}
}





@inproceedings{elmo,
  title={Deep contextualized word representations},
  author={Peters, Matthew E and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher},
  booktitle=EMNLP,
  year={2014}
}

@inproceedings{word2vec,
  title={Distributed representations of words and phrases and their compositionality},
  author={Mikolov, Tomas and Sutskever, Ilya and Chen, Kai and Corrado, Greg S and Dean, Jeff},
  booktitle=NIPS,
  year={2013}
}

@inproceedings{zhou2017recent,
  title={Recent advance in content-based image retrieval: A literature survey},
  author={Zhou, Wengang and Li, Houqiang and Tian, Qi},
  booktitle={ARXIV},
  year={2017}
}

@inproceedings{faiss,
  title={Billion-scale similarity search with GPUs},
  author={Johnson, Jeff and Douze, Matthijs and J{\'e}gou, Herv{\'e}},
  booktitle={ARXIV},
  year={2017}
}

@inproceedings{torabi2016learning,
  title={Learning language-visual embedding for movie understanding with natural-language},
  author={Torabi, Atousa and Tandon, Niket and Sigal, Leonid},
  booktitle={ARXIV},
  year={2016}
}

@inproceedings{otani2016learning,
  title={Learning joint representations of videos and sentences with web image search},
  author={Otani, Mayu and Nakashima, Yuta and Rahtu, Esa and Heikkil{\"a}, Janne and Yokoya, Naokazu},
  booktitle=ECCV,
  year={2016},
}

@inproceedings{gao2017tall,
  title={Tall: Temporal activity localization via language query},
  author={Gao, Jiyang and Sun, Chen and Yang, Zhenheng and Nevatia, Ram},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{anne2017localizing,
  title={Localizing moments in video with natural language},
  author={Hendricks, Lisa Anne and Wang, Oliver and Shechtman, Eli and Sivic, Josef and Darrell, Trevor and Russell, Bryan},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{hendricks2018localizing,
  title={Localizing moments in video with temporal language},
  author={Hendricks, Lisa Anne and Wang, Oliver and Shechtman, Eli and Sivic, Josef and Darrell, Trevor and Russell, Bryan},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{xu2019multilevel,
  title={Multilevel language and vision integration for text-to-clip retrieval},
  author={Xu, Huijuan and He, Kun and Plummer, Bryan A and Sigal, Leonid and Sclaroff, Stan and Saenko, Kate},
  booktitle=AAAI,
  year={2019}
}

@inproceedings{miech2019howto100m,
  title={HowTo100M: Learning a Text-Video Embedding by Watching Hundred Million Narrated Video Clips},
  author={Miech, Antoine and Zhukov, Dimitri and Alayrac, Jean-Baptiste and Tapaswi, Makarand and Laptev, Ivan and Sivic, Josef},
  booktitle=ICCV,
  year={2019}
}


@inproceedings{huvideoretrieval,
        title={Query by Activity Video in the Wild},
        author={Tao Hu and William Thong and Pascal Mettes and Cees G. M. Snoek},
        booktitle={ARXIV},
        year={2019}
      }
      


@inproceedings{carbonneau2018multiple,
	title={Multiple instance learning: A survey of problem characteristics and applications},
	author={Carbonneau, Marc-Andr{\'e} and Cheplygina, Veronika and Granger, Eric and Gagnon, Ghyslain},
	booktitle={Pattern Recognition},
	year={2018}
}



@inproceedings{li2016weakly,
  title={Weakly supervised object localization with progressive domain adaptation},
  author={Li, Dong and Huang, Jia-Bin and Li, Yali and Wang, Shengjin and Yang, Ming-Hsuan},
  booktitle=CVPR,
  year={2016}
}








@inproceedings{deepsteer,
	title={Deep Steering: Learning End-to-End Driving Model from Spatial and Temporal Visual Cues},
	author={Chi, Lu and Mu, Yadong},
	booktitle={ARXIV},
	year={2017}
}







@inproceedings{zink2018automated,
	title={Automated dataset generation for image recognition using the example of taxonomy},
	author={Zink, Jaro Milan},
	booktitle={ARXIV},
	year={2018}
}

@inproceedings{han2016dsd,
	title={Dsd: Regularizing deep neural networks with dense-sparse-dense training flow},
	author={Han, Song and Pool, Jeff and Narang, Sharan and Mao, Huizi and Tang, Shijian and Elsen, Erich and Catanzaro, Bryan and Tran, John and Dally, William J},
	booktitle={ARXIV},
	year={2016}
}

@inproceedings{han2015deep,
	title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
	author={Han, Song and Mao, Huizi and Dally, William J},
	booktitle={ARXIV},
	year={2015}
}

@inproceedings{he2016identity,
	title={Identity mappings in deep residual networks},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=ECCV,
	year={2016},
}

@inproceedings{visin2016reseg,
	title={Reseg: A recurrent neural network-based model for semantic segmentation},
	author={Visin, Francesco and Romero, Adriana and Cho, Kyunghyun and Matteucci, Matteo and Ciccone, Marco and Kastner, Kyle and Bengio, Yoshua and Courville, Aaron},
	booktitle=CVPRW,
	year={2016}
}

@inproceedings{deconvnet,
	title={Learning deconvolution network for semantic segmentation},
	author={Noh, Hyeonwoo and Hong, Seunghoon and Han, Bohyung},
	booktitle=ICCV,
	year={2015}
}

@inproceedings{hed,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle=ICCV,
	year={2015}
}

@inproceedings{shen2017dsod,
	title={Dsod: Learning deeply supervised object detectors from scratch},
	author={Shen, Zhiqiang and Liu, Zhuang and Li, Jianguo and Jiang, Yu-Gang and Chen, Yurong and Xue, Xiangyang},
	booktitle=ICCV,
	year={2017}
}


@inproceedings{wang2017understanding,
	title={Understanding convolution for semantic segmentation},
	author={Wang, Panqu and Chen, Pengfei and Yuan, Ye and Liu, Ding and Huang, Zehua and Hou, Xiaodi and Cottrell, Garrison},
	booktitle=WACV,
	year={2018}
}

@inproceedings{maggiori2017dataset,
	title={Can Semantic Labeling Methods Generalize to Any City? The Inria Aerial Image Labeling Benchmark},
	author={Maggiori, Emmanuel and Tarabalka, Yuliya and Charpiat, Guillaume and Alliez, Pierre},
	booktitle=IGARSS,
	year={2017},
}


@inproceedings{chen2017rethinking,
	title={Rethinking atrous convolution for semantic image segmentation},
	author={Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig},
	booktitle={ARXIV},
	year={2017}
}







@inproceedings{jegou2017one,
	title={The one hundred layers tiramisu: Fully convolutional densenets for semantic segmentation},
	author={J{\'e}gou, Simon and Drozdzal, Michal and Vazquez, David and Romero, Adriana and Bengio, Yoshua},
	booktitle=CVPRW,
	year={2017}
}

@inproceedings{liu2017learning,
	title={Learning affinity via spatial propagation networks},
	author={Liu, Sifei and De Mello, Shalini and Gu, Jinwei and Zhong, Guangyu and Yang, Ming-Hsuan and Kautz, Jan},
	booktitle=NIPS,
	year={2017}
}

@inproceedings{zheng2015conditional,
	title={Conditional random fields as recurrent neural networks},
	author={Zheng, Shuai and Jayasumana, Sadeep and Romera-Paredes, Bernardino and Vineet, Vibhav and Su, Zhizhong and Du, Dalong and Huang, Chang and Torr, Philip H. S.},
	booktitle=CVPR,
	year={2015}
}




@inproceedings{
sinho_score1,
title={Sampling is as easy as learning the score: theory for diffusion models with minimal data assumptions},
author={Sitan Chen and Sinho Chewi and Jerry Li and Yuanzhi Li and Adil Salim and Anru Zhang},
booktitle=ICLR,
year={2023},
}
%%

@inproceedings{holden_score3,
    author = {Chen, Hongrui and Lee, Holden and Lu, Jianfeng},
    title = {Improved Analysis of Score-based Generative Modeling: User-Friendly Bounds under Minimal Smoothness Assumptions},
    booktitle = ICML,
    year = {2023}
}

@article{child2019generating,
  title={Generating long sequences with sparse transformers},
  author={Child, Rewon and Gray, Scott and Radford, Alec and Sutskever, Ilya},
  journal={arXiv preprint arXiv:1904.10509},
  year={2019}
}

@article{gupta2022diagonal,
  title={Diagonal state spaces are as effective as structured state spaces},
  author={Gupta, Ankit and Gu, Albert and Berant, Jonathan},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={22982--22994},
  year={2022}
}

@inproceedings{sun2021sparse,
  title={Sparse attention with learning to hash},
  author={Sun, Zhiqing and Yang, Yiming and Yoo, Shinjae},
  booktitle={International Conference on Learning Representations},
  year={2021}
}

@article{kingma2023understanding,
  title={Understanding the diffusion objective as a weighted integral of elbos},
  author={Kingma, Diederik P and Gao, Ruiqi},
  journal={arXiv preprint arXiv:2303.00848},
  year={2023}
}

%%

@article{anderson1979reverse-time,
title = {Reverse-time diffusion equation models},
journal = {Stochastic Processes and their Applications},
year = {1982},
author = {Brian D.O. Anderson},
abstract = {Reverse-time stochastic diffusion equation models are defined and it is shown how most processes defined via a forward-time or conventional diffusion equation model have an associated reverse-time model.}
}

@inproceedings{benhamu2022,
  title={Matching normalizing flows and probability paths on manifolds},
  author={Ben-Hamu, Heli and Cohen, Samuel and Bose, Joey and Amos, Brandon and Grover, Aditya and Nickel, Maximilian and Chen, Ricky TQ and Lipman, Yaron},
  booktitle=ICML,
  year={2022}
}

@InProceedings{holden_score2,
  title = 	 {Convergence of score-based generative modeling for general data distributions},
  author =       {Lee, Holden and Lu, Jianfeng and Tan, Yixin},
  booktitle = 	 {ALT},
  year = 	 {2023},
}
%%

@inproceedings{holden_score1,
  author = {Lee, Holden and Lu, Jianfeng and Tan, Yixin},
  booktitle = NeurIPS,
  title = {Convergence for score-based generative modeling with polynomial complexity},
  year = {2022}
}

@inproceedings{pspnet,
	title={Pyramid scene parsing network},
	author={Zhao, Hengshuang and Shi, Jianping and Qi, Xiaojuan and Wang, Xiaogang and Jia, Jiaya},
	booktitle=CVPR,
	year={2017}
}


@article{ma2024sit,
  title={SiT: Exploring Flow and Diffusion-based Generative Models with Scalable Interpolant Transformers},
  author={Ma, Nanye and Goldstein, Mark and Albergo, Michael S and Boffi, Nicholas M and Vanden-Eijnden, Eric and Xie, Saining},
  journal={arXiv preprint arXiv:2401.08740},
  year={2024}
}

@inproceedings{badrinarayanan2017segnet,
	title={SegNet: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle=PAMI,
	year={2017},
}



@inproceedings{xie2015holistically,
	title={Holistically-nested edge detection},
	author={Xie, Saining and Tu, Zhuowen},
	booktitle=ICCV,
	year={2015}
}

@inproceedings{oquab2014learning,
	title={Learning and transferring mid-level image representations using convolutional neural networks},
	author={Oquab, Maxime and Bottou, Leon and Laptev, Ivan and Sivic, Josef},
	booktitle=CVPR,
	year={2014}
}

@inproceedings{zagoruyko2016wide,
	title={Wide residual networks},
	author={Zagoruyko, Sergey and Komodakis, Nikos},
	booktitle={ARXIV},
	year={2016}
}

@inproceedings{krahenbuhl2011efficient,
	title={Efficient inference in fully connected crfs with gaussian edge potentials},
	author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
	booktitle=NIPS,
	year={2011}
}






@inproceedings{huang2017densely,
	title={Densely connected convolutional networks},
	author={Huang, Gao and Liu, Zhuang and Weinberger, Kilian Q and van der Maaten, Laurens},
	booktitle=CVPR,
	year={2017}
}



@inproceedings{yu2015multi,
	title={Multi-Scale Context Aggregation by Dilated Convolutions},
	author={Yu, Fisher and Koltun, Vladlen},
	booktitle=ICLR,
	year={2016}
}


@inproceedings{girshick2015fast,
	title={Fast r-cnn},
	author={Girshick, Ross},
	booktitle=ICCV,
	year={2015}
}



@inproceedings{Authors14,
  title={The Frobnicatable Foo Filter},
  author={Smith, F},
  booktitle={GreatBooks, Atown},
  year={2009}
}

@misc{Authors14b,
	author = {Authors},
	title = {Frobnication tutorial},
	note = {Supplied as additional material {\tt tr.pdf}},
	year = {2014}
}

@inproceedings{Alpher02,
	author = {A. Alpher},
	title = {Frobnication},
	booktitle = {booktitle of Foo},
	volume = 12,
	number = 1,
	pages = {234--778},
	year = 2002
}

@inproceedings{Alpher03,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe},
	title = {Frobnication revisited},
	booktitle = {booktitle of Foo},
	volume = 13,
	number = 1,
	pages = {234--778},
	year = 2003
}

@inproceedings{Alpher04,
	author = {A. Alpher and and J.~P.~N. Fotheringham-Smythe and G. Gamow},
	title = {Can a machine frobnicate?},
	booktitle = {booktitle of Foo},
	volume = 14,
	number = 1,
	pages = {234--778},
	year = 2004
}

@inproceedings{segnet,
	title={SegNet: A Deep Convolutional Encoder-Decoder Architecture for Image Segmentation},
	author={Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto},
	booktitle=PAMI,
	year={2017}
}

@inproceedings{sbd,
	title={Semantic Contours from Inverse Detectors},
	author={Hariharan, Bharath and Arbel{\'a}ez, Pablo and Bourdev, Lubomir and Maji, Subhransu and Malik, Jitendra},
	booktitle=ICCV,
	year={2011}
}


@inproceedings{aljundi2016expert,
	title={Expert Gate: Lifelong Learning with a Network of Experts},
	author={Aljundi, Rahaf and Chakravarty, Punarjay and Tuytelaars, Tinne},
	booktitle=ARXIV,
	year={2016}
}

@inproceedings{rannen2017encoder,
	title={Encoder based lifelong learning},
	author={Rannen Ep Triki, Amal and Aljundi, Rahaf and Blaschko, Matthew and Tuytelaars, Tinne},
	booktitle=ICCV,
	year={2017}
}
@inproceedings{catastrophic,
	title={Catastrophic forgetting in connectionist networks},
	author={French, Robert M},
	booktitle={Trends in cognitive sciences},
	year={1999},
}

@inproceedings{lwf,
	title={Learning without forgetting},
	author={Li, Zhizhong and Hoiem, Derek},
	booktitle=PAMI,
	year={2017}
}

@inproceedings{ewc,
	title={Overcoming catastrophic forgetting in neural networks},
	author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
	booktitle={Proceedings of the National Academy of Sciences},
	volume={114},
	number={13},
	pages={3521--3526},
	year={2017},
	publisher={National Acad Sciences}
}

@inproceedings{incremental-detector,
	title={Incremental Learning of Object Detectors without Catastrophic Forgetting},
	author={Shmelkov, Konstantin and Schmid, Cordelia and Alahari, Karteek},
	booktitle=ICCV,
	year={2017}
}

@inproceedings{ewc-moment,
	title={Overcoming catastrophic forgetting by incremental moment matching},
	author={Lee, Sang-Woo and Kim, Jin-Hwa and Jun, Jaehyun and Ha, Jung-Woo and Zhang, Byoung-Tak},
	booktitle={Advances in Neural Information Processing Systems},
	pages={4655--4665},
	year={2017}
}
@inproceedings{distilling,
	title={Distilling the knowledge in a neural network},
	author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
	booktitle=NIPS,
	year={2014}
}







@inproceedings{thrun1996learning,
	title={Is learning the n-th thing any easier than learning the first?},
	author={Thrun, Sebastian},
	booktitle=NIPS,
	year={1996}
}

@inproceedings{schlimmer1986case,
	title={A case study of incremental concept induction},
	author={Schlimmer, Jeffrey C and Fisher, Douglas},
	booktitle=AAAI,
	volume={86},
	pages={496--501},
	year={1986}
}

@inproceedings{ristin2014incremental,
	title={Incremental learning of NCM forests for large-scale image classification},
	author={Ristin, Marko and Guillaumin, Matthieu and Gall, Juergen and Van Gool, Luc},
	booktitle=CVPR,
	pages={3654--3661},
	year={2014}
}

@inproceedings{buciluǎ2006model,
	title={Model compression},
	author={Buciluǎ, Cristian and Caruana, Rich and Niculescu-Mizil, Alexandru},
	booktitle={Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={535--541},
	year={2006},
	organization={ACM}
}

@inproceedings{tzeng2015simultaneous,
	title={Simultaneous deep transfer across domains and tasks},
	author={Tzeng, Eric and Hoffman, Judy and Darrell, Trevor and Saenko, Kate},
	booktitle=ICCV,
	pages={4068--4076},
	year={2015},
	organization={IEEE}
}

@inproceedings{gupta2016cross,
	title={Cross modal distillation for supervision transfer},
	author={Gupta, Saurabh and Hoffman, Judy and Malik, Jitendra},
	booktitle=CVPR,
	pages={2827--2836},
	year={2016},
	organization={IEEE}
}

@inproceedings{goodfellow2013empirical,
	title={An empirical investigation of catastrophic forgetting in gradient-based neural networks},
	author={Goodfellow, Ian J and Mirza, Mehdi and Xiao, Da and Courville, Aaron and Bengio, Yoshua},
	booktitle={ARXIV preprint ARXIV:1312.6211},
	year={2013}
}

@inproceedings{french1994dynamically,
	title={Dynamically constraining connectionist networks to produce distributed, orthogonal representations to reduce catastrophic interference},
	author={French, Robert M},
	booktitle={network},
	volume={1111},
	pages={00001},
	year={1994},
	publisher={Citeseer}
}

@inproceedings{lecun1989backpropagation,
	title={Backpropagation applied to handwritten zip code recognition},
	author={LeCun, Yann and Boser, Bernhard and Denker, John S and Henderson, Donnie and Howard, Richard E and Hubbard, Wayne and Jackel, Lawrence D},
	booktitle={Neural computation},
	volume={1},
	number={4},
	pages={541--551},
	year={1989},
	publisher={MIT Press}
}

@inproceedings{ans2004self,
	title={Self-refreshing memory in artificial neural networks: Learning temporal sequences without catastrophic forgetting},
	author={Ans, Bernard and Rousset, St{\'e}phane and French, Robert M and Musca, Serban},
	booktitle={Connection Science},
	volume={16},
	number={2},
	pages={71--99},
	year={2004},
	publisher={Taylor \& Francis}
}


@inproceedings{torralba2011unbiased,
	title={Unbiased look at dataset bias},
	author={Torralba, Antonio and Efros, Alexei A},
	booktitle={Computer Vision and Pattern Recognition (CVPR), 2011 IEEE Conference on},
	pages={1521--1528},
	year={2011},
	organization={IEEE}
}

@inproceedings{icarl,
	title={icarl: Incremental classifier and representation learning},
	author={Rebuffi, Sylvestre-Alvise and Kolesnikov, Alexander and Sperl, Georg and Lampert, Christoph H},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{pnn,
	title={Progressive Neural Networks},
	author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
	booktitle=NIPS,
	year={2016}
}

@inproceedings{pathnet,
	title={Pathnet: Evolution channels gradient descent in super neural networks},
	author={Fernando, Chrisantha and Banarse, Dylan and Blundell, Charles and Zwols, Yori and Ha, David and Rusu, Andrei A and Pritzel, Alexander and Wierstra, Daan},
	booktitle={ARXIV preprint ARXIV:1701.08734},
	year={2017}
}

@inproceedings{road,
	title={ROAD: Reality oriented adaptation for semantic segmentation of urban scenes},
	author={Chen, Yuhua and Li, Wen and Van Gool, Luc},
	booktitle=CVPR,
	pages={7892--7901},
	year={2018}
}

@inproceedings{fcnwild,
	title={Fcns in the wild: Pixel-level adversarial and constraint-based adaptation},
	author={Hoffman, Judy and Wang, Dequan and Yu, Fisher and Darrell, Trevor},
	booktitle={ARXIV preprint ARXIV:1612.02649},
	year={2016}
}

@inproceedings{saito2017maximum,
	title={Maximum classifier discrepancy for unsupervised domain adaptation},
	author={Saito, Kuniaki and Watanabe, Kohei and Ushiku, Yoshitaka and Harada, Tatsuya},
	booktitle=CVPR,
	volume={3},
	year={2017}
}


@inproceedings{tsai2018learning,
	title={Learning to adapt structured output space for semantic segmentation},
	author={Tsai, Yi-Hsuan and Hung, Wei-Chih and Schulter, Samuel and Sohn, Kihyuk and Yang, Ming-Hsuan and Chandraker, Manmohan},
	booktitle=CVPR,
	year={2017}
}


@inproceedings{referseg,
	author = {Li, Ruiyu and Li, Kaican and Kuo, Yi-Chun and Shu, Michelle and Qi, Xiaojuan and Shen, Xiaoyong and Jia, Jiaya},
	title = {Referring Image Segmentation via Recurrent Refinement Networks},
	booktitle = CVPR,
	month = {June},
	year = {2018}
}

@inproceedings{ris,
	title={Recurrent Instance Segmentation},
	author={Romera-Paredes, Bernardino and Torr, Philip Hilaire Sean},
	booktitle=ECCV,
	pages={312--329},
	year={2016},
	organization={Springer}
}

@inproceedings{liu2018rotate,
	title={Rotate your Networks: Better Weight Consolidation and Less Catastrophic Forgetting},
	author={Liu, Xialei and Masana, Marc and Herranz, Luis and Van de Weijer, Joost and Lopez, Antonio M and Bagdanov, Andrew D},
	booktitle=ICPR,
	year={2018}
}




@inproceedings{yolo9000,
	title={YOLO9000: better, faster, stronger},
	author={Redmon, Joseph and Farhadi, Ali},
	booktitle={ARXIV preprint},
	year={2017}
}

@inproceedings{retinanet,
	title={Focal loss for dense object detection},
	author={Lin, Tsung-Yi and Goyal, Priyal and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
	booktitle=PAMI,
	year={2018},
	publisher={IEEE}
}

@inproceedings{ionet,
	title={Inside-outside net: Detecting objects in context with skip pooling and recurrent neural networks},
	author={Bell, Sean and Lawrence Zitnick, C. and Bala, Kavita and Girshick, Ross},
	booktitle=CVPR,
	pages={2874--2883},
	year={2016}
}




@inproceedings{rcnn,
	title={Rich feature hierarchies for accurate object detection and semantic segmentation},
	author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={580--587},
	year={2014}
}

@inproceedings{selectivesearch,
	title={Selective search for object recognition},
	author={Uijlings, Jasper RR and Van De Sande, Koen EA and Gevers, Theo and Smeulders, Arnold WM},
	booktitle=IJCV,
	volume={104},
	number={2},
	pages={154--171},
	year={2013},
	publisher={Springer}
}

@inproceedings{sppnet,
	title={Spatial pyramid pooling in deep convolutional networks for visual recognition},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=ECCV,
	year={2014},
}


@inproceedings{deformable,
	title={Deformable convolutional networks},
	author={Dai, Jifeng and Qi, Haozhi and Xiong, Yuwen and Li, Yi and Zhang, Guodong and Hu, Han and Wei, Yichen},
	booktitle={ARXIV},
	year={2017}
}



@inproceedings{kantorov2016contextlocnet,
	title={Contextlocnet: Context-aware deep network models for weakly supervised localization},
	author={Kantorov, Vadim and Oquab, Maxime and Cho, Minsu and Laptev, Ivan},
	booktitle=ECCV,
	pages={350--365},
	year={2016},
	organization={Springer}
}




@inproceedings{bai2017multiple,
	title={Multiple instance detection network with online instance classifier refinement},
	author={Bai, Peng Tang Xinggang Wang Xiang and Liu, Wenyu},
	year={2017}
}

@inproceedings{tang2016large,
	title={Large scale semi-supervised object detection using visual and semantic knowledge transfer},
	author={Tang, Yuxing and Wang, Josiah and Gao, Boyang and Dellandr{\'e}a, Emmanuel and Gaizauskas, Robert and Chen, Liming},
	booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
	pages={2119--2128},
	year={2016}
}

@inproceedings{kumar2016track,
	title={Track and transfer: Watching videos to simulate strong human supervision for weakly-supervised object detection},
	author={Kumar Singh, Krishna and Xiao, Fanyi and Jae Lee, Yong},
	booktitle=CVPR,
	pages={3548--3556},
	year={2016}
}



@inproceedings{yosinski2014transferable,
	title={How transferable are features in deep neural networks?},
	author={Yosinski, Jason and Clune, Jeff and Bengio, Yoshua and Lipson, Hod},
	booktitle=NIPS,
	pages={3320--3328},
	year={2014}
}

@article{hyvarinen2005estimation,
  title={Estimation of non-normalized statistical models by score matching.},
  author={Hyv{\"a}rinen, Aapo and Dayan, Peter},
  journal={Journal of Machine Learning Research},
  volume={6},
  number={4},
  year={2005}
}

@article{anderson1982reverse,
  title={Reverse-time diffusion equation models},
  author={Anderson, Brian DO},
  journal={Stochastic Processes and their Applications},
  volume={12},
  number={3},
  pages={313--326},
  year={1982},
  publisher={Elsevier}
}

@article{zheng2023improved,
  title={Improved Techniques for Maximum Likelihood Estimation for Diffusion ODEs},
  author={Zheng, Kaiwen and Lu, Cheng and Chen, Jianfei and Zhu, Jun},
  journal={arXiv preprint arXiv:2305.03935},
  year={2023}
}
@article{song2019generative,
	title        = {Generative modeling by estimating gradients of the data distribution},
	author       = {Song, Yang and Ermon, Stefano},
	year         = 2019,
	journal      = {arXiv}
}

@book{ambrosio2005gradient,
	address = {Boston},
	series = {Lectures in mathematics {ETH} {Zürich}},
	title = {Gradient flows: in metric spaces and in the space of probability measures},
	isbn = {978-3-7643-2428-5},
	shorttitle = {Gradient flows},
	language = {en},
	publisher = {Birkhäuser},
	author = {Ambrosio, Luigi and Gigli, Nicola and Savaré, Giuseppe},
	year = {2005},
}

@inproceedings{donahue2014decaf,
	title={Decaf: A deep convolutional activation feature for generic visual recognition},
	author={Donahue, Jeff and Jia, Yangqing and Vinyals, Oriol and Hoffman, Judy and Zhang, Ning and Tzeng, Eric and Darrell, Trevor},
	booktitle=ICML,
	year={2014}
}

@inproceedings{liang2015towards,
	title={Towards computational baby learning: A weakly-supervised approach for object detection},
	author={Liang, Xiaodan and Liu, Si and Wei, Yunchao and Liu, Luoqi and Lin, Liang and Yan, Shuicheng},
	booktitle=CVPR,
	pages={999--1007},
	year={2015}
}


@inproceedings{gong2023diffpose,
  title={Diffpose: Toward more reliable 3d pose estimation},
  author={Gong, Jia and Foo, Lin Geng and Fan, Zhipeng and Ke, Qiuhong and Rahmani, Hossein and Liu, Jun},
  booktitle=CVPR,
  year={2023}
}

@inproceedings{bilen2015weakly,
	title={Weakly supervised object detection with convex clustering},
	author={Bilen, Hakan and Pedersoli, Marco and Tuytelaars, Tinne},
	booktitle=CVPR,
	pages={1081--1089},
	year={2015}
}

@article{amit2021segdiff,
  title={Segdiff: Image segmentation with diffusion probabilistic models},
  author={Amit, Tomer and Shaharbany, Tal and Nachmani, Eliya and Wolf, Lior},
  journal={arXiv preprint arXiv:2112.00390},
  year={2021}
}

@inproceedings{fss_diff,
         title={Beyond Generation: Exploring Generalization of Diffusion Models in Few-shot Segmentation},
        author={Jie Liu and Tao HU and Jan jakob Sonke and Efstratios Gavves},
          year={2023},
          booktitle={NeurIPS Diffusion Workshop},
      }

@inproceedings{laina2020quantifying,
  title={Quantifying learnability and describability of visual concepts emerging in representation learning},
  author={Laina, Iro and Fong, Ruth and Vedaldi, Andrea},
  booktitle={NeurIPS},
  year={2020}
}

@article{jiang2023object,
  title={Object-centric slot diffusion},
  author={Jiang, Jindong and Deng, Fei and Singh, Gautam and Ahn, Sungjin},
  journal={arXiv},
  year={2023}
}

@article{chen2022diffusiondet,
  title={Diffusiondet: Diffusion model for object detection},
  author={Chen, Shoufa and Sun, Peize and Song, Yibing and Luo, Ping},
  journal={arXiv preprint arXiv:2211.09788},
  year={2022}
}

@article{wu2023slotdiffusion,
  title={SlotDiffusion: Object-Centric Generative Modeling with Diffusion Models},
  author={Wu, Ziyi and Hu, Jingyu and Lu, Wuyue and Gilitschenski, Igor and Garg, Animesh},
  journal={arXiv preprint arXiv:2305.11281},
  year={2023}
}

@article{holmquist2022diffpose,
  title={Diffpose: Multi-hypothesis human pose estimation using diffusion models},
  author={Holmquist, Karl and Wandt, Bastian},
  journal={arXiv},
  year={2022}
}


@article{zhang2023tale,
  title={A Tale of Two Features: Stable Diffusion Complements DINO for Zero-Shot Semantic Correspondence},
  author={Zhang, Junyi and Herrmann, Charles and Hur, Junhwa and Cabrera, Luisa Polania and Jampani, Varun and Sun, Deqing and Yang, Ming-Hsuan},
  journal={arXiv preprint arXiv:2305.15347},
  year={2023}
}



@article{qiu2023learning,
  title={Learning Structure-Guided Diffusion Model for 2D Human Pose Estimation},
  author={Qiu, Zhongwei and Yang, Qiansheng and Wang, Jian and Wang, Xiyu and Xu, Chang and Fu, Dongmei and Yao, Kun and Han, Junyu and Ding, Errui and Wang, Jingdong},
  journal={arXiv},
  year={2023}
}


@article{li2023your,
  title={Your diffusion model is secretly a zero-shot classifier},
  author={Li, Alexander C and Prabhudesai, Mihir and Duggal, Shivam and Brown, Ellis and Pathak, Deepak},
  journal={arXiv preprint arXiv:2303.16203},
  year={2023}
}
@article{karazija2023diffusion,
  title={Diffusion Models for Zero-Shot Open-Vocabulary Segmentation},
  author={Karazija, Laurynas and Laina, Iro and Vedaldi, Andrea and Rupprecht, Christian},
  journal={arXiv preprint arXiv:2306.09316},
  year={2023}
}

@article{du2023protodiff,
  title={ProtoDiff: Learning to Learn Prototypical Networks by Task-Guided Diffusion},
  author={Du, Yingjun and Xiao, Zehao and Liao, Shengcai and Snoek, Cees},
  journal={arXiv preprint arXiv:2306.14770},
  year={2023}
}


@article{mukhopadhyay2023diffusion_classification,
  title={Diffusion Models Beat GANs on Image Classification},
  author={Mukhopadhyay, Soumik and Gwilliam, Matthew and Agarwal, Vatsal and Padmanabhan, Namitha and Swaminathan, Archana and Hegde, Srinidhi and Zhou, Tianyi and Shrivastava, Abhinav},
  journal=Arxiv,
  year={2023}
}

@article{you2023diffusion_semi,
  title={Diffusion models and semi-supervised learners benefit mutually with few labels},
  author={You, Zebin and Zhong, Yong and Bao, Fan and Sun, Jiacheng and Li, Chongxuan and Zhu, Jun},
  journal={NeurIPS},
  year={2023}
}


@inproceedings{li2016weakly,
	title={Weakly supervised object localization with progressive domain adaptation},
	author={Li, Dong and Huang, Jia-Bin and Li, Yali and Wang, Shengjin and Yang, Ming-Hsuan},
	booktitle=CVPR,
	pages={3512--3520},
	year={2016}
}

@inproceedings{ren2018meta,
	title={Meta-learning for semi-supervised few-shot classification},
	author={Ren, Mengye and Triantafillou, Eleni and Ravi, Sachin and Snell, Jake and Swersky, Kevin and Tenenbaum, Joshua B and Larochelle, Hugo and Zemel, Richard S},
	booktitle={ARXIV preprint ARXIV:1803.00676},
	year={2018}
}

@inproceedings{garcia2017few,
	title={Few-shot learning with graph neural networks},
	author={Garcia, Victor and Bruna, Joan},
	booktitle={ARXIV preprint ARXIV:1711.04043},
	year={2017}
}

@InProceedings{Razavian_2014_CVPR_Workshops,
	author = {Sharif Razavian, Ali and Azizpour, Hossein and Sullivan, Josephine and Carlsson, Stefan},
	title = {CNN Features Off-the-Shelf: An Astounding Baseline for Recognition},
	booktitle = CVPRW,
	year = {2014}
}







@inproceedings{enet,
	title={ENet: A Deep Neural Network Architecture for Real-Time Semantic Segmentation},
	author={Paszke, Adam and Chaurasia, Abhishek and Kim, Sangpil and Culurciello, Eugenio},
	booktitle={ARXIV preprint ARXIV:1606.02147},
	year={2016}
}


@inproceedings{adelaide,
	title={Efficient piecewise training of deep structured models for semantic segmentation},
	author={Lin, Guosheng and Shen, Chunhua and Van Den Hengel, Anton and Reid, Ian},
	booktitle=CVPR,
	year={2016}
}


@inproceedings{erfnet,
	title={ERFNet: Efficient Residual Factorized ConvNet for Real-Time Semantic Segmentation},
	author={Romera, Eduardo and Alvarez, Jos{\'e} M and Bergasa, Luis M and Arroyo, Roberto},
	booktitle={IEEE Transactions on Intelligent Transportation Systems},
	year={2018}
}


@inproceedings{frrn,
	title={Full-Resolution Residual Networks for Semantic Segmentation in Street Scenes},
	author={Pohlen, Tobias and Hermans, Alexander and Mathias, Markus and Leibe, Bastian},
	booktitle=CVPR,
	year={2017}
}

@inproceedings{lrr,
	title={Laplacian pyramid reconstruction and refinement for semantic segmentation},
	author={Ghiasi, Golnaz and Fowlkes, Charless C},
	booktitle=ECCV,
	year={2016},
}



@inproceedings{gori2005new,
	title={A new model for learning in graph domains},
	author={Gori, Marco and Monfardini, Gabriele and Scarselli, Franco},
	booktitle=IJCNN,
	year={2005},
}

@inproceedings{scarselli2009graph,
	title={The graph neural network model},
	author={Scarselli, Franco and Gori, Marco and Tsoi, Ah Chung and Hagenbuchner, Markus and Monfardini, Gabriele},
	booktitle={IEEE Transactions on Neural Networks},
	year={2009},
}

@inproceedings{li2015gated,
	title={Gated graph sequence neural networks},
	author={Li, Yujia and Tarlow, Daniel and Brockschmidt, Marc and Zemel, Richard},
	booktitle={ARXIV},
	year={2015}
}

@inproceedings{sukhbaatar2016learning,
	title={Learning multiagent communication with backpropagation},
	author={Sukhbaatar, Sainbayar and Fergus, Rob and others},
	booktitle=NIPS,
	year={2016}
}


@inproceedings{duvenaud2015convolutional,
	title={Convolutional networks on graphs for learning molecular fingerprints},
	author={Duvenaud, David K and Maclaurin, Dougal and Iparraguirre, Jorge and Bombarell, Rafael and Hirzel, Timothy and Aspuru-Guzik, Al{\'a}n and Adams, Ryan P},
	booktitle=NIPS,
	year={2015}
}


@inproceedings{bruna2017community,
	title={Community detection with graph neural networks},
	author={Bruna, Joan and Li, Xiang},
	booktitle={ARXIV},
	year={2017}
}

















@inproceedings{wang2015relaxed,
  title={Relaxed multiple-instance SVM with application to object discovery},
  author={Wang, Xinggang and Zhu, Zhuotun and Yao, Cong and Bai, Xiang},
  booktitle=ICCV,
  year={2015}
}










@inproceedings{jie2017deep,
  title={Deep self-taught learning for weakly supervised object localization},
  author={Jie, Zequn and Wei, Yunchao and Jin, Xiaojie and Feng, Jiashi and Liu, Wei},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{tang2017multiple,
  title={Multiple instance detection network with online instance classifier refinement},
  author={Tang, Peng and Wang, Xinggang and Bai, Xiang and Liu, Wenyu},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{wang2014weakly,
  title={Weakly supervised object localization with latent category learning},
  author={Wang, Chong and Ren, Weiqiang and Huang, Kaiqi and Tan, Tieniu},
  booktitle=ECCV,
  year={2014},
}



@inproceedings{yu15lsun,
    Author = {Yu, Fisher and Zhang, Yinda and Song, Shuran and Seff, Ari and Xiao, Jianxiong},
    Title = {LSUN: Construction of a Large-scale Image Dataset using Deep Learning with Humans in the Loop},
    booktitle = {ARXIV},
    Year = {2015}
}

@inproceedings{vo2021large,
  title={Large-scale unsupervised object discovery},
  author={Vo, Van Huy and Sizikova, Elena and Schmid, Cordelia and P{\'e}rez, Patrick and Ponce, Jean},
  booktitle=NIPS,
  year={2021}
}
@inproceedings{vo2020toward,
  title={Toward unsupervised, multi-object discovery in large-scale image collections},
  author={Vo, Huy V and P{\'e}rez, Patrick and Ponce, Jean},
  booktitle=ECCV,
  year={2020},
}


@inproceedings{rolfe2016discrete,
  title={Discrete variational autoencoders},
  author={Rolfe, Jason Tyler},
  booktitle=ICLR,
  year={2017}
}

@inproceedings{gao2021large,
  title={Large-scale Unsupervised Semantic Segmentation},
  author={Gao, Shang-Hua and Li, Zhong-Yu and Yang, Ming-Hsuan and Cheng, Ming-Ming and Han, Junwei and Torr, Philip},
  booktitle={ARXIV},
  year={2021}
}

@inproceedings{panteli2021sparse,
  title={Sparse-shot Learning with Exclusive Cross-Entropy for Extremely Many Localisations},
  author={Panteli, Andreas and Teuwen, Jonas and Horlings, Hugo and Gavves, Efstratios},
  booktitle=ICCV,
  year={2021}
}

@inproceedings{hoogeboom2022equivariant,
  title={Equivariant diffusion for molecule generation in 3d},
  author={Hoogeboom, Emiel and Satorras, V{\i}́ctor Garcia and Vignac, Cl{\'e}ment and Welling, Max},
  booktitle=ICML,
  year={2022}
}
@article{zhou2111lafite,
  title={LAFITE: Towards Language-Free Training for Text-to-Image Generation. arXiv 2021},
  author={Zhou, Y and Zhang, R and Chen, C and Li, C and Tensmeyer, C and Yu, T and Gu, J and Xu, J and Sun, T},
  journal={arXiv}
}

@inproceedings{mittal2021symbolic,
  title={Symbolic music generation with diffusion models},
  author={Mittal, Gautam and Engel, Jesse and Hawthorne, Curtis and Simon, Ian},
  booktitle={ISMIR},
  year={2021}
}
@inproceedings{ziegler2022self,
  title={Self-Supervised Learning of Object Parts for Semantic Segmentation},
  author={Ziegler, Adrian and Asano, Yuki M},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{jing2020self,
  title={Self-supervised visual feature learning with deep neural networks: A survey},
  author={Jing, Longlong and Tian, Yingli},
  booktitle=PAMI,
  year={2020}
}

@inproceedings{ge2021evaluation,
  title={Evaluation of various open-set medical imaging tasks with deep neural networks},
  author={Ge, Zongyuan and Wang, Xin},
  booktitle={ARXIV},
  year={2021}
}

@inproceedings{bogdoll2022anomaly,
  title={Anomaly detection in autonomous driving: A survey},
  author={Bogdoll, Daniel and Nitsche, Maximilian and Z{\"o}llner, J Marius},
  booktitle={CVPR},
  year={2022}
}

@inproceedings{jain2022completr,
  title={ComplETR: Reducing the cost of annotations for object detection in dense scenes with vision transformers},
  author={Jain, Achin and Lee, Kibok and Swaminathan, Gurumurthy and Yang, Hao and Schiele, Bernt and Ravichandran, Avinash and Dabeer, Onkar},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{zheng2022towards,
  title={Towards open-set object detection and discovery},
  author={Zheng, Jiyang and Li, Weihao and Hong, Jie and Petersson, Lars and Barnes, Nick},
  booktitle={CVPR},
  year={2022}
}


@inproceedings{li2020analyzing,
  title={Analyzing overfitting under class imbalance in neural networks for image segmentation},
  author={Li, Zeju and Kamnitsas, Konstantinos and Glocker, Ben},
  booktitle={IEEE Transactions on Medical Imaging},
  year={2020},
}

@inproceedings{wang2022tokencut,
  title={TokenCut: Segmenting Objects in Images and Videos with Self-supervised Transformer and Normalized Cut},
  author={Wang, Yangtao and Shen, Xi and Yuan, Yuan and Du, Yuming and Li, Maomao and Hu, Shell Xu and Crowley, James L and Vaufreydaz, Dominique},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{amir2021deep_dino_coseg,
  title={Deep vit features as dense visual descriptors},
  author={Amir, Shir and Gandelsman, Yossi and Bagon, Shai and Dekel, Tali},
  booktitle={ARXIV},
  year={2021}
}

@inproceedings{mirza2014conditional_cgan,
  title={Conditional generative adversarial nets},
  author={Mirza, Mehdi and Osindero, Simon},
  booktitle={ARXIV},
  year={2014}
}

@inproceedings{srivastava2017veegan,
  title={Veegan: Reducing mode collapse in gans using implicit variational learning},
  author={Srivastava, Akash and Valkov, Lazar and Russell, Chris and Gutmann, Michael U and Sutton, Charles},
  booktitle=NIPS,
  year={2017}
}

@inproceedings{yu2020inclusive,
  title={Inclusive gan: Improving data and minority coverage in generative models},
  author={Yu, Ning and Li, Ke and Zhou, Peng and Malik, Jitendra and Davis, Larry and Fritz, Mario},
  booktitle=ECCV,
  year={2020},
}

@inproceedings{zhang2022motiondiffuse,
  title={MotionDiffuse: Text-Driven Human Motion Generation with Diffusion Model},
  author={Zhang, Mingyuan and Cai, Zhongang and Pan, Liang and Hong, Fangzhou and Guo, Xinying and Yang, Lei and Liu, Ziwei},
  booktitle={ARXIV preprint ARXIV:2208.15001},
  year={2022}
}

@inproceedings{esser2020disentangling,
  title={A disentangling invertible interpretation network for explaining latent representations},
  author={Esser, Patrick and Rombach, Robin and Ommer, Bjorn},
  booktitle=CVPR,
  year={2020}
}

@inproceedings{kingma2016improved,
  title={Improved variational inference with inverse autoregressive flow},
  author={Kingma, Durk P and Salimans, Tim and Jozefowicz, Rafal and Chen, Xi and Sutskever, Ilya and Welling, Max},
  booktitle=NIPS,
  year={2016}
}



@inproceedings{carion2020end_detr,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle=ECCV,
  year={2020}
}

@inproceedings{he2020momentum_moco,
  title={Momentum contrast for unsupervised visual representation learning},
  author={He, Kaiming and Fan, Haoqi and Wu, Yuxin and Xie, Saining and Girshick, Ross},
  booktitle=CVPR,
  year={2020}
}



@inproceedings{donahue2016adversarial,
  title={Adversarial feature learning},
  author={Donahue, Jeff and Kr{\"a}henb{\"u}hl, Philipp and Darrell, Trevor},
  booktitle=ICLR,
  year={2017}
}

@inproceedings{morozov2020self,
  title={On self-supervised image representations for GAN evaluation},
  author={Morozov, Stanislav and Voynov, Andrey and Babenko, Artem},
  booktitle=ICLR,
  year={2020}
}

@inproceedings{donahue2019large_bigbigan,
  title={Large scale adversarial representation learning},
  author={Donahue, Jeff and Simonyan, Karen},
  booktitle=NIPS,
  year={2019}
}

@inproceedings{melas2022deep,
  title={Deep Spectral Methods: A Surprisingly Strong Baseline for Unsupervised Semantic Segmentation and Localization},
  author={Melas-Kyriazi, Luke and Rupprecht, Christian and Laina, Iro and Vedaldi, Andrea},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{song2021solving,
  title={Solving inverse problems in medical imaging with score-based generative models},
  author={Song, Yang and Shen, Liyue and Xing, Lei and Ermon, Stefano},
  booktitle=ICLR,
  year={2022}
}

@inproceedings{yang2022diffusion,
  title={Diffusion probabilistic modeling for video generation},
  author={Yang, Ruihan and Srivastava, Prakhar and Mandt, Stephan},
  booktitle={ARXIV},
  year={2022}
}


@inproceedings{wang2022semantic,
  title={Semantic image synthesis via diffusion models},
  author={Wang, Weilun and Bao, Jianmin and Zhou, Wengang and Chen, Dongdong and Chen, Dong and Yuan, Lu and Li, Houqiang},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{bordes2021high,
  title={High Fidelity Visualization of What Your Self-Supervised Representation Knows About},
  author={Bordes, Florian and Balestriero, Randall and Vincent, Pascal},
  booktitle={TMLR},
  year={2022}
}

@inproceedings{asano2019selflabelling,
  title={Self-labelling via simultaneous clustering and representation learning},
  author={Asano, Yuki Markus and Rupprecht, Christian and Vedaldi, Andrea},
  booktitle=ICLR,
  year={2020}
}

@inproceedings{papamakarios2021normalizing,
  title={Normalizing Flows for Probabilistic Modeling and Inference.},
  author={Papamakarios, George and Nalisnick, Eric T and Rezende, Danilo Jimenez and Mohamed, Shakir and Lakshminarayanan, Balaji},
  booktitle={JMLR},
  year={2021}
}

@inproceedings{kobyzev2020normalizing,
  title={Normalizing flows: An introduction and review of current methods},
  author={Kobyzev, Ivan and Prince, Simon JD and Brubaker, Marcus A},
  booktitle=PAMI,
  year={2020},
}


@inproceedings{caron2020unsupervised_swap,
  title={Unsupervised learning of visual features by contrasting cluster assignments},
  author={Caron, Mathilde and Misra, Ishan and Mairal, Julien and Goyal, Priya and Bojanowski, Piotr and Joulin, Armand},
  booktitle=NIPS,
  year={2020}
}



@inproceedings{luvcic2019high,
  title={High-fidelity image generation with fewer labels},
  author={Lu{\v{c}}i{\'c}, Mario and Tschannen, Michael and Ritter, Marvin and Zhai, Xiaohua and Bachem, Olivier and Gelly, Sylvain},
  booktitle=ICML,
  year={2019}
}


@inproceedings{zhou2021lafite,
  title={Lafite: Towards language-free training for text-to-image generation},
  author={Zhou, Yufan and Zhang, Ruiyi and Chen, Changyou and Li, Chunyuan and Tensmeyer, Chris and Yu, Tong and Gu, Jiuxiang and Xu, Jinhui and Sun, Tong},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{behrmann2021understanding,
  title={Understanding and mitigating exploding inverses in invertible neural networks},
  author={Behrmann, Jens and Vicol, Paul and Wang, Kuan-Chieh and Grosse, Roger and Jacobsen, J{\"o}rn-Henrik},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  year={2021}
}

@inproceedings{razavi2019preventing,
  title={Preventing posterior collapse with delta-vaes},
  author={Razavi, Ali and Oord, A{\"a}ron van den and Poole, Ben and Vinyals, Oriol},
  booktitle={ARXIV preprint ARXIV:1901.03416},
  year={2019}
}

@inproceedings{dinh2016density_realnvp,
  title={Density estimation using real nvp},
  author={Dinh, Laurent and Sohl-Dickstein, Jascha and Bengio, Samy},
  booktitle=ICLR,
  year={2017}
}

@inproceedings{vincent2011connection,
  title={A connection between score matching and denoising autoencoders},
  author={Vincent, Pascal},
  booktitle={Neural computation},
  year={2011}
}

@inproceedings{radford2021learning_clip,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle=ICML,
  year={2021},
}

@inproceedings{kingma2018glow,
  title={Glow: Generative flow with invertible 1x1 convolutions},
  author={Kingma, Durk P and Dhariwal, Prafulla},
  booktitle=NIPS,
  year={2018}
}

@inproceedings{rezende2015variational,
  title={Variational inference with normalizing flows},
  author={Rezende, Danilo and Mohamed, Shakir},
  booktitle=ICML,
  year={2015},
}

@inproceedings{rezende2014stochastic,
  title={Stochastic backpropagation and approximate inference in deep generative models},
  author={Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
  booktitle=ICML,
  year={2014},
}


@inproceedings{kingma2013auto_vae,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  booktitle=ICLR,
  year={2014}
}



@inproceedings{loshchilov2017decoupled_adamw,
  title={Decoupled weight decay regularization},
  author={Loshchilov, Ilya and Hutter, Frank},
  booktitle=ICLR,
  year={2019}
}


@inproceedings{dosovitskiy2020image_vit,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  booktitle=ICLR,
  year={2021}
}

@inproceedings{caesar2018_cocostuff,
  title={Coco-stuff: Thing and stuff classes in context},
  author={Caesar, Holger and Uijlings, Jasper and Ferrari, Vittorio},
  booktitle=CVPR,
  year={2018}
}

@inproceedings{zhang2022dense_dsn,
  title={Dense Siamese Network},
  author={Zhang, Wenwei and Pang, Jiangmiao and Chen, Kai and Loy, Chen Change},
  booktitle=ECCV,
  year={2022}
}

@inproceedings{ji2019invariant_iic,
  title={Invariant information clustering for unsupervised image classification and segmentation},
  author={Ji, Xu and Henriques, Joao F and Vedaldi, Andrea},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{cho2021picie,
  title={Picie: Unsupervised semantic segmentation using invariance and equivariance in clustering},
  author={Cho, Jang Hyun and Mall, Utkarsh and Bala, Kavita and Hariharan, Bharath},
  booktitle=CVPR,
  year={2021}
}


@inproceedings{krahenbuhl2011efficient_crf,
  title={Efficient inference in fully connected crfs with gaussian edge potentials},
  author={Kr{\"a}henb{\"u}hl, Philipp and Koltun, Vladlen},
  booktitle=NIPS,
  year={2011}
}
@inproceedings{barratt2018note,
  title={A note on the inception score},
  author={Barratt, Shane and Sharma, Rishi},
  booktitle={ARXIV},
  year={2018}
}

@inproceedings{parmar2021cleanfid,
  title={On Aliased Resizing and Surprising Subtleties in GAN Evaluation},
  author={Parmar, Gaurav and Zhang, Richard and Zhu, Jun-Yan},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{im2020fast_noisyclustering2,
  title={Fast noise removal for k-means clustering},
  author={Im, Sungjin and Qaem, Mahshid Montazer and Moseley, Benjamin and Sun, Xiaorui and Zhou, Rudy},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  year={2020}
}

@inproceedings{dave1991characterization_noisyclustering,
  title={Characterization and detection of noise in clustering},
  author={Dave, Rajesh N},
  booktitle={Pattern Recognition Letters},
  year={1991}
}

@inproceedings{last2017oversampling,
  title={Oversampling for imbalanced learning based on k-means and smote},
  author={Last, Felix and Douzas, Georgios and Bacao, Fernando},
  booktitle={ARXIV},
  year={2017}
}

@inproceedings{assran2022masked_msn,
  title={Masked siamese networks for label-efficient learning},
  author={Assran, Mahmoud and Caron, Mathilde and Misra, Ishan and Bojanowski, Piotr and Bordes, Florian and Vincent, Pascal and Joulin, Armand and Rabbat, Michael and Ballas, Nicolas},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{karras2019_stylegan,
  title={A style-based generator architecture for generative adversarial networks},
  author={Karras, Tero and Laine, Samuli and Aila, Timo},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{zhang2017split,
  title={Split-brain autoencoders: Unsupervised learning by cross-channel prediction},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A},
  booktitle=CVPR,
  year={2017}
}

@inproceedings{vincent2008extracting,
  title={Extracting and composing robust features with denoising autoencoders},
  author={Vincent, Pascal and Larochelle, Hugo and Bengio, Yoshua and Manzagol, Pierre-Antoine},
  booktitle=ICML,
  year={2008}
}
@inproceedings{gidaris2018unsupervised_rotate,
  title={Unsupervised representation learning by predicting image rotations},
  author={Gidaris, Spyros and Singh, Praveer and Komodakis, Nikos},
  booktitle=ICLR,
  year={2018}
}

@inproceedings{brock2018large_biggan,
  title={Large scale GAN training for high fidelity natural image synthesis},
  author={Brock, Andrew and Donahue, Jeff and Simonyan, Karen},
  booktitle=ICLR,
  year={2019}
}

@inproceedings{van2021revisiting,
  title={Revisiting contrastive methods for unsupervised learning of visual representations},
  author={Van Gansbeke, Wouter and Vandenhende, Simon and Georgoulis, Stamatios and Gool, Luc V},
  booktitle=NIPS,
  year={2021}
}


@inproceedings{lu2021soft_quadratic2,
  title={SOFT: softmax-free transformer with linear complexity},
  author={Lu, Jiachen and Yao, Jinghan and Zhang, Junge and Zhu, Xiatian and Xu, Hang and Gao, Weiguo and Xu, Chunjing and Xiang, Tao and Zhang, Li},
  booktitle=NIPS,
  year={2021}
}

@inproceedings{purushwalkam2020demystifying,
  title={Demystifying contrastive self-supervised learning: Invariances, augmentations and dataset biases},
  author={Purushwalkam, Senthil and Gupta, Abhinav},
  booktitle=NIPS,
  year={2020}
}

@inproceedings{he2019rethinking,
  title={Rethinking imagenet pre-training},
  author={He, Kaiming and Girshick, Ross and Doll{\'a}r, Piotr},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{giannone2022_fewshot,
  title={Few-Shot Diffusion Models},
  author={Giannone, Giorgio and Nielsen, Didrik and Winther, Ole},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{katharopoulos2020transformers_quadratic,
  title={Transformers are rnns: Fast autoregressive transformers with linear attention},
  author={Katharopoulos, Angelos and Vyas, Apoorv and Pappas, Nikolaos and Fleuret, Fran{\c{c}}ois},
  booktitle=ICML,
  year={2020}
}

@inproceedings{chen2020big_simclr_v2,
  title={Big self-supervised models are strong semi-supervised learners},
  author={Chen, Ting and Kornblith, Simon and Swersky, Kevin and Norouzi, Mohammad and Hinton, Geoffrey E},
  booktitle=NIPS,
  year={2020}
}

@inproceedings{ali2021xcit,
  title={Xcit: Cross-covariance image transformers},
  author={Ali, Alaaeldin and Touvron, Hugo and Caron, Mathilde and Bojanowski, Piotr and Douze, Matthijs and Joulin, Armand and Laptev, Ivan and Neverova, Natalia and Synnaeve, Gabriel and Verbeek, Jakob and others},
  booktitle=NIPS,
  year={2021}
}

@inproceedings{armandpour2021partition,
  title={Partition-guided gans},
  author={Armandpour, Mohammadreza and Sadeghian, Ali and Li, Chunyuan and Zhou, Mingyuan},
  booktitle=CVPR,
  year={2021}
}

@inproceedings{mangla2022data,
  title={Data instance prior (disp) in generative adversarial networks},
  author={Mangla, Puneet and Kumari, Nupur and Singh, Mayank and Krishnamurthy, Balaji and Balasubramanian, Vineeth N},
  booktitle=WACV,
  year={2022}
}

@inproceedings{chen2019self,
  title={Self-supervised gans via auxiliary rotation loss},
  author={Chen, Ting and Zhai, Xiaohua and Ritter, Marvin and Lucic, Mario and Houlsby, Neil},
  booktitle=CVPR,
  year={2019}
}




@inproceedings{everingham2010pascal_voc,
  title={The pascal visual object classes (voc) challenge},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  booktitle=IJCV,
  year={2010}
}


@inproceedings{salimans2016improved_is_inceptionscore,
  title={Improved techniques for training gans},
  author={Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi},
  booktitle=NIPS,
  year={2016}
}

@inproceedings{szegedy2016rethinking_inceptionv3,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle=CVPR,
  year={2016}
}

@misc{obukhov2020torchfidelity,
  author={Anton Obukhov and Maximilian Seitzer and Po-Wei Wu and Semen Zhydenko and Jonathan Kyl and Elvis Yu-Jing Lin},
  year=2020,
  title={High-fidelity performance metrics for generative models in PyTorch},
  url={https://github.com/toshas/torch-fidelity},
  publisher={Zenodo},
}

@inproceedings{heusel2017gans_fid,
  title={Gans trained by a two time-scale update rule converge to a local nash equilibrium},
  author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
  booktitle=NIPS,
  year={2017}
}


@inproceedings{song2020denoising_ddim,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  booktitle=ICLR,
  year={2021}
}

@inproceedings{johnson2019billion_faiss,
  title={Billion-scale similarity search with {GPUs}},
  author={Johnson, Jeff and Douze, Matthijs and J{\'e}gou, Herv{\'e}},
  booktitle={IEEE Transactions on Big Data},
  year={2019}
}

@inproceedings{hamilton2022unsupervised_stego,
  title={Unsupervised Semantic Segmentation by Distilling Feature Correspondences},
  author={Hamilton, Mark and Zhang, Zhoutong and Hariharan, Bharath and Snavely, Noah and Freeman, William T},
  booktitle=ICLR,
  year={2022}
}

@inproceedings{simeoni2021localizing_lost,
  title={Localizing objects with self-supervised transformers and no labels},
  author={Sim{\'e}oni, Oriane and Puy, Gilles and Vo, Huy V and Roburin, Simon and Gidaris, Spyros and Bursuc, Andrei and P{\'e}rez, Patrick and Marlet, Renaud and Ponce, Jean},
  booktitle=BMVC,
  year={2021}
}

@inproceedings{meng2021sdedit,
  title={Sdedit: Guided image synthesis and editing with stochastic differential equations},
  author={Meng, Chenlin and He, Yutong and Song, Yang and Song, Jiaming and Wu, Jiajun and Zhu, Jun-Yan and Ermon, Stefano},
  booktitle=ICLR,
  year={2021}
}

@inproceedings{lugmayr2022repaint,
  title={Repaint: Inpainting using denoising diffusion probabilistic models},
  author={Lugmayr, Andreas and Danelljan, Martin and Romero, Andres and Yu, Fisher and Timofte, Radu and Van Gool, Luc},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{choi2021ilvr,
  title={Ilvr: Conditioning method for denoising diffusion probabilistic models},
  author={Choi, Jooyoung and Kim, Sungwon and Jeong, Yonghyun and Gwon, Youngjune and Yoon, Sungroh},
  booktitle=ICCV,
  year={2021}
}

@inproceedings{liu2022compositional_diff,
  title={Compositional Visual Generation with Composable Diffusion Models},
  author={Liu, Nan and Li, Shuang and Du, Yilun and Torralba, Antonio and Tenenbaum, Joshua B},
  booktitle=ECCV,
  year={2022}
}

@article{caron2022location,
  title={Location-Aware Self-Supervised Transformers},
  author={Caron, Mathilde and Houlsby, Neil and Schmid, Cordelia},
  journal={arXiv},
  year={2022}
}

@inproceedings{DSSIDERen2019DeepRS,
  title={Deep Robust Single Image Depth Estimation Neural Network Using Scene Understanding},
  author={Haoyu Ren and Mostafa El-Khamy and Jungwon Lee},
  booktitle={CVPR Workshops},
  year={2019}
}

@article{pokle2023training_imageinversion_fm,
  title={Training-free Linear Image Inversion via Flows},
  author={Pokle, Ashwini and Muckley, Matthew J and Chen, Ricky TQ and Karrer, Brian},
  journal={arXiv},
  year={2023}
}

@inproceedings{lu2022dpmsolver,
  title={Dpm-solver: A fast ode solver for diffusion probabilistic model sampling in around 10 steps},
  author={Lu, Cheng and Zhou, Yuhao and Bao, Fan and Chen, Jianfei and Li, Chongxuan and Zhu, Jun},
  journal={NeurIPS},
  year={2022}
}

@inproceedings{tong2023improving_alex,
  title={Improving and generalizing flow-based generative models with minibatch optimal transport},
  author={Tong, Alexander and Malkin, Nikolay and Huguet, Guillaume and Zhang, Yanlei and Rector-Brooks, Jarrid and Fatras, Kilian and Wolf, Guy and Bengio, Yoshua},
  booktitle={ICML Workshop on New Frontiers in Learning, Control, and Dynamical Systems},
  year={2023}
}

@inproceedings{li2022bigdatasetgan,
  title={BigDatasetGAN: Synthesizing ImageNet with Pixel-wise Annotations},
  author={Li, Daiqing and Ling, Huan and Kim, Seung Wook and Kreis, Karsten and Fidler, Sanja and Torralba, Antonio},
  booktitle=CVPR,
  year={2022}
}

@article{dao2023flow_lfm,
  title={Flow matching in latent space},
  author={Dao, Quan and Phung, Hao and Nguyen, Binh and Tran, Anh},
  journal={arXiv},
  year={2023}
}

@article{he2021sosd,
  title={SOSD-Net: Joint semantic object segmentation and depth estimation from monocular images},
  author={He, Lei and Lu, Jiwen and Wang, Guanghui and Song, Shiyu and Zhou, Jie},
  journal={Neurocomputing},
  year={2021}
}

@inproceedings{wu2023fast,
  title={Fast Point Cloud Generation with Straight Flows},
  author={Wu, Lemeng and Wang, Dilin and Gong, Chengyue and Liu, Xingchao and Xiong, Yunyang and Ranjan, Rakesh and Krishnamoorthi, Raghuraman and Chandra, Vikas and Liu, Qiang},
  booktitle=CVPR,
  year={2023}
}

@article{dormand1980family,
  title={A family of embedded Runge-Kutta formulae},
  author={Dormand, John R and Prince, Peter J},
  journal={Journal of computational and applied mathematics},
  year={1980},
}

@article{lee2023minimizing,
  title={Minimizing Trajectory Curvature of ODE-based Generative Models},
  author={Lee, Sangyun and Kim, Beomsu and Ye, Jong Chul},
  journal=ICML,
  year={2023}
}

@inproceedings{zhang2021datasetgan,
  title={Datasetgan: Efficient labeled data factory with minimal human effort},
  author={Zhang, Yuxuan and Ling, Huan and Gao, Jun and Yin, Kangxue and Lafleche, Jean-Francois and Barriuso, Adela and Torralba, Antonio and Fidler, Sanja},
  booktitle=CVPR,
  year={2021}
}


@inproceedings{chen2020simple_simclr,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle=ICML,
  year={2020},
}

@inproceedings{he2022masked_mae,
  title={Masked autoencoders are scalable vision learners},
  author={He, Kaiming and Chen, Xinlei and Xie, Saining and Li, Yanghao and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{lyu2021conditional,
  title={A conditional point diffusion-refinement paradigm for 3d point cloud completion},
  author={Lyu, Zhaoyang and Kong, Zhifeng and Xu, Xudong and Pan, Liang and Lin, Dahua},
  booktitle=ICLR,
  year={2021}
}
@inproceedings{luo2021diffusion,
  title={Diffusion probabilistic models for 3d point cloud generation},
  author={Luo, Shitong and Hu, Wei},
  booktitle=CVPR,
  year={2021}
}

@inproceedings{saharia2022photorealistic_imagen,
  title={Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding},
  author={Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily and Ghasemipour, Seyed Kamyar Seyed and Ayan, Burcu Karagol and Mahdavi, S Sara and Lopes, Rapha Gontijo and others},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{dhariwal2021diffusion_beat,
  title={Diffusion models beat gans on image synthesis},
  author={Dhariwal, Prafulla and Nichol, Alexander},
  booktitle=NIPS,
  year={2021}
}

@inproceedings{kong2020diffwave,
  title={Diffwave: A versatile diffusion model for audio synthesis},
  author={Kong, Zhifeng and Ping, Wei and Huang, Jiaji and Zhao, Kexin and Catanzaro, Bryan},
  booktitle=ICLR,
  year={2020}
}

@inproceedings{chen2020wavegrad,
  title={WaveGrad: Estimating gradients for waveform generation},
  author={Chen, Nanxin and Zhang, Yu and Zen, Heiga and Weiss, Ron J and Norouzi, Mohammad and Chan, William},
  booktitle=ICLR,
  year={2021}
}

@inproceedings{
  song2021scorebased_sde,
  title={Score-Based Generative Modeling through Stochastic Differential Equations},
  author={Yang Song and Jascha Sohl-Dickstein and Diederik P Kingma and Abhishek Kumar and Stefano Ermon and Ben Poole},
  booktitle=ICLR,
  year={2021}
}

@inproceedings{ho2022video,
  title={Video diffusion models},
  author={Ho, Jonathan and Salimans, Tim and Gritsenko, Alexey and Chan, William and Norouzi, Mohammad and Fleet, David J},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{nichol2021glide,
  title={Glide: Towards photorealistic image generation and editing with text-guided diffusion models},
  author={Nichol, Alex and Dhariwal, Prafulla and Ramesh, Aditya and Shyam, Pranav and Mishkin, Pamela and McGrew, Bob and Sutskever, Ilya and Chen, Mark},
   booktitle=ICML,
  year={2022}
}


@inproceedings{ramesh2022hierarchical_dalle2,
  title={Hierarchical text-conditional image generation with clip latents},
  author={Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{ramesh2021zero_dalle1,
  title={Zero-shot text-to-image generation},
  author={Ramesh, Aditya and Pavlov, Mikhail and Goh, Gabriel and Gray, Scott and Voss, Chelsea and Radford, Alec and Chen, Mark and Sutskever, Ilya},
  booktitle=ICML,
  year={2021},
}

@inproceedings{ashual2022knn,
  title={Knn-diffusion: Image generation via large-scale retrieval},
  author={Ashual, Oron and Sheynin, Shelly and Polyak, Adam and Singer, Uriel and Gafni, Oran and Nachmani, Eliya and Taigman, Yaniv},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{blattmann2022retrieval,
  title={Retrieval-Augmented Diffusion Models},
  author={Blattmann, Andreas and Rombach, Robin and Oktay, Kaan and Ommer, Bj{\"o}rn},
  booktitle={ARXIV},
  year={2022}
}

@inproceedings{dino,
  title={Emerging Properties in Self-Supervised Vision Transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J\'egou, Herv\'e  and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  booktitle=ICCV,
  year={2021}
}

@inproceedings{icgan,
  title={Instance-conditioned gan},
  author={Casanova, Arantxa and Careil, Marlene and Verbeek, Jakob and Drozdzal, Michal and Romero Soriano, Adriana},
  booktitle=NIPS,
  year={2021}
}

@inproceedings{ho2021classifier,
  title={Classifier-free diffusion guidance},
  author={Ho, Jonathan and Salimans, Tim},
  booktitle={NeurIPS  Workshop},
  year={2021}
}


@inproceedings{preechakul2022diffusion_autoencoder,
  title={Diffusion autoencoders: Toward a meaningful and decodable representation},
  author={Preechakul, Konpat and Chatthee, Nattanat and Wizadwongsa, Suttisak and Suwajanakorn, Supasorn},
  booktitle=CVPR,
  year={2022}
}

@inproceedings{sinha2021d2c,
  title={D2c: Diffusion-decoding models for few-shot conditional generation},
  author={Sinha, Abhishek and Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  booktitle=NIPS,
  year={2021}
}


@inproceedings{karras2022elucidating,
  title={Elucidating the Design Space of Diffusion-Based Generative Models},
  author={Karras, Tero and Aittala, Miika and Aila, Timo and Laine, Samuli},
  booktitle={NeurIPS},
  year={2022}
}


@inproceedings{kingma2021variational,
  title={Variational diffusion models},
  author={Kingma, Diederik and Salimans, Tim and Poole, Ben and Ho, Jonathan},
  booktitle={NeurIPS},
  year={2021}
}

@inproceedings{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  booktitle={ARXIV},
  year={2009},
}

@inproceedings{laina2020quantifying,
  title={Quantifying learnability and describability of visual concepts emerging in representation learning},
  author={Laina, Iro and Fong, Ruth and Vedaldi, Andrea},
  booktitle={NeurIPS},
  year={2020}
}


@inproceedings{ganea_hyperbolic_2018,
	title = {Hyperbolic {Entailment} {Cones} for {Learning} {Hierarchical} {Embeddings}},
	url = {https://proceedings.mlr.press/v80/ganea18a.html},
	abstract = {Learning graph representations via low-dimensional embeddings that preserve relevant network properties is an important class of problems in machine learning. We here present a novel method to embed directed acyclic graphs. Following prior work, we first advocate for using hyperbolic spaces which provably model tree-like structures better than Euclidean geometry. Second, we view hierarchical relations as partial orders defined using a family of nested geodesically convex cones. We prove that these entailment cones admit an optimal shape with a closed form expression both in the Euclidean and hyperbolic spaces, and they canonically define the embedding learning process. Experiments show significant improvements of our method over strong recent baselines both in terms of representational capacity and generalization.},
	language = {en},
	urldate = {2023-03-02},
	booktitle = {Proceedings of the 35th {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Ganea, Octavian and Becigneul, Gary and Hofmann, Thomas},
	month = jul,
	year = {2018},
	note = {ISSN: 2640-3498},
	pages = {1646--1655},
	file = {Full Text PDF:/Users/longteng/Zotero/storage/CC6VF9N9/Ganea et al. - 2018 - Hyperbolic Entailment Cones for Learning Hierarchi.pdf:application/pdf;Supplementary PDF:/Users/longteng/Zotero/storage/NP976BSH/Ganea et al. - 2018 - Hyperbolic Entailment Cones for Learning Hierarchi.pdf:application/pdf},
}



@inproceedings{mathieu_continuous_2019,
	title = {Continuous {Hierarchical} {Representations} with {Poincaré} {Variational} {Auto}-{Encoders}},
	volume = {32},
	url = {https://proceedings.neurips.cc/paper/2019/hash/0ec04cb3912c4f08874dd03716f80df1-Abstract.html},
	abstract = {The Variational Auto-Encoder (VAE)  is a popular method for learning a generative model and embeddings of the data. Many real datasets are hierarchically structured. However, traditional VAEs map data in a Euclidean latent space which cannot efficiently embed tree-like structures. Hyperbolic spaces with negative curvature can. We therefore endow VAEs with a Poincaré ball model of hyperbolic geometry as a latent space and rigorously derive the necessary methods to work with two main Gaussian generalisations on that space. We empirically show better generalisation to unseen data than the Euclidean counterpart, and can qualitatively and quantitatively better recover hierarchical structures.},
	urldate = {2023-09-12},
	booktitle = {Advances in {Neural} {Information} {Processing} {Systems}},
	publisher = {Curran Associates, Inc.},
	author = {Mathieu, Emile and Le Lan, Charline and Maddison, Chris J. and Tomioka, Ryota and Teh, Yee Whye},
	year = {2019},
	file = {Full Text PDF:/Users/longteng/Zotero/storage/SUWMB7KX/Mathieu et al. - 2019 - Continuous Hierarchical Representations with Poinc.pdf:application/pdf},
}




@article{sinkhorn1967concerning,
  title={Concerning nonnegative matrices and doubly stochastic matrices},
  author={Sinkhorn, Richard and Knopp, Paul},
  journal={Pacific Journal of Mathematics},
  volume={21},
  number={2},
  pages={343--348},
  year={1967},
  publisher={Mathematical Sciences Publishers}
}


% ------------------ DATASETS -------------------------- %
@inproceedings{roberts2021hypersim,
    author    = {Mike Roberts AND Jason Ramapuram AND Anurag Ranjan AND Atulit Kumar AND
                 Miguel Angel Bautista AND Nathan Paczan AND Russ Webb AND Joshua M. Susskind},
    title     = {{Hypersim}: {A} Photorealistic Synthetic Dataset for Holistic Indoor Scene Understanding},
    booktitle = {ICCV},
    year      = {2021}
}

@article{diode_dataset,
  title={{DIODE}: {A} {D}ense {I}ndoor and {O}utdoor {DE}pth {D}ataset},
  author={Igor Vasiljevic and Nick Kolkin and Shanyi Zhang and Ruotian Luo and
  Haochen Wang and Falcon Z. Dai and Andrea F. Daniele and Mohammadreza Mostajabi and
  Steven Basart and Matthew R. Walter and Gregory Shakhnarovich},
  journal={CoRR},
  year={2019}
}

@inproceedings{silberman12nyuv2,
  author    = {Nathan Silberman, Derek Hoiem, Pushmeet Kohli and Rob Fergus},
  title     = {Indoor Segmentation and Support Inference from RGBD Images},
  booktitle = {ECCV},
  year      = {2012}
}

@inproceedings{packnetDDAD,
  author = {Vitor Guizilini and Rares Ambrus and Sudeep Pillai and Allan Raventos and Adrien Gaidon},
  title = {3D Packing for Self-Supervised Monocular Depth Estimation},
  booktitle = {CVPR},
  year = {2020},
}

@misc{cho2021dimlcvl,
      title={DIML/CVL RGB-D Dataset: 2M RGB-D Images of Natural Indoor and Outdoor Scenes}, 
      author={Jaehoon Cho and Dongbo Min and Youngjung Kim and Kwanghoon Sohn},
      year={2021},
 booktitle = {Arxiv},   
}

@article{koch2020ibims-1,
	author = {Koch, Tobias and Liebel, Lukas and Körner, Marco and Fraundorfer, Friedrich},
	title = {Comparison of monocular depth estimation methods using geometrically relevant metrics on the IBims-1 dataset},
	journal = {Computer Vision and Image Understanding (CVIU)},
	year = {2020}
}

@article{zhou2014learning,
  title={Learning deep features for scene recognition using places database},
  author={Zhou, Bolei and Lapedriza, Agata and Xiao, Jianxiong and Torralba, Antonio and Oliva, Aude},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}




@inproceedings{NEURIPS2019_bdbca288,
 author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {8026--8037},
 publisher = {Curran Associates, Inc.},
 title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
 url = {https://proceedings.neurips.cc/paper/2019/file/bdbca288fee7f92f2bfa9f7012727740-Paper.pdf},
 volume = {32},
 year = {2019}
}

@inproceedings{Loshchilov2019DecoupledWD,
  title={Decoupled Weight Decay Regularization},
  author={I. Loshchilov and F. Hutter},
  booktitle={ICLR},
  year={2019}
}

@article{DBLP:journals/corr/abs-1708-07120,
  author    = {Leslie N. Smith and
               Nicholay Topin},
  title     = {Super-Convergence: Very Fast Training of Residual Networks Using Large
               Learning Rates},
  journal   = {CoRR},
  volume    = {abs/1708.07120},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.07120},
  archivePrefix = {arXiv},
  eprint    = {1708.07120},
  timestamp = {Mon, 13 Aug 2018 16:48:13 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-07120.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{tensorflow2015-whitepaper,
title={ {TensorFlow}: Large-Scale Machine Learning on Heterogeneous Systems},
url={https://www.tensorflow.org/},
note={Software available from tensorflow.org},
author={
    Mart\'{\i}n~Abadi and
    Ashish~Agarwal and
    Paul~Barham and
    Eugene~Brevdo and
    Zhifeng~Chen and
    Craig~Citro and
    Greg~S.~Corrado and
    Andy~Davis and
    Jeffrey~Dean and
    Matthieu~Devin and
    Sanjay~Ghemawat and
    Ian~Goodfellow and
    Andrew~Harp and
    Geoffrey~Irving and
    Michael~Isard and
    Yangqing Jia and
    Rafal~Jozefowicz and
    Lukasz~Kaiser and
    Manjunath~Kudlur and
    Josh~Levenberg and
    Dandelion~Man\'{e} and
    Rajat~Monga and
    Sherry~Moore and
    Derek~Murray and
    Chris~Olah and
    Mike~Schuster and
    Jonathon~Shlens and
    Benoit~Steiner and
    Ilya~Sutskever and
    Kunal~Talwar and
    Paul~Tucker and
    Vincent~Vanhoucke and
    Vijay~Vasudevan and
    Fernanda~Vi\'{e}gas and
    Oriol~Vinyals and
    Pete~Warden and
    Martin~Wattenberg and
    Martin~Wicke and
    Yuan~Yu and
    Xiaoqiang~Zheng},
  year={2015},
}

@article{Bianco2018,
  title={Benchmark Analysis of Representative Deep Neural Network Architectures},
  author={Simone Bianco and R{\'e}mi Cad{\`e}ne and Luigi Celona and Paolo Napoletano},
  journal={IEEE Access},
  year={2018},
  volume={6},
  pages={64270-64277}
}

@article{Cao2018,
  title={Stabilized real-time face tracking via a learned dynamic rigidity prior},
  author={Chen Cao and Menglei Chai and Oliver J. Woodford and Linjie Luo},
  journal={ACM Trans. Graph.},
  year={2018},
  volume={37},
  pages={233:1-233:11}
}

@article{Cubuk2018AutoAugmentLA,
  title={AutoAugment: Learning Augmentation Policies from Data},
  author={Ekin Dogus Cubuk and Barret Zoph and Dandelion Man{\'e} and Vijay Vasudevan and Quoc V. Le},
  journal={CoRR},
  year={2018},
  volume={abs/1805.09501}
}

@article{Deng2009,
  title={ImageNet: A large-scale hierarchical image database},
  author={Jia Deng and Wei Dong and Richard Socher and Li-Jia Li and Kai Li and Li Fei-Fei},
  journal={2009 IEEE Conference on Computer Vision and Pattern Recognition},
  year={2009},
  pages={248-255}
}

@article{Dosovitskiy2015,
  title={FlowNet: Learning Optical Flow with Convolutional Networks},
  author={Philipp Fischer and Alexey Dosovitskiy and Eddy Ilg and Philip H{\"a}usser and Caner Hazirbas and Vladimir Golkov and Patrick van der Smagt and Daniel Cremers and Thomas Brox},
  journal={2015 IEEE International Conference on Computer Vision (ICCV)},
  year={2015},
  pages={2758-2766}
}

@inproceedings{Eigen2014,
  title={Depth Map Prediction from a Single Image using a Multi-Scale Deep Network},
  author={David Eigen and Christian Puhrsch and Rob Fergus},
  booktitle={NIPS},
  year={2014}
}

@misc{UnrealMarket2018,
  title={{Marketplace - UE4 Marketplace}},
  author={{Epic Games, Inc.}},
  url={https://www.unrealengine.com/marketplace/store},
  year={2018}
}

@article{Fu2018DeepOR,
  title={Deep Ordinal Regression Network for Monocular Depth Estimation},
  author={Huan Fu and Mingming Gong and Chaohui Wang and Nematollah Batmanghelich and Dacheng Tao},
  journal={CVPR},
  year={2018}
}

@article{geiger2013vision,
  title={Vision meets robotics: The KITTI dataset},
  author={Andreas Geiger and Philip Lenz and Christoph Stiller and Raquel Urtasun},
  journal={I. J. Robotics Res.},
  year={2013}
}

@inproceedings{glorot2010understanding,
  title={Understanding the difficulty of training deep feedforward neural networks},
  author={Xavier Glorot and Yoshua Bengio},
  booktitle={AISTATS},
  year={2010}
}

@article{Godard2017,
  title={Unsupervised Monocular Depth Estimation with Left-Right Consistency},
  author={Cl{\'e}ment Godard and Oisin Mac Aodha and Gabriel J. Brostow},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={6602-6611}
}

@article{Godard2018DiggingIS,
  title={Digging Into Self-Supervised Monocular Depth Estimation},
  author={Cl{\'e}ment Godard and Oisin Mac Aodha and Gabriel J. Brostow},
  journal={CoRR},
  year={2018},
  volume={abs/1806.01260}
}

@InProceedings{Watson_2021_CVPR,
    author    = {Watson, Jamie and Mac Aodha, Oisin and Prisacariu, Victor and Brostow, Gabriel and Firman, Michael},
    title     = {The Temporal Opportunist: Self-Supervised Multi-Frame Monocular Depth},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2021},
    pages     = {1164-1174}
}


@inproceedings{Zhou2021Diffnet,
    title={Self-Supervised Monocular Depth Estimation with Internal Feature Fusion},
    author={Zhou, Hang and Greenwood, David and Taylor, Sarah},
    booktitle={British Machine Vision Conference (BMVC)},
    year={2021}
    }



@article{Hao2018DetailPD,
  title={Detail Preserving Depth Estimation from a Single Image Using Attention Guided Networks},
  author={Zhixiang Hao and Yu Li and Shaodi You and Feng Lu},
  journal={2018 International Conference on 3D Vision (3DV)},
  year={2018},
  pages={304-313}
}


@inproceedings{Hazirbas2016FuseNetID,
  title={FuseNet: Incorporating Depth into Semantic Segmentation via Fusion-Based CNN Architecture},
  author={Caner Hazirbas and Lingni Ma and Csaba Domokos and Daniel Cremers},
  booktitle={ACCV},
  year={2016}
}

@article{Hedman2018,
  title={Instant 3D photography},
  author={Peter Hedman and Johannes Kopf},
  journal={ACM Trans. Graph.},
  year={2018},
  volume={37},
  pages={101:1-101:12}
}

@article{huang2017densely,
  title={Densely Connected Convolutional Networks},
  author={Gao Huang and Zhuang Liu and Laurens van der Maaten and Kilian Q. Weinberger},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={2261-2269}
}

@article{Huang2018DeepMVSLM,
  title={DeepMVS: Learning Multi-view Stereopsis},
  author={Po-Han Huang and Kevin Matzen and Johannes Kopf and Narendra Ahuja and Jia-Bin Huang},
  journal={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2018},
  pages={2821-2830}
}

@inproceedings{Ioffe2015BNA,
  title={Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift},
  author={Sergey Ioffe and Christian Szegedy},
  booktitle={ICML},
  year={2015}
}

@inproceedings{jlb2015adam,
  author    = {Diederik P. Kingma and Jimmy Ba},
  title     = {{Adam: {A} Method for Stochastic Optimization}},
  booktitle = {Proceedings of the 3rd International Conference on Learning Representations (ICLR)},
  year      = {2015},
  journal   = {Proceedings of the 3rd International Conference on Learning Representations (ICLR)},
}

@inproceedings{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097-1105},
  year={2012}
}

@article{Kuznietsov2017,
  title={Semi-Supervised Deep Learning for Monocular Depth Map Prediction},
  author={Yevhen Kuznietsov and J{\"o}rg St{\"u}ckler and Bastian Leibe},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={2215-2223}
}

@article{Laina2016,
  title={Deeper Depth Prediction with Fully Convolutional Residual Networks},
  author={Iro Laina and Christian Rupprecht and Vasileios Belagiannis and Federico Tombari and Nassir Navab},
  journal={2016 Fourth International Conference on 3D Vision (3DV)},
  year={2016},
  pages={239-248}
}

@article{Lee2011,
  title={Depth-assisted real-time 3D object detection for augmented reality},
  author={Lee, Wonwoo and Park, Nohyoung and Woo, Woontack},
  journal={ICAT’11},
  volume={2},
  pages={126-132},
  year={2011}
}


@inproceedings{LehtinenMHLKAA18,
  title = 	 {{N}oise2{N}oise: Learning Image Restoration without Clean Data},
  author = 	 {Lehtinen, Jaakko and Munkberg, Jacob and Hasselgren, Jon and Laine, Samuli and Karras, Tero and Aittala, Miika and Aila, Timo},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {2965--2974},
  year = 	 {2018},
  editor = 	 {Dy, Jennifer and Krause, Andreas},
  volume = 	 {80},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Stockholmsmässan, Stockholm Sweden},
  month = 	 {10--15 Jul},
  publisher = 	 {PMLR}
}

@article{Levin2004,
  title={Colorization using optimization},
  author={Anat Levin and Dani Lischinski and Yair Weiss},
  journal={ACM Trans. Graph.},
  year={2004},
  volume={23},
  pages={689-694}
}

@article{Li2015,
  title={Depth and surface normal estimation from monocular images using regression on deep features and hierarchical CRFs},
  author={Bo Li and Chunhua Shen and Yuchao Dai and Anton van den Hengel and Mingyi He},
  journal={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2015},
  pages={1119-1127}
}

@inproceedings{Maas13LeRELU,
  title={Rectifier nonlinearities improve neural network acoustic models},
  author={Maas, Andrew L and Hannun, Awni Y and Ng, Andrew Y},
  booktitle={Proc. icml},
  volume={30},
  issue={1},
  pages={3},
  year={2013}
}

@article{moreno2007active,
 author = {Moreno-Noguer, Francesc and Belhumeur, Peter N. and Nayar, Shree K.},
 title = {Active Refocusing of Images and Videos},
 journal = {ACM Trans. Graph.},
 issue_date = {July 2007},
 volume = {26},
 number = {3},
 month = jul,
 year = {2007},
 issn = {0730-0301},
 articleno = {67},
 url = {http://doi.acm.org/10.1145/1276377.1276461},
 doi = {10.1145/1276377.1276461},
 acmid = {1276461},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {active illumination, computational photography, depth from defocus, depth of field, image segmentation, refocusing},
} 

@inproceedings{Ronneberger2015u,
 author="Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas",
 title="U-Net: Convolutional Networks for Biomedical Image Segmentation",
 booktitle="Medical Image Computing and Computer-Assisted Intervention -- MICCAI 2015",
 year={2015},
 publisher="Springer International Publishing",
 address="Cham",
 pages="234--241",
 isbn="978-3-319-24574-4"
}

@article{Sobel1968,
  title={A 3x3 Isotropic Gradient Operator for Image Processing. Stanford Artificial Intelligence Project},
  author={Sobel, I},
  year={1968},
  journal={SAIL}
}

@article{Ummenhofer2017,
  title={DeMoN: Depth and Motion Network for Learning Monocular Stereo},
  author={Benjamin Ummenhofer and Huizhong Zhou and Jonas Uhrig and Nikolaus Mayer and Eddy Ilg and Alexey Dosovitskiy and Thomas Brox},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={5622-5631}
}

@article{Wang2018,
  title={DeepLens: shallow depth of field from a single image},
  author={Lijun Wang and Xiaohui Shen and Jianming Zhang and Oliver Wang and Zhe L. Lin and Chih-Yao Hsieh and Sarah Kong and Huchuan Lu},
  journal={ACM Trans. Graph.},
  year={2018},
  volume={37},
  pages={245:1-245:11}
}

@article{Wang2004SSIM,
  title={Image quality assessment: from error visibility to structural similarity},
  author={Jiheng Wang and Alan C. Bovik and Hamid R. Sheikh and Eero P. Simoncelli},
  journal={IEEE Transactions on Image Processing},
  year={2004},
  volume={13},
  pages={600-612}
}

@inproceedings{Wojna2017TheDI,
title	= {The Devil is in the Decoders},
author	= {Zbigniew Wojna and Vittorio Ferrari and Sergio Guadarrama and Nathan Silberman and Liang-chieh Chen and Alireza Fathi and Jasper Uijlings},
year	= {2017},
URL	= {https://arxiv.org/abs/1707.05847},
booktitle	= {BMVC}
}

@inproceedings{Xu2017,
  title={Multi-scale continuous crfs as sequential deep networks for monocular depth estimation},
  author={Xu, Dan and Ricci, Elisa and Ouyang, Wanli and Wang, Xiaogang and Sebe, Nicu},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5354--5362},
  year={2017}
}

@article{Xu2018StructuredAG,
  title={Structured Attention Guided Convolutional Neural Fields for Monocular Depth Estimation},
  author={Dong Xu and Wei Wang and Hao Tang and Hong W. Liu and Nicu Sebe and Elisa Ricci},
  journal={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2018},
  pages={3917-3925}
}

@article{Zamir2018TaskonomyDT,
  title={Taskonomy: Disentangling Task Transfer Learning},
  author={Amir Roshan Zamir and Alexander Sax and William B. Shen and Leonidas J. Guibas and Jitendra Malik and Silvio Savarese},
  journal={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2018},
  pages={3712-3722}
}

@inproceedings{Zhou2018DeepTAMDT,
  title={Deeptam: Deep tracking and mapping},
  author={Zhou, Huizhong and Ummenhofer, Benjamin and Brox, Thomas},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={822--838},
  year={2018}
}

@inproceedings{Xie2016Deep3DFA,
  title={Deep3D: Fully Automatic 2D-to-3D Video Conversion with Deep Convolutional Neural Networks},
  author={Junyuan Xie and Ross B. Girshick and Ali Farhadi},
  booktitle={ECCV},
  year={2016}
}

@article{Zhou2017,
  title={Unsupervised Learning of Depth and Ego-Motion from Video},
  author={Tinghui Zhou and Matthew R. Brown and Noah Snavely and David G. Lowe},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={6612-6619}
}

@article{Hu2018RevisitingSI,
  title={Revisiting Single Image Depth Estimation: Toward Higher Resolution Maps With Accurate Object Boundaries},
  author={Junjie Hu and Mete Ozay and Yan Zhang and Takayuki Okatani},
  journal={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  year={2018},
  pages={1043-1051}
}

@inproceedings{kopf2021rcvd,
 title={Robust Consistent Video Depth Estimation},
 author={Kopf, Johannes and Rong, Xuejian and Huang, Jia-Bin},
 year={2021},
 booktitle={IEEE/CVF Conference on Computer Vision and Pattern Recognition}
}

@inproceedings{MDLi18,
  	title={MegaDepth: Learning Single-View Depth Prediction from Internet Photos},
  	author={Zhengqi Li and Noah Snavely},
  	booktitle={Computer Vision and Pattern Recognition (CVPR)},
  	year={2018}
}

@article{Ranftl2020MiDaS,
	author    = {Ren\'{e} Ranftl and Katrin Lasinger and David Hafner and Konrad Schindler and Vladlen Koltun},
	title     = {Towards Robust Monocular Depth Estimation: Mixing Datasets for Zero-shot Cross-dataset Transfer},
	journal   = {TPAMI},
	year      = {2020},
}

@misc{birkl2023midas31,
      title={MiDaS v3.1 -- A Model Zoo for Robust Monocular Relative Depth Estimation}, 
      author={Reiner Birkl and Diana Wofk and Matthias Müller},
      year={2023},
      eprint={2307.14460},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@InProceedings{Ranftl_2021_ICCV_DPT,
    author    = {Ranftl, Ren\'e and Bochkovskiy, Alexey and Koltun, Vladlen},
    title     = {Vision Transformers for Dense Prediction},
    booktitle = {ICCV},
    year      = {2021}
}

@inproceedings{casser2019unsupervised,
  title={Unsupervised Monocular Depth and Ego-Motion Learning with Structure and Semantics},
  author={Casser, Vincent and Pirk, Soeren and Mahjourian, Reza and Angelova, Anelia},
  booktitle={CVPR Workshop on Visual Odometry and Computer Vision Applications Based on Location Cues (VOCVALC)},
  year={2019}
}
 
@inproceedings{atapour2018real,
  title={Real-time monocular depth estimation using synthetic data with domain adaptation via image style transfer},
  author={Atapour-Abarghouei, Amir and Breckon, Toby P},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2800--2810},
  year={2018}
}

@inproceedings{zhao2019geometry,
  title={Geometry-aware symmetric domain adaptation for monocular depth estimation},
  author={Zhao, Shanshan and Fu, Huan and Gong, Mingming and Tao, Dacheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9788--9798},
  year={2019}
}

@article{Tonioni2019,
  author    = {Alessio Tonioni and
               Matteo Poggi and
               Stefano Mattoccia and
               Luigi di Stefano},
  title     = {Unsupervised Domain Adaptation for Depth Prediction from Images},
  journal   = {CoRR},
  volume    = {abs/1909.03943},
  year      = {2019},
  url       = {http://arxiv.org/abs/1909.03943},
  archivePrefix = {arXiv},
  eprint    = {1909.03943},
  timestamp = {Tue, 17 Sep 2019 11:23:44 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1909-03943.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{CrDoCo2019,
  author    = {Chen, Yun-Chun and Lin, Yen-Yu and Yang, Ming-Hsuan and Huang, Jia-Bin}, 
  title     = {CrDoCo: Pixel-level Domain Transfer with Cross-Domain Consistency},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year      = {2019}
}

@article{kim2022global,
  title={Global-Local Path Networks for Monocular Depth Estimation with Vertical CutDepth},
  author={Kim, Doyeon and Ga, Woonghyun and Ahn, Pyungwhan and Joo, Donggyu and Chun, Sehwan and Kim, Junmo},
  journal={arXiv preprint arXiv:2201.07436},
  year={2022}
}

@ARTICLE{Yuan2022_cvpr_crf,
       author = {{Yuan}, Weihao and {Gu}, Xiaodong and {Dai}, Zuozhuo and {Zhu}, Siyu and {Tan}, Ping},
        title = "{NeW CRFs: Neural Window Fully-connected CRFs for Monocular Depth Estimation}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Computer Vision and Pattern Recognition},
         year = 2022,
        month = mar,
          eid = {arXiv:2203.01502},
        pages = {arXiv:2203.01502},
archivePrefix = {arXiv},
       eprint = {2203.01502},
 primaryClass = {cs.CV},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220301502Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@inproceedings{LoshchilovH19,
  author    = {Ilya Loshchilov and
               Frank Hutter},
  title     = {Decoupled Weight Decay Regularization},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/forum?id=Bkg6RiCqY7},
  timestamp = {Thu, 25 Jul 2019 14:26:04 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LoshchilovH19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{AkadaBAW22,
  author    = {Hiroyasu Akada and
               Shariq Farooq Bhat and
               Ibraheem Alhashim and
               Peter Wonka},
  title     = {Self-Supervised Learning of Domain Invariant Features for Depth Estimation},
  booktitle = {{IEEE/CVF} Winter Conference on Applications of Computer Vision, {WACV}
               2022, Waikoloa, HI, USA, January 3-8, 2022},
  pages     = {997--1007},
  publisher = {{IEEE}},
  year      = {2022},
  url       = {https://doi.org/10.1109/WACV51458.2022.00107},
  doi       = {10.1109/WACV51458.2022.00107},
  timestamp = {Thu, 17 Feb 2022 14:51:17 +0100},
  biburl    = {https://dblp.org/rec/conf/wacv/AkadaBAW22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Gordon_2019_ICCV,
    author = {Gordon, Ariel and Li, Hanhan and Jonschkowski, Rico and Angelova, Anelia},
    title = {Depth From Videos in the Wild: Unsupervised Monocular Depth Learning From Unknown Cameras},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month = {October},
    year = {2019}
}

@article{li2020unsupervised,
  title={Unsupervised Monocular Depth Learning in Dynamic Scenes},
  author={Li, Hanhan and Gordon, Ariel and Zhao, Hang and Casser, Vincent and Angelova, Anelia},
  journal={arXiv preprint arXiv:2010.16404},
  year={2020}
}

% ResNet
@article{He2016DeepRL,
  title={Deep Residual Learning for Image Recognition},
  author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
  journal={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2016},
  pages={770-778}
}

% ResNet V2
@inproceedings{He2016IdentityMI,
  title={Identity Mappings in Deep Residual Networks},
  author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
  booktitle={ECCV},
  year={2016}
}

% ResNext
@article{Xie2017AggregatedRT,
  title={Aggregated Residual Transformations for Deep Neural Networks},
  author={Saining Xie and Ross B. Girshick and Piotr Doll{\'a}r and Zhuowen Tu and Kaiming He},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={5987-5995}
}

% NASNet
@article{Zoph2018LearningTA,
  title={Learning Transferable Architectures for Scalable Image Recognition},
  author={Barret Zoph and Vijay Vasudevan and Jonathon Shlens and Quoc V. Le},
  journal={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  year={2018},
  pages={8697-8710}
}

% Xception
@article{Chollet2017XceptionDL,
  title={Xception: Deep Learning with Depthwise Separable Convolutions},
  author={François Chollet},
  journal={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  pages={1800-1807}
}

% VGG
@article{Simonyan2015VeryDC,
  title={Very Deep Convolutional Networks for Large-Scale Image Recognition},
  author={Karen Simonyan and Andrew Zisserman},
  journal={CoRR},
  year={2015},
  volume={abs/1409.1556}
}

% BTS
@article{bts_lee2019big,
  title={From big to small: Multi-scale local planar guidance for monocular depth estimation},
  author={Lee, Jin Han and Han, Myung-Kyu and Ko, Dong Wook and Suh, Il Hong},
  journal={arXiv preprint arXiv:1907.10326},
  year={2019}
}

% Ren 
@InProceedings{Ren_2019_CVPR_Workshops,
author = {Ren, Haoyu and El-khamy, Mostafa and Lee, Jungwon},
title = {Deep Robust Single Image Depth Estimation Neural Network Using Scene Understanding},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
month = {June},
year = {2019}
}

@InProceedings{Zhang_2019_CVPR,
author = {Zhang, Zhenyu and Cui, Zhen and Xu, Chunyan and Yan, Yan and Sebe, Nicu and Yang, Jian},
title = {Pattern-Affinitive Propagation Across Depth, Surface Normal and Semantic Segmentation},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}

% Ramam et al
@InProceedings{Ramamonjisoa_2019_ICCV,
author = {Ramamonjisoa, Michael and Lepetit, Vincent},
title = {SharpNet: Fast and Accurate Recovery of Occluding Contours in Monocular Depth Estimation},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV) Workshops},
month = {Oct},
year = {2019}
}

% Chen et al
@inproceedings{ijcai2019-98,
  title     = {Structure-Aware Residual Pyramid Network for Monocular Depth Estimation},
  author    = {Chen, Xiaotian and Chen, Xuejin and Zha, Zheng-Jun},
  booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
               Artificial Intelligence, {IJCAI-19}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},             
  pages     = {694--700},
  year      = {2019},
  month     = {7},
  doi       = {10.24963/ijcai.2019/98},
  url       = {https://doi.org/10.24963/ijcai.2019/98},
}

@InProceedings{Yin_2019_ICCV,
author = {Yin, Wei and Liu, Yifan and Shen, Chunhua and Yan, Youliang},
title = {Enforcing Geometric Constraints of Virtual Normal for Depth Prediction},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}


% DAV
@article{dav_huynh2020guiding,
  title={Guiding Monocular Depth Estimation Using Depth-Attention Volume},
  author={Huynh, Lam and Nguyen-Ha, Phong and Matas, Jiri and Rahtu, Esa and Heikkila, Janne},
  journal={arXiv preprint arXiv:2004.02760},
  year={2020}
}

@inproceedings{DepthLab2020,
title	= {DepthLab: Real-time 3D Interaction with Depth Maps for Mobile Augmented Reality},
author	= {Ruofei Du and Eric Lee Turner and Maksym Dzitsiuk and Luca Prasso and Ivo Duarte and Jason Dourgarian and Joao Afonso and Jose Pascoal and Josh Gladstone and Nuno Moura e Silva Cruces and Shahram Izadi and Adarsh Kowdle and Konstantine Nicholas John Tsotsos and David Kim},
year	= {2020},
booktitle	= {Proceedings of the 33rd Annual ACM Symposium on User Interface Software and Technology},
pages	= {15}
}

@InProceedings{Gan2018,
author="Gan, Yukang
and Xu, Xiangyu
and Sun, Wenxiu
and Lin, Liang",
editor="Ferrari, Vittorio
and Hebert, Martial
and Sminchisescu, Cristian
and Weiss, Yair",
title="Monocular Depth Estimation with Affinity, Vertical Pooling, and Label Enhancement",
booktitle="Computer Vision -- ECCV 2018",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="232--247",
abstract="Significant progress has been made in monocular depth estimation with Convolutional Neural Networks (CNNs). While absolute features, such as edges and textures, could be effectively extracted, the depth constraint of neighboring pixels, namely relative features, has been mostly ignored by recent CNN-based methods. To overcome this limitation, we explicitly model the relationships of different image locations with an affinity layer and combine absolute and relative features in an end-to-end network. In addition, we consider prior knowledge that major depth changes lie in the vertical direction, and thus, it is beneficial to capture long-range vertical features for refined depth estimation. In the proposed algorithm we introduce vertical pooling to aggregate image features vertically to improve the depth accuracy. Furthermore, since the Lidar depth ground truth is quite sparse, we enhance the depth labels by generating high-quality dense depth maps with off-the-shelf stereo matching method taking left-right image pairs as input. We also integrate multi-scale structure in our network to obtain global understanding of the image depth and exploit residual learning to help depth refinement. We demonstrate that the proposed algorithm performs favorably against state-of-the-art methods both qualitatively and quantitatively on the KITTI driving dataset.",
isbn="978-3-030-01219-9"
}

@inproceedings{Saxena2005,
author = {Saxena, Ashutosh and Chung, Sung H. and Ng, Andrew Y.},
title = {Learning Depth from Single Monocular Images},
year = {2005},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {We consider the task of depth estimation from a single monocular image. We take a supervised learning approach to this problem, in which we begin by collecting a training set of monocular images (of unstructured outdoor environments which include forests, trees, buildings, etc.) and their corresponding ground-truth depthmaps. Then, we apply supervised learning to predict the depthmap as a function of the image. Depth estimation is a challenging problem, since local features alone are insufficient to estimate depth at a point, and one needs to consider the global context of the image. Our model uses a discriminatively-trained Markov Random Field (MRF) that incorporates multiscale local- and global-image features, and models both depths at individual points as well as the relation between depths at different points. We show that, even on unstructured scenes, our algorithm is frequently able to recover fairly accurate depthmaps.},
booktitle = {Proceedings of the 18th International Conference on Neural Information Processing Systems},
pages = {1161–1168},
numpages = {8},
location = {Vancouver, British Columbia, Canada},
series = {NIPS'05}
}

@article{Liu2016LearningDF,
  title={Learning Depth from Single Monocular Images Using Deep Convolutional Neural Fields},
  author={Fayao Liu and Chunhua Shen and Guosheng Lin and I. Reid},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2016},
  volume={38},
  pages={2024-2039}
}

@article{Alhashim2018,
  author    = {Ibraheem Alhashim and
               Peter Wonka},
  title     = {High Quality Monocular Depth Estimation via Transfer Learning},
  journal   = {CoRR},
  volume    = {abs/1812.11941},
  year      = {2018},
  url       = {http://arxiv.org/abs/1812.11941},
  archivePrefix = {arXiv},
  eprint    = {1812.11941},
  timestamp = {Wed, 02 Jan 2019 14:40:18 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1812-11941.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{efficentnet_TanL19,
  author    = {Mingxing Tan and
               Quoc V. Le},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {6105--6114},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v97/tan19a.html},
  timestamp = {Tue, 11 Jun 2019 15:37:38 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/TanL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{dosovitskiy2020,
  title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and  Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@INPROCEEDINGS{Fan2017_chamfer_loss,
  author={H. {Fan} and H. {Su} and L. {Guibas}},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={A Point Set Generation Network for 3D Object Reconstruction from a Single Image}, 
  year={2017},
  volume={},
  number={},
  pages={2463-2471},
  doi={10.1109/CVPR.2017.264}}
  
  
@InProceedings{Shu2020_eccv2020,
author="Shu, Chang
and Yu, Kun
and Duan, Zhixiang
and Yang, Kuiyuan",
editor="Vedaldi, Andrea
and Bischof, Horst
and Brox, Thomas
and Frahm, Jan-Michael",
title="Feature-Metric Loss for Self-supervised Learning of Depth and Egomotion",
booktitle="Computer Vision -- ECCV 2020",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="572--588",
isbn="978-3-030-58529-7"
}

@INPROCEEDINGS{Song2015_sunrgbd,
  author={S. {Song} and S. P. {Lichtenberg} and J. {Xiao}},
  booktitle={CVPR}, 
  title={SUN RGB-D: A RGB-D scene understanding benchmark suite}, 
  year={2015}
  }
  

@InProceedings{pmlr-v80-parmar18a,
title = 	 {Image Transformer},
author =       {Parmar, Niki and Vaswani, Ashish and Uszkoreit, Jakob and Kaiser, Lukasz and Shazeer, Noam and Ku, Alexander and Tran, Dustin},
pages = 	 {4055--4064},
year = 	 {2018},
editor = 	 {Jennifer Dy and Andreas Krause},
volume = 	 {80},
series = 	 {Proceedings of Machine Learning Research},
booktitle={Proceedings of Machine Learning Research},
address = 	 {Stockholmsmässan, Stockholm Sweden},
month = 	 {10--15 Jul},
publisher =    {PMLR},
pdf = 	 {http://proceedings.mlr.press/v80/parmar18a/parmar18a.pdf},
url = 	 {http://proceedings.mlr.press/v80/parmar18a.html}
}

@inproceedings{HuEACL2024_flowseq,
        title = {Flow Matching for Conditional Text Generation in a Few Sampling Steps},
        author = {Vincent Tao Hu and Di Wu and Yuki M Asano and Pascal Mettes and Basura Fernando and Björn Ommer and Cees G M Snoek},
        year = {2024},
        date = {2024-03-27},
        booktitle = {EACL},
        tppubtype = {inproceedings}
        }

@InProceedings{detr2020,
author="Carion, Nicolas
and Massa, Francisco
and Synnaeve, Gabriel
and Usunier, Nicolas
and Kirillov, Alexander
and Zagoruyko, Sergey",
editor="Vedaldi, Andrea
and Bischof, Horst
and Brox, Thomas
and Frahm, Jan-Michael",
title="End-to-End Object Detection with Transformers",
booktitle="Computer Vision -- ECCV 2020",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="213--229"
}

@InProceedings{Wang_2018_CVPR,
author = {Wang, Xiaolong and Girshick, Ross and Gupta, Abhinav and He, Kaiming},
title = {Non-Local Neural Networks},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}

@inproceedings{transf_obj_NEURIPS2019_680390c5,
 author = {Herdade, Simao and Kappeler, Armin and Boakye, Kofi and Soares, Joao},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {11137--11147},
 publisher = {Curran Associates, Inc.},
 title = {Image Captioning: Transforming Objects into Words},
 url = {https://proceedings.neurips.cc/paper/2019/file/680390c55bbd9ce416d1d69a9ab4760d-Paper.pdf},
 volume = {32},
 year = {2019}
}

@InProceedings{Cornia_2020_CVPR,
author = {Cornia, Marcella and Stefanini, Matteo and Baraldi, Lorenzo and Cucchiara, Rita},
title = {Meshed-Memory Transformer for Image Captioning},
booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@InProceedings{garg10.1007/978-3-319-46484-8_45,
author="Garg, Ravi
and B.G., Vijay Kumar
and Carneiro, Gustavo
and Reid, Ian",
editor="Leibe, Bastian
and Matas, Jiri
and Sebe, Nicu
and Welling, Max",
title="Unsupervised CNN for Single View Depth Estimation: Geometry to the Rescue",
booktitle="Computer Vision -- ECCV 2016",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="740--756",
abstract="A significant weakness of most current deep Convolutional Neural Networks is the need to train them using vast amounts of manually labelled data. In this work we propose a unsupervised framework to learn a deep convolutional neural network for single view depth prediction, without requiring a pre-training stage or annotated ground-truth depths. We achieve this by training the network in a manner analogous to an autoencoder. At training time we consider a pair of images, source and target, with small, known camera motion between the two such as a stereo pair. We train the convolutional encoder for the task of predicting the depth map for the source image. To do so, we explicitly generate an inverse warp of the target image using the predicted depth and known inter-view displacement, to reconstruct the source image; the photometric error in the reconstruction is the reconstruction loss for the encoder. The acquisition of this training data is considerably simpler than for equivalent systems, requiring no manual annotation, nor calibration of depth sensor to camera. We show that our network trained on less than half of the KITTI dataset gives comparable performance to that of the state-of-the-art supervised methods for single view depth estimation.",
isbn="978-3-319-46484-8"
}

@incollection{janoch2013category,
  title={A category-level 3d object dataset: Putting the kinect to work},
  author={Janoch, Allison and Karayev, Sergey and Jia, Yangqing and Barron, Jonathan T and Fritz, Mario and Saenko, Kate and Darrell, Trevor},
  booktitle={Consumer depth cameras for computer vision},
  pages={141--165},
  year={2013},
  publisher={Springer}
}

@INPROCEEDINGS{sun6751312,
author={J. {Xiao} and A. {Owens} and A. {Torralba}},
booktitle={2013 IEEE International Conference on Computer Vision},
title={SUN3D: A Database of Big Spaces Reconstructed Using SfM and Object Labels},
year={2013},
volume={}, 
number={},
pages={1625-1632},
doi={10.1109/ICCV.2013.458}
}


@inproceedings{deeplabv3plus2018,
  title={Encoder-Decoder with Atrous Separable Convolution for Semantic Image Segmentation},
  author={Liang-Chieh Chen and Yukun Zhu and George Papandreou and Florian Schroff and Hartwig Adam},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{koch2019,
title = "Evaluation of CNN-based Single-Image Depth Estimation Methods",
author = "Tobias Koch and Lukas Liebel and Friedrich Fraundorfer and Marco K{\"o}rner",
year = "2019",
language = "English",
booktitle = "Proceedings ECCV 2018 Workshops",
}

@INPROCEEDINGS{He2017_MaskRCNN,
  author={He, Kaiming and Gkioxari, Georgia and Dollár, Piotr and Girshick, Ross},
  booktitle={2017 IEEE International Conference on Computer Vision (ICCV)}, 
  title={Mask R-CNN}, 
  year={2017},
  volume={},
  number={},
  pages={2980-2988},
  doi={10.1109/ICCV.2017.322}}
  
 @InProceedings{Zhao_2020_CVPR,
author = {Zhao, Yunhan and Kong, Shu and Shin, Daeyun and Fowlkes, Charless},
title = {Domain Decluttering: Simplifying Images to Mitigate Synthetic-Real Domain Shift and Improve Depth Estimation},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@inproceedings{bhat2021adabins,
  title={Adabins: Depth estimation using adaptive bins},
  author={Bhat, Shariq Farooq and Alhashim, Ibraheem and Wonka, Peter},
  booktitle={CVPR},
  year={2021}
}

@inproceedings{bhat2022localbins,
  title={LocalBins: Improving Depth Estimation by Learning Local Distributions},
  author={Bhat, Shariq Farooq and Alhashim, Ibraheem and Wonka, Peter},
  booktitle={ECCV},
  year={2022}
}

@article{yuan2022new,
  title={New crfs: Neural window fully-connected crfs for monocular depth estimation},
  author={Yuan, Weihao and Gu, Xiaodong and Dai, Zuozhuo and Zhu, Siyu and Tan, Ping},
  journal={arXiv},
  year={2022}
}

@article{li2022binsformer,
  title={BinsFormer: Revisiting Adaptive Bins for Monocular Depth Estimation},
  author={Li, Zhenyu and Wang, Xuyang and Liu, Xianming and Jiang, Junjun},
  journal={arXiv},
  year={2022}
}

@article{SIDEreviewMERTAN2022103441,
title = {Single image depth estimation: An overview},
journal = {Digital Signal Processing},
year = {2022},
author = {Alican Mertan and Damien Jade Duff and Gozde Unal},
}


@article{agarwal2022attention,
  title={Attention Attention Everywhere: Monocular Depth Prediction with Skip Attention},
  author={Agarwal, Ashutosh and Arora, Chetan},
  journal={arXiv preprint arXiv:2210.09071},
  year={2022}
}


@InProceedings{unimodal-pmlr-v70-beckham17a,
  title = 	 {Unimodal Probability Distributions for Deep Ordinal Classification},
  author =       {Christopher Beckham and Christopher Pal},
  booktitle = 	 {Proceedings of the 34th International Conference on Machine Learning},
  pages = 	 {411--419},
  year = 	 {2017},
  editor = 	 {Precup, Doina and Teh, Yee Whye},
  volume = 	 {70},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {06--11 Aug},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v70/beckham17a/beckham17a.pdf},
  url = 	 {https://proceedings.mlr.press/v70/beckham17a.html},
  abstract = 	 {Probability distributions produced by the cross-entropy loss for ordinal classification problems can possess undesired properties. We propose a straightforward technique to constrain discrete ordinal probability distributions to be unimodal via the use of the Poisson and binomial probability distributions. We evaluate this approach in the context of deep learning on two large ordinal image datasets, obtaining promising results.}
}

@article{DBLP:journals/corr/abs-2106-08254,
  author    = {Hangbo Bao and
               Li Dong and
               Furu Wei},
  title     = {BEiT: {BERT} Pre-Training of Image Transformers},
  journal   = {CoRR},
  volume    = {abs/2106.08254},
  year      = {2021},
  url       = {https://arxiv.org/abs/2106.08254},
  eprinttype = {arXiv},
  eprint    = {2106.08254},
  timestamp = {Tue, 29 Jun 2021 16:55:04 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2106-08254.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Menze_2015_CVPR,
author = {Menze, Moritz and Geiger, Andreas},
title = {Object Scene Flow for Autonomous Vehicles},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2015}
}

@inproceedings{xian2018monocular,
  title={Monocular relative depth perception with web stereo data supervision},
  author={Xian, Ke and Shen, Chunhua and Cao, Zhiguo and Lu, Hao and Xiao, Yang and Li, Ruibo and Luo, Zhenbo},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={311--320},
  year={2018}
}

@inproceedings{wang2019web,
  title={Web stereo video supervision for depth prediction from dynamic scenes},
  author={Wang, Chaoyang and Lucey, Simon and Perazzi, Federico and Wang, Oliver},
  booktitle={2019 International Conference on 3D Vision (3DV)},
  pages={348--357},
  year={2019},
  organization={IEEE}
}

@article{kim2018deep,
  title={Deep monocular depth estimation via integration of global and local predictions},
  author={Kim, Youngjung and Jung, Hyungjoo and Min, Dongbo and Sohn, Kwanghoon},
  journal={IEEE transactions on Image Processing},
  volume={27},
  number={8},
  pages={4131--4144},
  year={2018},
  publisher={IEEE}
}

@inproceedings{yao2020blendedmvs,
  title={Blendedmvs: A large-scale dataset for generalized multi-view stereo networks},
  author={Yao, Yao and Luo, Zixin and Li, Shiwei and Zhang, Jingyang and Ren, Yufan and Zhou, Lei and Fang, Tian and Quan, Long},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1790--1799},
  year={2020}
}

@inproceedings{wang2020tartanair,
  title={Tartanair: A dataset to push the limits of visual slam},
  author={Wang, Wenshan and Zhu, Delong and Wang, Xiangwei and Hu, Yaoyu and Qiu, Yuheng and Wang, Chen and Hu, Yafei and Kapoor, Ashish and Scherer, Sebastian},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4909--4916},
  year={2020},
  organization={IEEE}
}

@article{huang2019apolloscape,
  title={The apolloscape open dataset for autonomous driving and its application},
  author={Huang, Xinyu and Wang, Peng and Cheng, Xinjing and Zhou, Dingfu and Geng, Qichuan and Yang, Ruigang},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={42},
  number={10},
  pages={2702--2719},
  year={2019},
  publisher={IEEE}
}

@article{wang2019irs,
  title={Irs: A large naturalistic indoor robotics stereo dataset to train deep models for disparity and surface normal estimation},
  author={Wang, Qiang and Zheng, Shizhen and Yan, Qingsong and Deng, Fei and Zhao, Kaiyong and Chu, Xiaowen},
  journal={arXiv preprint arXiv:1912.09678},
  year={2019}
}

@inproceedings{xian2020structure,
  title={Structure-guided ranking loss for single image depth prediction},
  author={Xian, Ke and Zhang, Jianming and Wang, Oliver and Mai, Long and Lin, Zhe and Cao, Zhiguo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={611--620},
  year={2020}
}

@inproceedings{yin2021learning,
  title={Learning to recover 3d scene shape from a single image},
  author={Yin, Wei and Zhang, Jianming and Wang, Oliver and Niklaus, Simon and Mai, Long and Chen, Simon and Shen, Chunhua},
  booktitle={CVPR},
  year={2021}
}

@article{jun2022depth,
  title={Depth Map Decomposition for Monocular Depth Estimation},
  author={Jun, Jinyoung and Lee, Jae-Han and Lee, Chul and Kim, Chang-Su},
  journal={arXiv},
  year={2022}
}

@inproceedings{roberts:2021,
    author    = {Mike Roberts AND Jason Ramapuram AND Anurag Ranjan AND Atulit Kumar AND
                 Miguel Angel Bautista AND Nathan Paczan AND Russ Webb AND Joshua M. Susskind},
    title     = {{Hypersim}: {A} Photorealistic Synthetic Dataset for Holistic Indoor Scene Understanding},
    booktitle = {ICCV},
    year      = {2021}
}

@inproceedings{packnet,
  author = {Vitor Guizilini and Rares Ambrus and Sudeep Pillai and Allan Raventos and Adrien Gaidon},
  title = {3D Packing for Self-Supervised Monocular Depth Estimation},
  booktitle = {IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  primaryClass = {cs.CV},
  year = {2020},
}

@inproceedings{liu2022swin,
  title={Swin transformer v2: Scaling up capacity and resolution},
  author={Liu, Ze and Hu, Han and Lin, Yutong and Yao, Zhuliang and Xie, Zhenda and Wei, Yixuan and Ning, Jia and Cao, Yue and Zhang, Zheng and Dong, Li and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12009--12019},
  year={2022}
}

@inproceedings{liu2021swin,
  title={Swin transformer: Hierarchical vision transformer using shifted windows},
  author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={10012--10022},
  year={2021}
}

@article{abramowitz2002stegun,
  title={Stegun., IA (1972). Handbook of mathematical functions},
  author={Abramowitz, Miton},
  journal={Formulas, Graphs and Mathematical Tables},
  year={2002}
}

@inproceedings{lee2019monocular,
  title={Monocular depth estimation using relative depth maps},
  author={Lee, Jae-Han and Kim, Chang-Su},
  booktitle={CVPR},
  year={2019}
}

@misc{cabon2020vkitti2,
  title={Virtual KITTI 2},
  author={Cabon, Yohann and Murray, Naila and Humenberger, Martin},
  year={2020},
  eprint={2001.10773},
  archivePrefix={arXiv},
  primaryClass={cs.CV}
}

@misc{rw2019timm,
  author = {Ross Wightman},
  title = {PyTorch Image Models},
  year = {2019},
  publisher = {GitHub},
  journal = {GitHub repository},
  doi = {10.5281/zenodo.4414861},
  howpublished = {\url{https://github.com/rwightman/pytorch-image-models}}
}

@article{fedus2022review,
  title={A review of sparse expert models in deep learning},
  author={Fedus, William and Dean, Jeff and Zoph, Barret},
  journal={arXiv preprint arXiv:2209.01667},
  year={2022}
}


@mastersthesis{pixelbinsSarwari:EECS-2021-32,
    Author = {Sarwari, Khalil and Laine, Forrest and Tomlin, Claire},
    Title = {Progress and Proposals: A Case Study of Monocular Depth Estimation},
    School = {EECS Department, University of California, Berkeley},
    Year = {2021},
    Month = {May},
    URL = {http://www2.eecs.berkeley.edu/Pubs/TechRpts/2021/EECS-2021-32.html},
    Number = {UCB/EECS-2021-32},
    Abstract = {Deep learning has achieved great results and made rapid progress over the past few years, particularly in the field of computer vision. Deep learning models are composed of artificial neural networks and a supervised, semi-supervised, or unsupervised learning scheme. Larger models have neural network architectures with more parameters, often resulting from more/wider layers. In this paper, we perform a case study in the domain of monocular depth estimation and contribute both a new model as well as a new dataset. We propose PixelBins, a simplification to AdaBins, the existing state-of-the-art model, and obtain comparable performance to state-of-the-art methods. Our method achieves a ~20x reduction in model size as well as an absolute relative error of 0.057 on the popular KITTI benchmark. Furthermore, we conceptualize and justify the need for truly open datasets. Consequently, we introduce a modern, extensible dataset consisting of high quality, cross-calibrated image+point cloud pairs across a diverse set of locations. The dataset is uniquely suited for the designation of truly open for a variety of reasons, such as a ~100x reduction in cost to contribute a new image+pointcloud pair. We make our code and dataset publicly available and provide instructions for contributing to and replicating our experiments.}
}




@article{LI2018328CSWS,
title = {Monocular depth estimation with hierarchical fusion of dilated CNNs and soft-weighted-sum inference},
journal = {Pattern Recognition},
year = {2018},
author = {Bo Li and Yuchao Dai and Mingyi He},
}

@InProceedings{DABC_10.1007/978-3-030-20870-7_41,
author="Li, Ruibo
and Xian, Ke
and Shen, Chunhua
and Cao, Zhiguo
and Lu, Hao
and Hang, Lingxiao",
editor="Jawahar, C.V.
and Li, Hongdong
and Mori, Greg
and Schindler, Konrad",
title="Deep Attention-Based Classification Network for Robust Depth Prediction",
booktitle="ACCV",
year="2019"
}




--------------- Typical methods ---------------
@inproceedings{eigen_depth_2014,
  title   = {Depth Map Prediction from a Single Image using a Multi-Scale Deep Network},
  author  = {Eigen, David and Puhrsch, Christian and Fergus, Rob},
  year    = 2014,
  booktitle = NIPS
}

@inproceedings{fu2018dorn,
  title   = {Deep ordinal regression network for monocular depth estimation},
  author  = {Fu, Huan and Gong, Mingming and Wang, Chaohui and Batmanghelich, Kayhan and Tao, Dacheng},
  year    = 2018,
  booktitle = CVPR,
  pages   = {2002--2011}
}

@inproceedings{yuan2022newcrfs,
  title   = {{NeWCRFs}: Neural Window Fully-connected {CRFs} for Monocular Depth Estimation},
  author  = {Yuan, Weihao and Gu, Xiaodong and Dai, Zuozhuo and Zhu, Siyu and Tan, Ping},
  year    = 2022,
  booktitle = CVPR
}

@inproceedings{aich2021bidirectional,
  title   = {Bidirectional Attention Network for Monocular Depth Estimation},
  author  = {Shubhra Aich and Jean Marie Uwabeza Vianney and Md Amirul Islam and Mannat Kaur and Bingbing Liu},
  year    = 2021,
  booktitle = {ICRA}
}

@inproceedings{zhang_pattern-affinitive_2019,
  title   = {Pattern-Affinitive Propagation Across Depth, Surface Normal and Semantic Segmentation},
  author  = {Zhang, Zhenyu and Cui, Zhen and Xu, Chunyan and Yan, Yan and Sebe, Nicu and Yang, Jian},
  year    = 2019,
  booktitle = CVPR
}

@article{lee2019big,
  title   = {From big to small: Multi-scale local planar guidance for monocular depth estimation},
  author  = {Lee, Jin Han and Han, Myung-Kyu and Ko, Dong Wook and Suh, Il Hong},
  year    = 2019,
  journal = {arXiv preprint arXiv:1907.10326}
}

@inproceedings{yin2019enforcing,
  title   = {Enforcing geometric constraints of virtual normal for depth prediction},
  author  = {Yin, Wei and Liu, Yifan and Shen, Chunhua and Yan, Youliang},
  year    = 2019,
  booktitle = ICCV,
  pages   = {5684--5693}
}

@inproceedings{Farooq_Bhat_2021,
  title   = {{AdaBins}: Depth Estimation Using Adaptive Bins},
  author  = {Shariq Farooq Bhat and Ibraheem Alhashim and Peter Wonka},
  year    = 2021,
  booktitle = CVPR
}

@inproceedings{yang2021transformers,
  title   = {Transformer-Based Attention Networks for Continuous Pixel-Wise Prediction},
  author  = {Yang, Guanglei and Tang, Hao and Ding, Mingli and Sebe, Nicu and Ricci, Elisa},
  year    = 2021,
  booktitle = {ICCV}
}

@inproceedings{patil2022p3depth,
  title   = {P3depth: Monocular depth estimation with a piecewise planarity prior},
  author  = {Patil, Vaishakh and Sakaridis, Christos and Liniger, Alexander and Van Gool, Luc},
  year    = 2022,
  booktitle = CVPR
}

@inproceedings{kumar_monocular_2018,
  title   = {Monocular Depth Prediction Using Generative Adversarial Networks},
  author  = {Kumar, Aran {CS} and Bhandarkar, Suchendra M. and Prasad, Mukta},
  year    = 2018,
  booktitle = CVPRW
}

@article{li2023depthformer,
  title   = {Depthformer: Exploiting long-range correlation and local information for accurate monocular depth estimation},
  author  = {Li, Zhenyu and Chen, Zehui and Liu, Xianming and Jiang, Junjun},
  year    = 2023,
  journal = {Machine Intelligence Research},
  publisher = {Springer},
  pages   = {1--18}
}

@inproceedings{liu2023vadepth,
  title   = {{VA-DepthNet}: A variational approach to single image depth prediction},
  author  = {Liu, Ce and Kumar, Suryansh and Gu, Shuhang and Timofte, Radu and {Van Gool}, Luc},
  year    = 2023,
  booktitle = ICLR
}

@inproceedings{ning2023ait,
  title   = {All in tokens: Unifying output space of visual tasks via soft token},
  author  = {Ning, Jia and Li, Chen and Zhang, Zheng and Wang, Chunyu and Geng, Zigang and Dai, Qi and He, Kun and Hu, Han},
  year    = 2023,
  booktitle = ICCV,
  pages   = {19900--19910}
}

@article{bhat2023zoedepth,
  title   = {{ZoeDepth}: Zero-shot transfer by combining relative and metric depth},
  author  = {Bhat, Shariq Farooq and Birkl, Reiner and Wofk, Diana and Wonka, Peter and M{\"u}ller, Matthias},
  year    = 2023,
  journal = {arXiv}
}

@article{saxena2023dmd,
  title={Zero-Shot Metric Depth with a Field-of-View Conditioned Diffusion Model},
  author={Saxena, Saurabh and Hur, Junhwa and Herrmann, Charles and Sun, Deqing and Fleet, David J},
  journal={arXiv},
  year={2023}
}

@inproceedings{jun2022depthdecomp,
  title   = {Depth map decomposition for monocular depth estimation},
  author  = {Jun, Jinyoung and Lee, Jae-Han and Lee, Chul and Kim, Chang-Su},
  year    = 2022,
  booktitle = ECCV,
  pages   = {18--34},
  organization = {Springer}
}

@inproceedings{cs2018monocular,
  title={Monocular depth prediction using generative adversarial networks},
  author={CS Kumar, Arun and Bhandarkar, Suchendra M and Prasad, Mukta},
  booktitle=CVPR,
  pages={300--308},
  year={2018}
}

--------------- zero-shot affine-invariant methods ---------------
@inproceedings{MDLi18_megadepth,
  title   = {{MegaDepth}: Learning Single-View Depth Prediction from Internet Photos},
  author  = {Zhengqi Li and Noah Snavely},
  year    = 2018,
  booktitle = CVPR
}

@article{yin2020diversedepth,
  title   = {Diversedepth: Affine-invariant depth prediction using diverse data},
  author  = {Yin, Wei and Wang, Xinlong and Shen, Chunhua and Liu, Yifan and Tian, Zhi and Xu, Songcen and Sun, Changming and Renyin, Dou},
  year    = 2020,
  journal = {arXiv preprint arXiv:2002.00569}
}


@inproceedings{ranftl2021_dpt,
  title   = {Vision transformers for dense prediction},
  author  = {Ranftl, Ren{\'e} and Bochkovskiy, Alexey and Koltun, Vladlen},
  year    = 2021,
  booktitle = ICCV
}

@inproceedings{eftekhar2021omnidata,
  title   = {Omnidata: A scalable pipeline for making multi-task mid-level vision datasets from 3d scans},
  author  = {Eftekhar, Ainaz and Sax, Alexander and Malik, Jitendra and Zamir, Amir},
  year    = 2021,
  booktitle = ICCV,
  pages   = {10786--10796}
}

@inproceedings{Wei2021CVPR_leres,
  title   = {Learning to Recover 3D Scene Shape from a Single Image},
  author  = {Wei Yin and Jianming Zhang and Oliver Wang and Simon Niklaus and Long Mai and Simon Chen and Chunhua Shen},
  year    = 2021,
  booktitle = CVPR
}

@article{zhang2022_hdn,
  title   = {Hierarchical Normalization for Robust Monocular Depth Estimation},
  author  = {Zhang, Chi and Yin, Wei and Wang, Billzb and Yu, Gang and Fu, Bin and Shen, Chunhua},
  year    = 2022,
  journal = NeurIPS,
  volume  = 35,
}

@inproceedings{xian2020structure,
  title={Structure-guided ranking loss for single image depth prediction},
  author={Xian, Ke and Zhang, Jianming and Wang, Oliver and Mai, Long and Lin, Zhe and Cao, Zhiguo},
  booktitle=CVPR,
  pages={611--620},
  year={2020}
}


--------------- relative depth ---------------
@article{chen2016single,
  title={Single-image depth perception in the wild},
  author={Chen, Weifeng and Fu, Zhao and Yang, Dawei and Deng, Jia},
  journal=NIPS,
  volume={29},
  year={2016}
}

@inproceedings{chen2020oasis,
  title={{OASIS}: A large-scale dataset for single image 3d in the wild},
  author={Chen, Weifeng and Qian, Shengyi and Fan, David and Kojima, Noriyuki and Hamilton, Max and Deng, Jia},
  booktitle={CVPR},
  year={2020}
}

--------------- zero-shot with camera intrinsics ---------------
@inproceedings{guizilini2023towards_zero_depth,
  title   = {Towards zero-shot scale-aware monocular depth estimation},
  author  = {Guizilini, Vitor and Vasiljevic, Igor and Chen, Dian and Ambruș, Rareș and Gaidon, Adrien},
  year    = 2023,
  booktitle = ICCV
}

@inproceedings{yin2023metric3d,
  title   = {{Metric3D}: Towards zero-shot metric 3d prediction from a single image},
  author  = {Yin, Wei and Zhang, Chi and Chen, Hao and Cai, Zhipeng and Yu, Gang and Wang, Kaixuan and Chen, Xiaozhi and Shen, Chunhua},
  year    = 2023,
  booktitle = ICCV
}

--------------- depth + diffusion ---------------

# TODO: check
@inproceedings{ji2023ddp,
  title   = {{DDP}: Diffusion Model for Dense Visual Prediction},
  author  = {Ji, Yuanfeng and Chen, Zhe and Xie, Enze and Hong, Lanqing and Liu, Xihui and Liu, Zhaoqiang and Lu, Tong and Li, Zhenguo and Luo, Ping},
  year    = 2023,
  booktitle = ICCV
}

@article{zhao2023vpd,
  title   = {Unleashing Text-to-Image Diffusion Models for Visual Perception},
  author  = {Zhao, Wenliang and Rao, Yongming and Liu, Zuyan and Liu, Benlin and Zhou, Jie and Lu, Jiwen},
  year    = 2023,
  journal  = {arXiv},
}

@article{saxena2023surprising_ddvm,
  title   = {The Surprising Effectiveness of Diffusion Models for Optical Flow and Monocular Depth Estimation},
  author  = {Saurabh Saxena and Charles Herrmann and Junhwa Hur and Abhishek Kar and Mohammad Norouzi and Deqing Sun and David J. Fleet},
  year    = 2023,
  journal  = {arXiv}
}

@article{duan2023diffusiondepth,
  title   = {{DiffusionDepth}: Diffusion denoising approach for monocular depth estimation},
  author  = {Duan, Yiqun and Guo, Xianda and Zhu, Zheng},
  year    = 2023,
  journal = {arXiv}
}

@article{saxena2023depthgen,
  title={Monocular depth estimation using diffusion models},
  author={Saxena, Saurabh and Kar, Abhishek and Norouzi, Mohammad and Fleet, David J},
  journal={arXiv},
  year={2023}
}


--------------- diffusion ---------------
@inproceedings{rombach2022high,
  title   = {High-resolution image synthesis with latent diffusion models},
  author  = {Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Bj{\"o}rn},
  year    = 2022,
  booktitle = {CVPR}
}

@article{schuhmann2022laion5b,
  title={{LAION-5B}: An open large-scale dataset for training next generation image-text models},
  author={Schuhmann, Christoph and Beaumont, Romain and Vencu, Richard and Gordon, Cade and Wightman, Ross and Cherti, Mehdi and Coombes, Theo and Katta, Aarush and Mullis, Clayton and Wortsman, Mitchell and others},
  journal={NeurIPS},
  volume={35},
  pages={25278--25294},
  year={2022}
}

@article{song2020denoising_ddim,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv preprint arXiv:2010.02502},
  year={2020}
}

@article{ramesh2022hierarchical_dalle2,
  title={Hierarchical text-conditional image generation with {CLIP} latents},
  author={Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  journal={arXiv preprint arXiv:2204.06125},
  year={2022}
}

@article{betker_dalle3improving_nodate,
	title = {Improving Image Generation with Better Captions},
	author = {Betker, James and Goh, Gabriel and Jing, Li and Brooks, Tim and Wang, Jianfeng and Li, Linjie and Ouyang, Long and Zhuang, Juntang and Lee, Joyce and Guo, Yufei and Manassra, Wesam and Dhariwal, Prafulla and Chu, Casey and Jiao, Yunxin and Ramesh, Aditya},
    year = 2023,
    journal = {\url{https://cdn.openai.com/papers/dall-e-3.pdf}}
}


@article{saharia2022photorealistic,
  title={Photorealistic text-to-image diffusion models with deep language understanding},
  author={Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily L and Ghasemipour, Kamyar and Gontijo Lopes, Raphael and Karagol Ayan, Burcu and Salimans, Tim and others},
  journal={NeurIPS},
  volume={35},
  year={2022}
}

@inproceedings{saharia2022palette,
  title={Palette: Image-to-image diffusion models},
  author={Saharia, Chitwan and Chan, William and Chang, Huiwen and Lee, Chris and Ho, Jonathan and Salimans, Tim and Fleet, David and Norouzi, Mohammad},
  booktitle={ACM SIGGRAPH},
  pages={1--10},
  year={2022}
}

--------------- other diffusion application ---------------
@article{wu2022medsegdiff,
  title={{MedSegDiff}: Medical image segmentation with diffusion probabilistic model},
  author={Wu, Junde and Fang, Huihui and Zhang, Yu and Yang, Yehui and Xu, Yanwu},
  journal={arXiv preprint arXiv:2211.00611},
  year={2022}
}
@inproceedings{wolleb2022diffusion,
  title={Diffusion models for implicit image segmentation ensembles},
  author={Wolleb, Julia and Sandk{\"u}hler, Robin and Bieder, Florentin and Valmaggia, Philippe and Cattin, Philippe C},
  booktitle={MIDL},
  pages={1336--1348},
  year={2022}
}
@article{amit2021segdiff,
  title={Segdiff: Image segmentation with diffusion probabilistic models},
  author={Amit, Tomer and Nachmani, Eliya and Shaharbany, Tal and Wolf, Lior},
  journal={arXiv preprint arXiv:2112.00390},
  year={2021}
}
@inproceedings{chen2023generalist,
  title={A generalist framework for panoptic segmentation of images and videos},
  author={Chen, Ting and Li, Lala and Saxena, Saurabh and Hinton, Geoffrey and Fleet, David J},
  booktitle={ICCV},
  year={2023}
}

@article{choi2022diffupose,
  title={{DiffuPose}: Monocular 3d human pose estimation via denoising diffusion probabilistic model},
  author={Choi, Jeongjun and Shim, Dongseok and Kim, H Jin},
  journal={arXiv preprint arXiv:2212.02796},
  year={2022}
}
@inproceedings{chen2023diffusiondet,
  title={{DiffusionDet}: Diffusion model for object detection},
  author={Chen, Shoufa and Sun, Peize and Song, Yibing and Luo, Ping},
  booktitle={ICCV},
  pages={19830--19843},
  year={2023}
}

@inproceedings{mei2023vidm,
  title={{VIDM}: Video implicit diffusion models},
  author={Mei, Kangfu and Patel, Vishal},
  booktitle=AAAI,
  volume={37},
  number={8},
  pages={9117--9125},
  year={2023}
}
@inproceedings{cai2022diffdreamer,
  title     = {{DiffDreamer}: Towards Consistent Unsupervised Single-view Scene Extrapolation with Conditional Diffusion Models},
  author    = {Cai, Shengqu and Chan, Eric Ryan and Peng, Songyou and Shahbazi, Mohamad and Obukhov, Anton 
               and {Van Gool}, Luc and Wetzstein, Gordon},
  booktitle = ICCV,
  year      = {2023}
}
@inproceedings{wang2023breathing,
  title={Breathing New Life into 3D Assets with Generative Repainting},
  author={Wang, Tianfu and Kanakis, Menelaos and Schindler, Konrad and {Van Gool}, Luc and Obukhov, Anton},
  booktitle=BMVC,
  year={2023},
  publisher={BMVA Press}
}


--------------- utilizing vision foundation models ---------------
@article{bommasani2022opportunities,
      title={On the Opportunities and Risks of Foundation Models}, 
      author={Rishi Bommasani and Drew A. Hudson and Ehsan Adeli and Russ Altman and Simran Arora and Sydney von Arx and Michael S. Bernstein and Jeannette Bohg and Antoine Bosselut and Emma Brunskill and Erik Brynjolfsson and others},
      year={2022},
      journal={arXiv preprint arXiv:2108.07258}
}

%misc{bommasani2022opportunities,
      title={On the Opportunities and Risks of Foundation Models}, 
      author={Rishi Bommasani and Drew A. Hudson and Ehsan Adeli and Russ Altman and Simran Arora and Sydney von Arx and Michael S. Bernstein and Jeannette Bohg and Antoine Bosselut and Emma Brunskill and Erik Brynjolfsson and Shyamal Buch and Dallas Card and Rodrigo Castellon and Niladri Chatterji and Annie Chen and Kathleen Creel and Jared Quincy Davis and Dora Demszky and Chris Donahue and Moussa Doumbouya and Esin Durmus and Stefano Ermon and John Etchemendy and Kawin Ethayarajh and Li Fei-Fei and Chelsea Finn and Trevor Gale and Lauren Gillespie and Karan Goel and Noah Goodman and Shelby Grossman and Neel Guha and Tatsunori Hashimoto and Peter Henderson and John Hewitt and Daniel E. Ho and Jenny Hong and Kyle Hsu and Jing Huang and Thomas Icard and Saahil Jain and Dan Jurafsky and Pratyusha Kalluri and Siddharth Karamcheti and Geoff Keeling and Fereshte Khani and Omar Khattab and Pang Wei Koh and Mark Krass and Ranjay Krishna and Rohith Kuditipudi and Ananya Kumar and Faisal Ladhak and Mina Lee and Tony Lee and Jure Leskovec and Isabelle Levent and Xiang Lisa Li and Xuechen Li and Tengyu Ma and Ali Malik and Christopher D. Manning and Suvir Mirchandani and Eric Mitchell and Zanele Munyikwa and Suraj Nair and Avanika Narayan and Deepak Narayanan and Ben Newman and Allen Nie and Juan Carlos Niebles and Hamed Nilforoshan and Julian Nyarko and Giray Ogut and Laurel Orr and Isabel Papadimitriou and Joon Sung Park and Chris Piech and Eva Portelance and Christopher Potts and Aditi Raghunathan and Rob Reich and Hongyu Ren and Frieda Rong and Yusuf Roohani and Camilo Ruiz and Jack Ryan and Christopher Ré and Dorsa Sadigh and Shiori Sagawa and Keshav Santhanam and Andy Shih and Krishnan Srinivasan and Alex Tamkin and Rohan Taori and Armin W. Thomas and Florian Tramèr and Rose E. Wang and William Wang and Bohan Wu and Jiajun Wu and Yuhuai Wu and Sang Michael Xie and Michihiro Yasunaga and Jiaxuan You and Matei Zaharia and Michael Zhang and Tianyi Zhang and Xikun Zhang and Yuhui Zhang and Lucia Zheng and Kaitlyn Zhou and Percy Liang},
      year={2022},
      eprint={2108.07258},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{ruiz2023dreambooth,
  title={{DreamBooth}: Fine tuning text-to-image diffusion models for subject-driven generation},
  author={Ruiz, Nataniel and Li, Yuanzhen and Jampani, Varun and Pritch, Yael and Rubinstein, Michael and Aberman, Kfir},
  booktitle=CVPR,
  pages={22500--22510},
  year={2023}
}

@InProceedings{zhou2022maskclip,
    author = {Zhou, Chong and Loy, Chen Change and Dai, Bo},
    title = {Extract Free Dense Labels from {CLIP}},
    booktitle = {ECCV},
    year = {2022}
}

@inproceedings{yao2023visual,
  title={Visual-language prompt tuning with knowledge-guided context optimization},
  author={Yao, Hantao and Zhang, Rui and Xu, Changsheng},
  booktitle=CVPR,
  pages={6757--6767},
  year={2023}
}
@inproceedings{zhang2023prompt,
  title={Prompt, generate, then cache: Cascade of foundation models makes strong few-shot learners},
  author={Zhang, Renrui and Hu, Xiangfei and Li, Bohao and Huang, Siyuan and Deng, Hanqiu and Qiao, Yu and Gao, Peng and Li, Hongsheng},
  booktitle=CVPR,
  pages={15211--15222},
  year={2023}
}
@article{bahng2022exploring,
  title={Exploring visual prompts for adapting large-scale models},
  author={Bahng, Hyojin and Jahanian, Ali and Sankaranarayanan, Swami and Isola, Phillip},
  journal={arXiv preprint arXiv:2203.17274},
  year={2022}
}
@article{gao2023clip,
  title={{CLIP}-adapter: Better vision-language models with feature adapters},
  author={Gao, Peng and Geng, Shijie and Zhang, Renrui and Ma, Teli and Fang, Rongyao and Zhang, Yongfeng and Li, Hongsheng and Qiao, Yu},
  journal={International Journal of Computer Vision},
  year={2023},
  publisher={Springer}
}
@article{zhang2021tip,
  title={Tip-adapter: Training-free {CLIP}-adapter for better vision-language modeling},
  author={Zhang, Renrui and Fang, Rongyao and Zhang, Wei and Gao, Peng and Li, Kunchang and Dai, Jifeng and Qiao, Yu and Li, Hongsheng},
  journal={arXiv:2111.03930},
  year={2021}
}
@inproceedings{svladapterbmvc2022,
    author    = {Pantazis, Omiros and Brostow, Gabriel and Jones, Kate and Mac Aodha, Oisin},
    title     = {{SVL}-Adapter: Self-Supervised Adapter for Vision-Language Pretrained Models},
    booktitle = BMVC,
    year      = {2022}
}

@inproceedings{zhou2022extract,
  title={Extract free dense labels from {CLIP}},
  author={Zhou, Chong and Loy, Chen Change and Dai, Bo},
  booktitle=ECCV,
  pages={696--712},
  year={2022}
}

@inproceedings{zhang2023adding,
  title={Adding conditional control to text-to-image diffusion models},
  author={Zhang, Lvmin and Rao, Anyi and Agrawala, Maneesh},
  booktitle=ICCV,
  year={2023}
}

@misc{xiang2023closer,
      title={A Closer Look at Parameter-Efficient Tuning in Diffusion Models}, 
      author={Chendong Xiang and Fan Bao and Chongxuan Li and Hang Su and Jun Zhu},
      year={2023},
      eprint={2303.18181},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{wortsman2022robust,
  title={Robust fine-tuning of zero-shot models},
  author={Wortsman, Mitchell and Ilharco, Gabriel and Kim, Jong Wook and Li, Mike and Kornblith, Simon and Roelofs, Rebecca and Lopes, Raphael Gontijo and Hajishirzi, Hannaneh and Farhadi, Ali and Namkoong, Hongseok and others},
  booktitle=CVPR,
  pages={7959--7971},
  year={2022}
}

@article{poole2022dreamfusion,
  author = {Poole, Ben and Jain, Ajay and Barron, Jonathan T. and Mildenhall, Ben},
  title = {{DreamFusion}: Text-to-3D using 2D Diffusion},
  journal = {arXiv},
  year = {2022},
}

@article{xu20233difftection,
      title={{3DiffTection}: 3D Object Detection with Geometry-Aware Diffusion Features}, 
      author={Chenfeng Xu and Huan Ling and Sanja Fidler and Or Litany},
      year={2023},
      journal={arXiv}, 
}

--------------- other ---------------
@inproceedings{miangoleh2021boosting,
  title={Boosting monocular depth estimation models to high-resolution via content-adaptive multi-resolution merging},
  author={Miangoleh, S Mahdi H and Dille, Sebastian and Mai, Long and Paris, Sylvain and Aksoy, Yagiz},
  booktitle=CVPR,
  pages={9685--9694},
  year={2021}
}

@misc{whitaker2023multi-resolution,
author = {Kasiopy},
title = {Multi-Resolution Noise for Diffusion Model Training},
howpublished = {\url{https://wandb.ai/johnowhitaker/multires_noise/reports/Multi-Resolution-Noise-for-Diffusion-Model-Training--VmlldzozNjYyOTU2?s=31}},
note = {last accessed 17.11.2023},
year = 2023
}


@article{whitaker2023multi-resolution_bingxin,
	title = {Multi-Resolution Noise for Diffusion Model Training},
	journal = {\url{https://wandb.ai/johnowhitaker/multires_noise/reports/Multi-Resolution-Noise-for-Diffusion-Model-Training--VmlldzozNjYyOTU2?s=31}},
	author = {Whitaker, Jonathan},
        year = 2023,
	urldate = {2023-11-06},
}

@article{nachmani2021non,
  title={Non {Gaussian} denoising diffusion models},
  author={Nachmani, Eliya and Roman, Robin San and Wolf, Lior},
  journal={arXiv preprint arXiv:2106.07582},
  year={2021}
}

@article{fan2023optimizing,
  title={Optimizing {DDPM} sampling with shortcut fine-tuning},
  author={Fan, Ying and Lee, Kangwook},
  journal={arXiv preprint arXiv:2301.13362},
  year={2023}
}

@inproceedings{neuhold2017mapillary,
  title={The {Mapillary} {Vistas} dataset for semantic understanding of street scenes},
  author={Neuhold, Gerhard and Ollmann, Tobias and Rota Bulo, Samuel and Kontschieder, Peter},
  booktitle={IEEE International Conference on Computer Vision},
  year={2017}
}

@ARTICLE{Geiger2013IJRR,
  author = {Andreas Geiger and Philip Lenz and Christoph Stiller and Raquel Urtasun},
  title = {Vision meets Robotics: The {KITTI} Dataset},
  journal = {International Journal of Robotics Research},
  year = {2013}
}

@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={MICCAI},
  pages={234--241},
  year={2015}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={CVPR},
  pages={248--255},
  year={2009}
}

@article{oquab2023dinov2,
  title={{DINOv2}: Learning robust visual features without supervision},
  author={Oquab, Maxime and Darcet, Timoth{\'e}e and Moutakanni, Th{\'e}o and Vo, Huy and Szafraniec, Marc and Khalidov, Vasil and Fernandez, Pierre and Haziza, Daniel and Massa, Francisco and El-Nouby, Alaaeldin and others},
  journal={arXiv preprint arXiv:2304.07193},
  year={2023}
}


@article{razavi2019generating,
  title={Generating diverse high-fidelity images with vq-vae-2},
  author={Razavi, Ali and Van den Oord, Aaron and Vinyals, Oriol},
  journal={NIPS},
  volume={32},
  year={2019}
}

@article{yan2021videogpt,
  title={{VideoGPT}: Video generation using vq-vae and transformers},
  author={Yan, Wilson and Zhang, Yunzhi and Abbeel, Pieter and Srinivas, Aravind},
  journal={arXiv preprint arXiv:2104.10157},
  year={2021}
}

@inproceedings{zhang2018unreasonable,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle={CVPR},
  pages={586--595},
  year={2018}
}

@article{dosovitskiy2016generating,
  title={Generating images with perceptual similarity metrics based on deep networks},
  author={Dosovitskiy, Alexey and Brox, Thomas},
  journal={NeurIPS},
  volume={29},
  year={2016}
}



------------------- datasets ---------------------------
@inproceedings{qu2021bayesian,
  title={Bayesian deep basis fitting for depth completion with uncertainty},
  author={Qu, Chao and Liu, Wenxin and Taylor, Camillo J},
  booktitle={ICCV},
  pages={16147--16157},
  year={2021}
}


@INPROCEEDINGS{Geiger2012CVPR,
  author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
  title = {Are we ready for Autonomous Driving? The {KITTI} Vision Benchmark Suite},
  booktitle = {CVPR},
  year = {2012}
}

@inproceedings{schoeps2017cvpr,
	author = {Thomas Sch\"ops and Johannes L. Sch\"onberger and Silvano Galliani and Torsten Sattler and Konrad Schindler and Marc Pollefeys and Andreas Geiger},
	booktitle = {CVPR},
	title = {A Multi-View Stereo Benchmark with High-Resolution Images and Multi-Camera Videos},
	year = {2017}}

@inproceedings{gaidon2016virtual,
  title={Virtual worlds as proxy for multi-object tracking analysis},
  author={Gaidon, Adrien and Wang, Qiao and Cabon, Yohann and Vig, Eleonora},
  booktitle={CVPR},
  pages={4340--4349},
  year={2016}
}

@inproceedings{schops2017multiEth3d,
  title={A multi-view stereo benchmark with high-resolution images and multi-camera videos},
  author={Schops, Thomas and Schonberger, Johannes L and Galliani, Silvano and Sattler, Torsten and Schindler, Konrad and Pollefeys, Marc and Geiger, Andreas},
  booktitle={CVPR},
  pages={3260--3269},
  year={2017}
}

@inproceedings{dai2017scannet,
    title={{ScanNet}: Richly-annotated 3D Reconstructions of Indoor Scenes},
    author={Dai, Angela and Chang, Angel X. and Savva, Manolis and Halber, Maciej and Funkhouser, Thomas and Nie{\ss}ner, Matthias},
    booktitle = {CVPR},
    year = {2017}
}

@article{mirza2014conditional,
  title={Conditional generative adversarial nets},
  author={Mirza, Mehdi and Osindero, Simon},
  journal={arXiv preprint arXiv:1411.1784},
  year={2014}
}

@inproceedings{sohn2015cvae,
 author = {Sohn, Kihyuk and Lee, Honglak and Yan, Xinchen},
 booktitle = {NIPS},
 title = {Learning Structured Output Representation using Deep Conditional Generative Models},
 volume = {28},
 year = {2015}
}


@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{Huang2023nfl,
        title={Neural LiDAR Fields for Novel View Synthesis},
        author={Huang, Shengyu and Gojcic, Zan and Wang, Zian and Williams, Francis and Kasten, Yoni and Fidler, Sanja and Schindler, Konrad and Litany, Or},
        booktitle={ICCV},
        year={2023}
    }

@article{wagner2006gaussian,
  title={Gaussian decomposition and calibration of a novel small-footprint full-waveform digitising airborne laser scanner},
  author={Wagner, Wolfgang and Ullrich, Andreas and Ducic, Vesna and Melzer, Thomas and Studnicka, Nick},
  journal={ISPRS journal of Photogrammetry and Remote Sensing},
  volume={60},
  number={2},
  pages={100--112},
  year={2006},
  publisher={Elsevier}
}


@article{ZhangColorization2016,
  title = {Colorful Image Colorization},
  author = {Zhang, Richard and Isola, Phillip and Efros, Alexei A.},
  journal = {arXiv:1603.08511},
  year = {2016}
}

@article{Shakhnarovich2016,
  title = {Learning Representations for Automatic Colorization},
  author = {Larsson, Gustav and Maire, Michael and Shakhnarovich, Gregory},
  journal = {arXiv:1603.06668},
  year = {2016}
}

@article{dreamfusion,
    title = {DreamFusion: Text-to-3D using 2D Diffusion},
    author = {Poole, Ben and Jain, Ajay and Barron, Jonathan T. and Mildenhall, Ben},
    journal = {arXiv:2209.14988},
    year = {2022}
}

@article{instructpix2pix,
    title = {InstructPix2Pix: {L}earning to Follow Image Editing Instructions},
    author = {Brooks, Tim and Holynski, Aleksander and Efros, Alexei A.},
    journal = {arXiv},
    year = {2022}
}

@article{rin-2022,
  author = {Jabri, Allan and Fleet, David and Chen, Ting},
  title = {Scalable Adaptive Computation for Iterative Generation},
  journal = {arXiv:2212.11972},
  year = {2022}
}

@article{ImagenEditor, 
  title = {Imagen Editor and EditBench: Advancing and Evaluating Text-Guided Image Inpainting},
  author = {Wang, Su and Saharia, Chitwan and Montgomery, Ceslee and Pont-Tuset, Jordi and Noy, Shai and Pellegrini, Stefano and Onoe, Yasumasa and Laszlo, Sarah and Fleet, David J. and Soricut, Radu and Baldridge, Jason and Norouzi, Mohammad and Anderson, Peter and Chan, William},
  journal = {arXiv},
  year = {2022}
}

@article{3dim,
    title = {Novel View Synthesis with Diffusion Models},
    author = {Watson, Daniel and Chan, William and Martin-Brualla, Ricardo and Ho, Jonathan and Tagliasacchi, Andrea and Norouzi, Mohammad},
    journal = {arXiv:2210.04628},
     year = {2022}
}






@article{Bengio-2015-scheduled-sampling,
  author = {Bengio, Samy and Vinyals, Oriol and Jaitly, Navdeep and Shazeer, Noam},
  title = {Scheduled Sampling for Sequence Prediction with Recurrent Neural Networks},
  journal = {arXiv:1506.03099},
  year = {2015}
}

@inproceedings{Whang-cvpr2022,
  title={Deblurring via stochastic refinement
},
  author={Jay Whang and Mauricio Delbracio and Hossein Talebi and Chitwan Saharia and Alexandros G Dimakis and Peyman Milanfar},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={16293-16303},
  year={2022}
}

@article{AllInTokens,
  author = {Ning, Jia and Li, Chen and Zhang, Zheng and Geng, Zigang and Dai, Qi and He, Kun and Hu, Han},
  title = {All in Tokens: Unifying Output Space of Visual Tasks via Soft Token},
  journal = {arXiv:2301.02229},
  year = {2023}
}

@article{simmim,
  author = {Xie, Zhenda and Zhang, Zheng and Cao, Yue and Lin, Yutong and Bao, Jianmin and Yao, Zhuliang and Dai, Qi and Hu, Han},
  title = {{SimMIM}: {A} Simple Framework for Masked Image Modeling},
  journal = {arXiv:2111.09886},
  year = {2021}
}

@article{xie2022revealing,
    author={Zhenda Xie and Zigang Geng and Jingcheng Hu and Zheng Zhang and Han Hu and Yue Cao},
    title={Revealing the Dark Secrets of Masked Image Modeling},
    year={2022},
    journal={arxiv:2205.13543}
}

@article{shapenet,
  author = {Chang, Angel X. and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and Xiao, Jianxiong and Yi, Li and Yu, Fisher},
  title = {Shape{N}et: An Information-Rich 3D Model Repository},
  journal = {arXiv:1512.03012},
  year = {2015}
}

@article{pixelformer,
  author = {Agarwal, Ashutosh and Arora, Chetan},
  title = {Attention Attention Everywhere: Monocular Depth Prediction with Skip Attention},
  journal = {arxiv.2210.09071},
  year = {2022}
}

@article{binsformer,
  author = {Li, Zhenyu and Wang, Xuyang and Liu, Xianming and Jiang, Junjun},
  title = {BinsFormer: Revisiting Adaptive Bins for Monocular Depth Estimation},
  journal = {arxiv},
  year = {2022}
}

@inproceedings{dorn,
  title={Deep ordinal regression network for monocular depth estimation},
  author={Fu, Huan and Gong, Mingming and Wang, Chaohui and Batmanghelich, Kayhan and Tao, Dacheng},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={2002--2011},
  year={2018}
}

@article{scannet,
  author = {Dai, Angela and Chang, Angel X. and Savva, Manolis and Halber, Maciej and Funkhouser, Thomas and Nießner, Matthias},
  title = {{ScanNet}: Richly-annotated 3D Reconstructions of Indoor Scenes},
  journal = {arxiv:1702.04405},
  year = {2017}
}

@article{https://doi.org/10.48550/arxiv.1511.07041,
  author = {Handa, Ankur and Patraucean, Viorica and Badrinarayanan, Vijay and Stent, Simon and Cipolla, Roberto},
  title = {SceneNet: Understanding Real World Indoor Scenes With Synthetic Data},
  journal = {arXiv:1511.07041},
  year = {2015}
}


@article{scenenet-rgbd,
  author = {McCormac, John and Handa, Ankur and Leutenegger, Stefan and Davison, Andrew J.},
  title = {SceneNet RGB-D: 5M Photorealistic Images of Synthetic Indoor Trajectories with Ground Truth},
  journal = {arxiv:1612.05079},
  year = {2016}
}

@INPROCEEDINGS{waymoOpenDataset,
  author = {Sun, Pei and Kretzschmar, Henrik and Dotiwalla, Xerxes and Chouard, Aurelien and Patnaik, Vijaysai and Tsui, Paul and Guo, James and Zhou, Yin and Chai, Yuning and Caine, Benjamin and Vasudevan, Vijay and Han, Wei and Ngiam, Jiquan and Zhao, Hang and Timofeev, Aleksei and Ettinger, Scott and Krivokon, Maxim and Gao, Amy and Joshi, Aditya and Zhao, Sheng and Cheng, Shuyang and Zhang, Yu and Shlens, Jonathon and Chen, Zhifeng and Anguelov, Dragomir},
  title = {Scalability in Perception for Autonomous Driving: Waymo Open Dataset},
  booktitle = {CVPR},
  year = {2020}
}

@article{bts,
  title={From big to small: Multi-scale local planar guidance for monocular depth estimation},
  author={Lee, Jin Han and Han, Myung-Kyu and Ko, Dong Wook and Suh, Il Hong},
  journal={arXiv:1907.10326},
  year={2019}
}

@inproceedings{dpt,
    author    = {Ranftl, Ren\'e and Bochkovskiy, Alexey and Koltun, Vladlen},
    title     = {Vision transformers for dense prediction},
    booktitle = {ICCV},
    year      = {2021}
}

@article{ranftl2019robust,
    title={Towards Robust Monocular Depth Estimation: Mixing Datasets for Zero-shot Cross-dataset Transfer},
    author={René Ranftl and Katrin Lasinger and David Hafner and Konrad Schindler and Vladlen Koltun},
    year={2019},
    journal={arXiv}
}

@article{ren2017crossdomain,
    title={Cross-Domain Self-supervised Multi-task Feature Learning using Synthetic Imagery},
    author={Zhongzheng Ren and Yong Jae Lee},
    year={2017},
    journal={arXiv:1711.09082}
}

@article{zhou2017unsupervised,
    title={Unsupervised Learning of Depth and Ego-Motion from Video},
    author={Tinghui Zhou and Matthew Brown and Noah Snavely and David G. Lowe},
    year={2017},
    journal={arXiv:1704.07813}
}

@inproceedings{dav,
  title={Guiding monocular depth estimation using depth-attention volume},
  author={Huynh, Lam and Nguyen-Ha, Phong and Matas, Jiri and Rahtu, Esa and Heikkil{\"a}, Janne},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={581--597},
  year={2020},
  organization={Springer}
}

@inproceedings{adabins,
  title={Adabins: Depth estimation using adaptive bins},
  author={Bhat, Shariq Farooq and Alhashim, Ibraheem and Wonka, Peter},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={4009--4018},
  year={2021}
}

@inproceedings{carion2020detr,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={213--229},
  year={2020},
  organization={Springer}
}

@article{dosovitskiy2020vit,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@inproceedings{liu2021swin,
    author={Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
    title={Swin Transformer: Hierarchical vision transformer using shifted windows},
    booktitle={International Conference on Computer Vision (ICCV)},
    year={2021},
    pages={10012-10022}
}

@article{kitti,
  title={Vision meets robotics: The kitti dataset},
  author={Geiger, Andreas and Lenz, Philip and Stiller, Christoph and Urtasun, Raquel},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={11},
  pages={1231--1237},
  year={2013},
  publisher={Sage Publications Sage UK: London, England}
}

@inproceedings{sunrgbd,
  title={Sun rgb-d: A rgb-d scene understanding benchmark suite},
  author={Song, Shuran and Lichtenberg, Samuel P and Xiao, Jianxiong},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={567--576},
  year={2015}
}

@inproceedings{eigen2014depth,
 author = {Eigen, David and Puhrsch, Christian and Fergus, Rob},
 title = {Depth Map Prediction from a Single Image using a Multi-Scale Deep Network},
booktitle = {Advances in Neural Information Processing Systems (NIPS)},
 volume = {27},
 year = {2014}
}

@article{eigen2014predicting,
    title={Predicting Depth, Surface Normals and Semantic Labels with a Common Multi-Scale Convolutional Architecture},
    author={David Eigen and Rob Fergus},
    year={2014},
    journal={arXiv:1411.4734}
}

@inproceedings{diaz2019soft,
  title={Soft labels for ordinal regression},
  author={Diaz, Raul and Marathe, Amit},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={4738--4747},
  year={2019}
}


@InProceedings{transdepth,
    author={Zhao, Jiawei and Yan, Ke and Zhao, Yifan and Guo, Xiaowei and Huang, Feiyue and Li, Jia},
    title={Transformer-based dual relation graph for multi-label image recognition},
    booktitle={International Conference on Computer Vision (ICCV)},
    year={2021},
    pages={163-172}
}

@inproceedings{laina2016deeper,
  title={Deeper depth prediction with fully convolutional residual networks},
  author={Laina, Iro and Rupprecht, Christian and Belagiannis, Vasileios and Tombari, Federico and Navab, Nassir},
  booktitle={2016 Fourth international conference on 3D vision (3DV)},
  pages={239--248},
  year={2016},
}

@article{alhashim2018densedepth,
  title={High quality monocular depth estimation via transfer learning},
  author={Alhashim, Ibraheem and Wonka, Peter},
  journal={arXiv preprint arXiv:1812.11941},
  year={2018}
}

@inproceedings{wang2020cliffnet,
  title={Cliffnet for monocular depth estimation with hierarchical embedding loss},
  author={Wang, Lijun and Zhang, Jianming and Wang, Yifan and Lu, Huchuan and Ruan, Xiang},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={316--331},
  year={2020},
}

@inproceedings{zheng2021setr,
  title={Rethinking semantic segmentation from a sequence-to-sequence perspective with transformers},
  author={Zheng, Sixiao and Lu, Jiachen and Zhao, Hengshuang and Zhu, Xiatian and Luo, Zekun and Wang, Yabiao and Fu, Yanwei and Feng, Jianfeng and Xiang, Tao and Torr, Philip HS and others},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={6881--6890},
  year={2021}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems (NIPS)},
  pages={5998--6008},
  year={2017}
}

@inproceedings{hu2018senet,
  title={Squeeze-and-excitation networks},
  author={Hu, Jie and Shen, Li and Sun, Gang},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={7132--7141},
  year={2018}
}

@article{chen2019structure,
  title={Structure-aware residual pyramid network for monocular depth estimation},
  author={Chen, Xiaotian and Chen, Xuejin and Zha, Zheng-Jun},
  journal={arXiv preprint arXiv:1907.06023},
  year={2019}
}

@inproceedings{yin2019enforcing,
  title={Enforcing geometric constraints of virtual normal for depth prediction},
  author={Yin, Wei and Liu, Yifan and Shen, Chunhua and Yan, Youliang},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={5684--5693},
  year={2019}
}

@inproceedings{godard2017unsupervised,
  title={Unsupervised monocular depth estimation with left-right consistency},
  author={Godard, Cl{\'e}ment and Mac Aodha, Oisin and Brostow, Gabriel J},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={270--279},
  year={2017}
}

@inproceedings{johnston2020self,
  title={Self-supervised monocular trained depth estimation using self-attention and discrete disparity volume},
  author={Johnston, Adrian and Carneiro, Gustavo},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={4756--4765},
  year={2020}
}

@inproceedings{gan2018monocular,
  title={Monocular depth estimation with affinity, vertical pooling, and label enhancement},
  author={Gan, Yukang and Xu, Xiangyu and Sun, Wenxiu and Lin, Liang},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={224--239},
  year={2018}
}

@article{xu2020probabilistic,
  title={Probabilistic graph attention network with conditional kernels for pixel-wise prediction},
  author={Xu, Dan and Alameda-Pineda, Xavier and Ouyang, Wanli and Ricci, Elisa and Wang, Xiaogang and Sebe, Nicu},
  journal={Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  year={2020},
  publisher={IEEE}
}

@inproceedings{song2015sun,
  title={Sun rgb-d: A rgb-d scene understanding benchmark suite},
  author={Song, Shuran and Lichtenberg, Samuel P and Xiao, Jianxiong},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={567--576},
  year={2015}
}

@inproceedings{tan2019efficientnet,
  title={Efficientnet: Rethinking model scaling for convolutional neural networks},
  author={Tan, Mingxing and Le, Quoc},
  booktitle={International Conference on Machine Learning (ICML)},
  pages={6105--6114},
  year={2019},
}

@inproceedings{uhrig2017sparsity,
  title={Sparsity invariant cnns},
  author={Uhrig, Jonas and Schneider, Nick and Schneider, Lukas and Franke, Uwe and Brox, Thomas and Geiger, Andreas},
  booktitle={International Conference on 3D Vision (3DV)},
  pages={11--20},
  year={2017},
  organization={IEEE}
}

@inproceedings{garg2016unsupervised,
  title={Unsupervised cnn for single view depth estimation: {G}eometry to the rescue},
  author={Garg, Ravi and Bg, Vijay Kumar and Carneiro, Gustavo and Reid, Ian},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={740--756},
  year={2016},
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems (NIPS)},
  volume={32},
  pages={8026--8037},
  year={2019}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{he2016resenet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={770--778},
  year={2016}
}

@inproceedings{lin2017fpn,
  title={Feature pyramid networks for object detection},
  author={Lin, Tsung-Yi and Doll{\'a}r, Piotr and Girshick, Ross and He, Kaiming and Hariharan, Bharath and Belongie, Serge},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={2117--2125},
  year={2017}
}

@article{cheng2021maskformer,
  title={Per-pixel classification is not all you need for semantic segmentation},
  author={Cheng, Bowen and Schwing, Alex and Kirillov, Alexander},
  journal={Advances in Neural Information Processing Systems (NIPS)},
  volume={34},
  year={2021}
}

@article{chen2017deeplab,
  title={Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs},
  author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L},
  journal={IEEE transactions on pattern analysis and machine intelligence (TPAMI)},
  volume={40},
  number={4},
  pages={834--848},
  year={2017},
  publisher={IEEE}
}

@inproceedings{woo2018cbam,
  title={Cbam: Convolutional block attention module},
  author={Woo, Sanghyun and Park, Jongchan and Lee, Joon-Young and Kweon, In So},
  booktitle={European Conference on Computer Vision (ECCV)},
  pages={3--19},
  year={2018}
}

@article{cheng2021mask2former,
  title={Masked-attention mask transformer for universal image segmentation},
  author={Cheng, Bowen and Misra, Ishan and Schwing, Alexander G and Kirillov, Alexander and Girdhar, Rohit},
  journal={arXiv preprint arXiv:2112.01527},
  year={2021}
}

@inproceedings{zhu2020deformabledetr,
  title={Deformable detr: Deformable transformers for end-to-end object detection},
  author={Zhu, Xizhou and Su, Weijie and Lu, Lewei and Li, Bin and Wang, Xiaogang and Dai, Jifeng},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2021}
}

@article{aich2020BANet,
  title={Bidirectional attention network for monocular depth estimation},
  author={Aich, Shubhra and Vianney, Jean Marie Uwabeza and Islam, Md Amirul and Kaur, Mannat and Liu, Bingbing},
  journal={arXiv preprint arXiv:2009.00743},
  year={2020}
}

@inproceedings{lee2021PWA,
  title={Patch-Wise Attention Network for Monocular Depth Estimation},
  author={Lee, Sihaeng and Lee, Janghyeon and Kim, Byungju and Yi, Eojindl and Kim, Junmo},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  pages={1873--1881},
  year={2021}
}

@inproceedings{qiao2021vip,
  title={Vip-deeplab: Learning visual perception with depth-aware video panoptic segmentation},
  author={Qiao, Siyuan and Zhu, Yukun and Adam, Hartwig and Yuille, Alan and Chen, Liang-Chieh},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={3997--4008},
  year={2021}
}

@inproceedings{liu2019neural,
  title={Neural rgb (r) d sensing: Depth and uncertainty from a video camera},
  author={Liu, Chao and Gu, Jinwei and Kim, Kihwan and Narasimhan, Srinivasa G and Kautz, Jan},
  booktitle={Computer Vision and Pattern Recognition (CVPR)},
  pages={10986--10995},
  year={2019}
}

@inproceedings{kendall2017uncertainties,
  author={Alex Kendall and Yarin Gal},
  title={What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?},
  booktitle={Neural Information Processing Systems (NIPS)},
  pages={5574--5584},
  year={2017},
}

@inproceedings{godard2019digging,
  title={Digging into self-supervised monocular depth estimation},
  author={Godard, Cl{\'e}ment and Mac Aodha, Oisin and Firman, Michael and Brostow, Gabriel J},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={3828--3838},
  year={2019}
}

@inproceedings{jung2021fine,
  title={Fine-grained Semantics-aware Representation Enhancement for Self-supervised Monocular Depth Estimation},
  author={Jung, Hyunyoung and Park, Eunhyeok and Yoo, Sungjoo},
  booktitle={International Conference on Computer Vision (ICCV)},
  pages={12642--12652},
  year={2021}
}

@inproceedings{Chen-Chou2021,
  title={Depth Estimation From Monocular Images And Sparse Radar Using Deep Ordinal Regression Network},
  author={Lo, Chen-Chou and Vandewalle, Patrick},
  booktitle={International Conference on Image Processing (ICIP)},
  pages={3343--3347},
  year={2021},
}


%%%%%%%%%%%%%%%%%%%%%%%%%

@INPROCEEDINGS{sahariac-imagen,
  title = {{Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding}},
  author = {Chitwan Saharia and William Chan and Saurabh Saxena and Lala Li and Jay Whang and Emily Denton and Seyed Kamyar Seyed Ghasemipour and Burcu Karagol Ayan and S. Sara Mahdavi and Rapha Gontijo Lopes and Tim Salimans and Jonathan Ho and David J Fleet and Mohammad Norouzi},
  booktitle = {{NeurIPS}},
  year = {2022}
}

@INPROCEEDINGS{sahariac-palette,
  title = {{Palette: Image-to-Image Diffusion Models}},
  author = {Chitwan Saharia and William Chan and Huiwen Chang and Chris A. Lee and Jonathan Ho and Tim Salimans and David J. Fleet and Mohammad Norouzi},
  booktitle = {SIGGRAPH},
  year = {2022},
}

@article{nichol-glide,
  title = {{GLIDE: Towards Photorealistic Image Generation and Editing with Text-Guided Diffusion Models}},
  author = {Alex Nichol and Prafulla Dhariwal and Aditya Ramesh and Pranav Shyam and Pamela Mishkin, Bob McGrew and Ilya Sutskever and Mark Chen},
  year = {2021},
  journal = {arXiv}
}

@article{ramesh-dalle2,
  title = {Hierarchical Text-Conditional Image Generation with CLIP Latents},
  author = {Aditya Ramesh and Prafulla Dhariwal and Alex Nichol and Casey Chu and Mark Chen},
  journal = {arXiv},
  year = {2022}
}

@article{ho2020denoising,
  title={{Denoising Diffusion Probabilistic Models}},
  author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  journal={{NeurIPS}},
  year={2020}
}

@INPROCEEDINGS{ho-videodiffusion,
  title = {{Video Diffusion Models}},
  author = {Jonathan Ho and Tim Salimans and Alexey Gritsenko and William Chan and Mohammad Norouzi and David J. Fleet},
  booktitle = {NeurIPS},
  year = {2022}
}

@INPROCEEDINGS{dhariwal2021diffusion,
  title={Diffusion Models Beat {GAN}s on Image Synthesis},
  author={Dhariwal, Prafulla and Nichol, Alex},
  booktitle={{NeurIPS}},
  year={2022}
}

@article{nichol2021improved,
  title={Improved denoising diffusion probabilistic models},
  author={Nichol, Alex and Dhariwal, Prafulla},
  journal={arXiv},
  year={2021}
}

@article{saharia2021image,
  title={Image Super-Resolution via Iterative Refinement},
  author={Saharia, Chitwan and Ho, Jonathan and Chan, William and Salimans, Tim and Fleet, David J and Norouzi, Mohammad},
  journal={TPAMI},
  year={2022}
}

@inproceedings{
ho2021classifierfree,
title={Classifier-Free Diffusion Guidance},
author={Jonathan Ho and Tim Salimans},
booktitle={NeurIPS 2021 Workshop on Deep Generative Models and Downstream Applications},
year={2021}
} %url={https://openreview.net/forum?id=qw8AKxfYbI}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@inproceedings{krizhevsky2012imagenet,
  title={ImageNet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  year={2012}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{sohl2015deep,
  title={Deep unsupervised learning using nonequilibrium thermodynamics},
  author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle={ICML},
  year={2015}
}

@article{song2020denoising,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv preprint arXiv:2010.02502},
  year={2020}
} 

@inproceedings{song2021scorebased,
  title={Score-Based Generative Modeling through Stochastic Differential Equations},
  author={Yang Song and Jascha Sohl-Dickstein and Diederik P Kingma and Abhishek Kumar and Stefano Ermon and Ben Poole},
  booktitle={International Conference on Learning Representations},
  year={2021},
}

@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015},
  organization={Springer}
}

@article{ba2016layer,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1607.06450},
  year={2016}
}

@article{kingma2021variational,
  title={Variational diffusion models},
  author={Kingma, Diederik and Salimans, Tim and Poole, Ben and Ho, Jonathan},
  journal={Advances in neural information processing systems},
  volume={34},
  pages={21696--21707},
  year={2021}
}

@article{russakovsky2015imagenet,
  title={Imagenet large scale visual recognition challenge},
  author={Russakovsky, Olga and Deng, Jia and Su, Hao and Krause, Jonathan and Satheesh, Sanjeev and Ma, Sean and Huang, Zhiheng and Karpathy, Andrej and Khosla, Aditya and Bernstein, Michael and others},
  journal={International journal of computer vision},
  volume={115},
  number={3},
  pages={211--252},
  year={2015},
  publisher={Springer}
}

@article{karras2022elucidating,
  title={Elucidating the Design Space of Diffusion-Based Generative Models},
  author={Karras, Tero and Aittala, Miika and Aila, Timo and Laine, Samuli},
  journal={arXiv preprint arXiv:2206.00364},
  year={2022}
}


@article{luhman2022improving,
  title={Improving diffusion model efficiency through patching},
  author={Luhman, Troy and Luhman, Eric},
  journal={arXiv preprint arXiv:2207.04316},
  year={2022}
}

@article{peebles2022dit,
  author = {Peebles, William and Xie, Saining},
  title = {Scalable Diffusion Models with Transformers},
  journal = {arXiv preprint arXiv:2212.09748},
  year = {2022},
}

@InProceedings{Liba_2020_CVPR_Workshops,
author = {Liba, Orly and Cai, Longqi and Tsai, Yun-Ta and Eban, Elad and Movshovitz-Attias, Yair and Pritch, Yael and Chen, Huizhong and Barron, Jonathan T.},
title = {Sky Optimization: Semantically Aware Image Processing of Skies in Low-Light Photography},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR) Workshops},
month = {June},
year = {2020}
}
@inproceedings{DBLP:journals/corr/RanzatoCAZ15,
  author    = {Marc'Aurelio Ranzato and
               Sumit Chopra and
               Michael Auli and
               Wojciech Zaremba},
  title     = {Sequence Level Training with Recurrent Neural Networks},
  booktitle = {4th International Conference on Learning Representations (ICLR},
  year      = {2016}
}

@inproceedings{10.5555/2969239.2969370,
author = {Bengio, Samy and Vinyals, Oriol and Jaitly, Navdeep and Shazeer, Noam},
title = {Scheduled Sampling for Sequence Prediction with Recurrent Neural Networks},
year = {2015},
publisher = {MIT Press},
address = {Cambridge, MA, USA},
abstract = {Recurrent Neural Networks can be trained to produce sequences of tokens given some input, as exemplified by recent results in machine translation and image captioning. The current approach to training them consists of maximizing the likelihood of each token in the sequence given the current (recurrent) state and the previous token. At inference, the unknown previous token is then replaced by a token generated by the model itself. This discrepancy between training and inference can yield errors that can accumulate quickly along the generated sequence. We propose a curriculum learning strategy to gently change the training process from a fully guided scheme using the true previous token, towards a less guided scheme which mostly uses the generated token instead. Experiments on several sequence prediction tasks show that this approach yields significant improvements. Moreover, it was used succesfully in our winning entry to the MSCOCO image captioning challenge, 2015.},
booktitle = {Proceedings of the 28th International Conference on Neural Information Processing Systems - Volume 1},
pages = {1171–1179},
numpages = {9},
location = {Montreal, Canada},
series = {NIPS'15}
}

@ARTICLE{6795228,
  author={Williams, Ronald J. and Zipser, David},
  journal={Neural Computation}, 
  title={A Learning Algorithm for Continually Running Fully Recurrent Neural Networks}, 
  year={1989},
  volume={1},
  number={2},
  pages={270-280},
  doi={10.1162/neco.1989.1.2.270}}

@article{lamb2016professor,
    title={Professor Forcing: A New Algorithm for Training Recurrent Networks},
    author={Alex Lamb and Anirudh Goyal and Ying Zhang and Saizheng Zhang and Aaron Courville and Yoshua Bengio},
    year={2016},
    journal={arXiv:1610.09038}
}

@article{yu2016seqgan,
    title={SeqGAN: Sequence Generative Adversarial Nets with Policy Gradient},
    author={Lantao Yu and Weinan Zhang and Jun Wang and Yong Yu},
    year={2016},
    journal={arXiv:1609.05473}
}

@InProceedings{infinite_nature_2020,
  author = {Liu, Andrew and Tucker, Richard and Jampani, Varun and
            Makadia, Ameesh and Snavely, Noah and Kanazawa, Angjoo},
  title = {Infinite Nature: Perpetual View Generation of Natural Scenes from a Single Image},
  booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  month = {October},
  year = {2021}
}

@article{jing2022depth,
    title={Depth Estimation Matters Most: Improving Per-Object Depth Estimation for Monocular 3D Detection and Tracking},
    author={Longlong Jing and Ruichi Yu and Henrik Kretzschmar and Kang Li and Charles R. Qi and Hang Zhao and Alper Ayvaci and Xu Chen and Dillon Cower and Yingwei Li and Yurong You and Han Deng and Congcong Li and Dragomir Anguelov},
    year={2022},
    journal={arXiv:2206.03666}}
}

@article{zhou2019does,
    title={Does computer vision matter for action?},
    author={Brady Zhou and Philipp Krähenbühl and Vladlen Koltun},
    year={2019},
    journal={arXiv:1905.12887}
}

@inproceedings{NIPS2005_17d8da81,
 author = {Saxena, Ashutosh and Chung, Sung and Ng, Andrew},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {Y. Weiss and B. Sch\"{o}lkopf and J. Platt},
 pages = {},
 publisher = {MIT Press},
 title = {Learning Depth from Single Monocular Images},
 volume = {18},
 year = {2005}
}

@ARTICLE{4531745,
  author={Saxena, Ashutosh and Sun, Min and Ng, Andrew Y.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Make3D: Learning 3D Scene Structure from a Single Still Image}, 
  year={2009},
  volume={31},
  number={5},
  pages={824-840}
}

@article{cao2016estimating,
    title={Estimating Depth from Monocular Images as Classification Using Deep Fully Convolutional Residual Networks},
    author={Yuanzhouhan Cao and Zifeng Wu and Chunhua Shen},
    year={2016},
    journal={arXiv:1605.02305}
}

@article{wang2017learning,
    title={Learning Depth from Monocular Videos using Direct Methods},
    author={Chaoyang Wang and Jose Miguel Buenaposada and Rui Zhu and Simon Lucey},
    year={2017},
    journal={arXiv:1712.00175}
}

@misc{ranjan2018competitive,
    title={Competitive Collaboration: Joint Unsupervised Learning of Depth, Camera Motion, Optical Flow and Motion Segmentation},
    author={Anurag Ranjan and Varun Jampani and Lukas Balles and Kihwan Kim and Deqing Sun and Jonas Wulff and Michael J. Black},
    year={2018},
    eprint={1805.09806},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@misc{peebles2022scalable,
    title={Scalable Diffusion Models with Transformers},
    author={William Peebles and Saining Xie},
    year={2022},
    eprint={2212.09748},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@article{hertz2022prompttoprompt,
    title={Prompt-to-Prompt Image Editing with Cross Attention Control},
    author={Amir Hertz and Ron Mokady and Jay Tenenbaum and Kfir Aberman and Yael Pritch and Daniel Cohen-Or},
    year={2022},
    journal={arXiv}
}

@article{kawar2022imagic,
    title={Imagic: Text-Based Real Image Editing with Diffusion Models},
    author={Bahjat Kawar and Shiran Zada and Oran Lang and Omer Tov and Huiwen Chang and Tali Dekel and Inbar Mosseri and Michal Irani},
    year={2022},
    journal={arXiv:2210.09276}
}


@article{ruiz2022dreambooth,
    title={DreamBooth: Fine Tuning Text-to-Image Diffusion Models for Subject-Driven Generation},
    author={Nataniel Ruiz and Yuanzhen Li and Varun Jampani and Yael Pritch and Michael Rubinstein and Kfir Aberman},
    year={2022},
    journal={arXiv:2208.12242}
}

@article{nichol2022pointe,
    title={Point-E: A System for Generating 3D Point Clouds from Complex Prompts},
    author={Alex Nichol and Heewoo Jun and Prafulla Dhariwal and Pamela Mishkin and Mark Chen},
    year={2022},
    journal={arXiv:2212.08751}
}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}

@article{zhou2017places,
  title={Places: A 10 million Image Database for Scene Recognition},
  author={Zhou, Bolei and Lapedriza, Agata and Khosla, Aditya and Oliva, Aude and Torralba, Antonio},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2017},
  publisher={IEEE}
}

@ARTICLE{6664993,
  author={Stommel, Martin and Beetz, Michael and Xu, Weiliang},
  journal={IEEE Sensors Journal}, 
  title={Inpainting of Missing Values in the Kinect Sensor's Depth Maps Based on Background Estimates}, 
  year={2014},
  volume={14},
  number={4},
  pages={1107-1116}
}

@article{chen2022analog,
    title={Analog Bits: Generating Discrete Data using Diffusion Models with Self-Conditioning},
    author={Ting Chen and Ruixiang Zhang and Geoffrey Hinton},
    year={2022},
    journal={arXiv:2208.04202}
}


@article{asiedu2022decoder,
    title={Decoder Denoising Pretraining for Semantic Segmentation},
    author={Emmanuel Brempong Asiedu and Simon Kornblith and Ting Chen and Niki Parmar and Matthias Minderer and Mohammad Norouzi},
    year={2022},
    journal={arXiv:2205.11423}
}

@article{chen2022generalist,
    title={A Generalist Framework for Panoptic Segmentation of Images and Videos},
    author={Ting Chen and Lala Li and Saurabh Saxena and Geoffrey Hinton and David J. Fleet},
    year={2022},
    journal={arXiv}
}


@article{PixelSynth,
   title={PixelSynth: Generating a 3D-Consistent Experience from a Single Image},
   journal={IEEE/CVF International Conference on Computer Vision (ICCV)},
   author={Rockwell, Chris and Fouhey, David F. and Johnson, Justin},
   year={2021}
}

@inproceedings{
savinov2022stepunrolled,
title={Step-unrolled Denoising Autoencoders for Text Generation},
author={Nikolay Savinov and Junyoung Chung and Mikolaj Binkowski and Erich Elsen and Aaron van den Oord},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=T0GpzBQ1Fg6}
}

@article{yu2022monosdf,
  title={Monosdf: Exploring monocular geometric cues for neural implicit surface reconstruction},
  author={Yu, Zehao and Peng, Songyou and Niemeyer, Michael and Sattler, Torsten and Geiger, Andreas},
  journal={NeurIPS},
  year={2022}
}

@inproceedings{zhang2023completionformer,
  title={Completionformer: Depth completion with convolutions and vision transformers},
  author={Zhang, Youmin and Guo, Xianda and Poggi, Matteo and Zhu, Zheng and Huang, Guan and Mattoccia, Stefano},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={18527--18536},
  year={2023}
}

@article{esser2024stablev3,
  title={Scaling Rectified Flow Transformers for High-Resolution Image Synthesis},
  author={Esser, Patrick and Kulal, Sumith and Blattmann, Andreas and Entezari, Rahim and M{\"u}ller, Jonas and Saini, Harry and Levi, Yam and Lorenz, Dominik and Sauer, Axel and Boesel, Frederic and others},
  journal={ICML},
  year={2024}
}

@inproceedings{zhang2024improving,
  title={Improving Training Efficiency of Diffusion Models via Multi-Stage Framework and Tailored Multi-Decoder Architecture},
  author={Zhang, Huijie and Lu, Yifu and Alkhouri, Ismail and Ravishankar, Saiprasad and Song, Dogyoon and Qu, Qing},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7372--7381},
  year={2024}
}

@inproceedings{geiger2012we_kitti,
  title={Are we ready for autonomous driving? the kitti vision benchmark suite},
  author={Geiger, Andreas and Lenz, Philip and Urtasun, Raquel},
  booktitle={2012 IEEE conference on computer vision and pattern recognition},
  pages={3354--3361},
  year={2012},
  organization={IEEE}
}


@article{lee2024improving,
  title={Improving the Training of Rectified Flows},
  author={Lee, Sangyun and Lin, Zinan and Fanti, Giulia},
  journal={arXiv preprint arXiv:2405.20320},
  year={2024}
}

@article{hu2024metric3d,
  title={Metric3D v2: A Versatile Monocular Geometric Foundation Model for Zero-shot Metric Depth and Surface Normal Estimation},
  author={Hu, Mu and Yin, Wei and Zhang, Chi and Cai, Zhipeng and Long, Xiaoxiao and Chen, Hao and Wang, Kaixuan and Yu, Gang and Shen, Chunhua and Shen, Shaojie},
  journal={arXiv preprint arXiv:2404.15506},
  year={2024}
}

@article{hu2021lora,
  title={Lora: Low-rank adaptation of large language models},
  author={Hu, Edward J and Shen, Yelong and Wallis, Phillip and Allen-Zhu, Zeyuan and Li, Yuanzhi and Wang, Shean and Wang, Lu and Chen, Weizhu},
  journal={arXiv preprint arXiv:2106.09685},
  year={2021}
}

@inproceedings{li2017learning,
  title={Learning from noisy labels with distillation},
  author={Li, Yuncheng and Yang, Jianchao and Song, Yale and Cao, Liangliang and Luo, Jiebo and Li, Li-Jia},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1910--1918},
  year={2017}
}


@article{fu2024geowizard,
  title={GeoWizard: Unleashing the Diffusion Priors for 3D Geometry Estimation from a Single Image},
  author={Fu, Xiao and Yin, Wei and Hu, Mu and Wang, Kaixuan and Ma, Yuexin and Tan, Ping and Shen, Shaojie and Lin, Dahua and Long, Xiaoxiao},
  journal={arXiv preprint arXiv:2403.12013},
  year={2024}
}

@article{zhang2024betterdepth,
  title={BetterDepth: Plug-and-Play Diffusion Refiner for Zero-Shot Monocular Depth Estimation},
  author={Zhang, Xiang and Ke, Bingxin and Riemenschneider, Hayko and Metzger, Nando and Obukhov, Anton and Gross, Markus and Schindler, Konrad and Schroers, Christopher},
  journal={arXiv preprint arXiv:2407.17952},
  year={2024}
}


@article{yang2024depthanything,
  title={Depth anything: Unleashing the power of large-scale unlabeled data},
  author={Yang, Lihe and Kang, Bingyi and Huang, Zilong and Xu, Xiaogang and Feng, Jiashi and Zhao, Hengshuang},
  journal={arXiv preprint arXiv:2401.10891},
  year={2024}
}


@article{yang2024depthanythingv2,
  title={Depth Anything V2},
  author={Yang, Lihe and Kang, Bingyi and Huang, Zilong and Zhao, Zhen and Xu, Xiaogang and Feng, Jiashi and Zhao, Hengshuang},
  journal={arXiv preprint arXiv:2406.09414},
  year={2024}
}

@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
}
@misc{sanh2020distilbert,
      title={DistilBERT, a distilled version of BERT: smaller, faster, cheaper and lighter}, 
      author={Victor Sanh and Lysandre Debut and Julien Chaumond and Thomas Wolf},
      year={2020},
      eprint={1910.01108},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{aguilar2020knowledge,
  title={Knowledge distillation from internal representations},
  author={^ar, Gustavo and Ling, Yuan and Zhang, Yu and Yao, Benjamin and Fan, Xing and Guo, Chenlei},
  booktitle={AAAI},
  volume={34},
  number={05},
  pages={7350--7357},
  year={2020}
}

@inproceedings{jin2019knowledge,
  title={Knowledge distillation via route constrained optimization},
  author={Jin, Xiao and Peng, Baoyun and Wu, Yichao and Liu, Yu and Liu, Jiaheng and Liang, Ding and Yan, Junjie and Hu, Xiaolin},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1345--1354},
  year={2019}
}

@article{tarvainen2017mean,
  title={Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
  author={Tarvainen, Antti and Valpola, Harri},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@InProceedings{zhang2019byot,
author = {Zhang, Linfeng and Song, Jiebo and Gao, Anni and Chen, Jingwei and Bao, Chenglong and Ma, Kaisheng},
title = {Be Your Own Teacher: Improve the Performance of Convolutional Neural Networks via Self Distillation},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}

@inproceedings{xie2020self,
  title={Self-training with noisy student improves imagenet classification},
  author={Xie, Qizhe and Luong, Minh-Thang and Hovy, Eduard and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={10687--10698},
  year={2020}
}

@inproceedings{shen2019amalgamating,
  title={Amalgamating knowledge towards comprehensive classification},
  author={Shen, Chengchao and Wang, Xinchao and Song, Jie and Sun, Li and Song, Mingli},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={3068--3075},
  year={2019}
}

@inproceedings{ye2019student,
  title={Student becoming the master: Knowledge amalgamation for joint scene parsing, depth estimation, and more},
  author={Ye, Jingwen and Ji, Yixin and Wang, Xinchao and Ou, Kairi and Tao, Dapeng and Song, Mingli},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2829--2838},
  year={2019}
}

@inproceedings{ye2020distilling,
  title={Distilling cross-task knowledge via relationship matching},
  author={Ye, Han-Jia and Lu, Su and Zhan, De-Chuan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12396--12405},
  year={2020}
}

@article{auty2024learning,
  title={Learning to Project for Cross-Task Knowledge Distillation},
  author={Auty, Dylan and Miles, Roy and Kolbeinsson, Benedikt and Mikolajczyk, Krystian},
  journal={arXiv preprint arXiv:2403.14494},
  year={2024}
}

@article{zhuang2020comprehensive,
  title={A comprehensive survey on transfer learning},
  author={Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  journal={Proceedings of the IEEE},
  volume={109},
  number={1},
  pages={43--76},
  year={2020},
  publisher={IEEE}
}
@inproceedings{evci2022head2toe,
  title={Head2toe: Utilizing intermediate representations for better transfer learning},
  author={Evci, Utku and Dumoulin, Vincent and Larochelle, Hugo and Mozer, Michael C},
  booktitle={International Conference on Machine Learning},
  pages={6009--6033},
  year={2022},
  organization={PMLR}
}
@inproceedings{zamir2018taskonomy,
  title={Taskonomy: Disentangling task transfer learning},
  author={Zamir, Amir R and Sax, Alexander and Shen, William and Guibas, Leonidas J and Malik, Jitendra and Savarese, Silvio},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3712--3722},
  year={2018}
}

@article{liu2021data_SFDA,
  title={Data-free knowledge transfer: A survey},
  author={Liu, Yuang and Zhang, Wei and Wang, Jun and Wang, Jianyong},
  journal={arXiv preprint arXiv:2112.15278},
  year={2021}
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak






\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\Eb}[2]{\E_{#1}\!\left[#2\right]}
\newcommand{\Vara}[1]{\Var\left[#1\right]}
\newcommand{\Varb}[2]{\Var_{#1}\left[#2\right]}
\newcommand{\kl}[2]{D_{\mathrm{KL}}\!\left(#1 ~ \| ~ #2\right)}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bk}{\mathbf{k}}

\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bt}{\mathbf{t}}

\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bxh}{\hat{\mathbf{x}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\bnu}{{\boldsymbol{\nu}}}
\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}




